Swarm Reinforcement Learning For Adaptive Mesh Refinement

Adaptive Mesh Refinement (AMR) enhances the Finite Element Method, an important technique for simulating complex problems in engineering, by dynamically refining mesh regions, enabling a favorable trade-off between computational speed and simulation accuracy. Classical methods for AMR depend on heuristics or expensive error estimators, hindering their use for complex simulations. Recent learning-based AMR methods tackle these issues, but so far scale only to simple toy examples. We formulate AMR as a novel Adaptive Swarm Markov Decision Process in which a mesh is modeled as a system of simple collaborating agents that may split into multiple new agents. This framework allows for a spatial reward formulation that simplifies the credit assignment problem, which we combine with Message Passing Networks to propagate information between neighboring mesh elements. We experimentally validate our approach, Adaptive Swarm Mesh Refinement (ASMR), on challenging refinement tasks. Our approach learns reliable and efficient refinement strategies that can robustly generalize to different domains during inference. Additionally, it achieves a speedup of up to $2$ orders of magnitude compared to uniform refinements in more demanding simulations. We outperform learned baselines and heuristics, achieving a refinement quality that is on par with costly error-based oracle AMR strategies.

==> figures/quantitative_results/group_laplace_1.tex <==
\nextgroupplot[
ylabel shift = -0.2cm,
clip marker paths=true,
width=0.52\textwidth,
height=4.5cm,
title style={yshift=-0.2cm},
scaled x ticks=false,
xlabel style={yshift=0.1cm},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
title={Laplace's Equation - $4$ Refinements},
x grid style={darkgray176},
xlabel={Elements \(\displaystyle (\times 10^3)\)},
xmajorgrids,
xmin=-25.683, xmax=1252.583,
xtick style={color=black},
xtick={-200,0,200,400,600,800,1000,1200,1400},
xticklabels={-0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2,1.4},
y grid style={darkgray176},
ylabel={Squared Error},
ymajorgrids,
% ymin=1.43078625778226e-05, ymax=1.8415257818879,
ymin=0.000709423733196768, ymax=1.47892507920094,
ymode=log,
ytick style={color=black},
ytick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
}
]
\addplot [
  draw=royalblue28108204,
  fill=royalblue28108204,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
65.38 0.19548033495384
66 0.191794835079591
66.08 0.192070664343811
66.3 0.196434785913276
66.78 0.192478475552629
67.06 0.187944471995452
68.46 0.184907868176787
69.66 0.177028533656822
70.36 0.182161958366189
120.36 0.0480171428430439
122.68 0.047694026845006
127.32 0.0448494192480857
130.62 0.0577881441547467
132.5 0.0509434521981089
136.8 0.0454124189116922
139.52 0.048932160446244
143.3 0.048400659507082
144.56 0.0427771745833412
150.74 0.0483446798498261
258.66 0.0126682442445898
268.2 0.0119073945970959
277.3 0.0160403455187249
279.14 0.0105238244566487
287.74 0.0098525040922498
288.44 0.0101456099695037
318.62 0.00977545048314397
357.1 0.00793074374419599
371.22 0.00799876854190584
385.82 0.00697000819392388
387.02 0.00786048126070514
393.24 0.00759085732896779
401.02 0.00854927962995766
402.34 0.00780930379844022
403.56 0.00598876394680501
411 0.00783458509412708
447.36 0.00757923107445133
474.88 0.00459983187757483
490.18 0.00440575062285678
493.86 0.00449417071987142
543.14 0.0037910104095389
551.02 0.00434450155829541
567.62 0.175482274900737
612.54 0.0034840871426638
682.36 0.00230171838471891
721.4 0.00208353576509125
728.54 0.00194643674934622
754.66 0.00189741573664042
765.54 0.00232687058677731
803.94 0.00227709803699267
846.98 0.00159855681453347
874.18 0.00194857048376805
890.84 0.00147871786175772
906.94 0.0018106475297806
924.56 0.00151829854728709
947.56 0.00168327417293627
963.4 0.0013293475544881
988.66 0.00133498670167742
1014 0.00153825568850375
1075.08 0.00140442811928879
1114.38 0.00163746488048957
1172.44 0.00127647737473206
1178.12 0.00129208752662382
1190.04 0.0013201040766007
1190.3 0.00128852533748617
};
\addplot [
  draw=cadetblue80178158,
  fill=cadetblue80178158,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
76.3 0.205465485159958
76.5 0.199728996348629
76.78 0.268508023059704
77.06 0.236432444157531
77.84 0.191046800565188
78.3 0.198393592452147
78.74 0.226829249696703
79.36 0.20664901867851
85.58 0.230586829427313
89.72 0.314227977860585
122.84 0.0751099614989759
123.94 0.0550291713900843
127.7 0.0982519814616353
128.9 0.0729185856055236
130.94 0.0582117661595359
131.68 0.0894814197730012
136 0.0534892036134652
137.08 0.0839454856366417
144.14 0.116363702510754
147.26 0.192013542511006
162.38 0.058818141504049
166.02 0.0798113724545108
167.68 0.0407616811811036
169.9 0.0332989052099363
172.1 0.198234939391934
172.16 0.0379111564401634
186.28 0.0392000099502411
187.32 0.0296236542170356
197.88 0.046516534625511
198.32 0.0519904933933881
199.76 0.0417115974343281
210.54 0.0335563741749861
212.02 0.0333089614738129
218.44 0.029758656471716
219.06 0.0258203544370221
220.54 0.0338868124414272
225.44 0.0277105074945794
230.38 0.0307941057612529
246.4 0.0188507527319903
255.96 0.0492440903377289
306.16 0.0319765826848031
309.92 0.0113919612392918
312.44 0.0190555258997786
313.98 0.0143824219205634
329.16 0.0204004016383545
336.42 0.0176956800622428
338.7 0.0165057453173889
341.14 0.017132807912558
342.02 0.0191829367864913
352.94 0.0121156794333723
381.18 0.0103917345920111
393.76 0.0160489631855795
395.52 0.0125323432328433
421.18 0.0098311083874372
425.28 0.0117035786213194
468.96 0.010873781193783
472.92 0.00556119277744241
475.62 0.00529001285822559
479.66 0.0695280395329216
505.24 0.0167444954541683
510.58 0.102603235715894
510.74 0.0106270855010055
520.4 0.00848185116164715
527.84 0.0108032058997219
535.68 0.00672643832235808
539.52 0.00582425314479223
550.58 0.00951400954749761
561.36 0.0037562560331028
571.02 0.0251786721937385
604.32 0.00613558297446528
608.56 0.00350353235520922
610.18 0.0107175801335459
616.82 0.00753919187970688
625.06 0.0135309989884857
646.76 0.00381163826325673
647.74 0.0118130395764562
648.42 0.0102063680100813
653.58 0.0092690441868852
677.28 0.0115928998175296
677.74 0.0071844851773329
709.78 0.00762817321203376
726.3 0.00728491513844455
741.84 0.00927074952933055
751.32 0.0148440487197465
807.48 0.0108265620792889
835.86 0.00979563012887476
856.3 0.0157451875434538
878.68 0.00546548489378337
885.34 0.0133596159845129
892.46 0.00962885303338184
907 0.00286763780992378
911.56 0.0128261695193435
913.28 0.00918311750268795
943.22 0.00251651347817735
961.66 0.0042055788663924
984.84 0.0104601463159832
1005.62 0.0110199942008356
1030.16 0.0105451279233217
1032.48 0.0105415645295325
1129.02 0.00291537514140832
};
\addplot [
  draw=chocolate21910927,
  fill=chocolate21910927,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
32.92 0.999999999807618
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
78.16 0.19208726520201
78.48 0.176679430275259
83.28 0.158069517465207
106.84 0.0892168474889401
148.24 0.0445069820912839
150.74 0.0427965849436475
159.52 0.0674090070489176
170.94 0.0341593755505335
188.24 0.0422337384659872
189.8 0.0360895476723526
192.32 0.0349828478017722
218.38 0.0285778121824681
231.62 0.0306930238865907
289.44 0.0161597828025763
306.1 0.0253617784590629
348.78 0.0161789154609732
350.28 0.0104280944022337
374.54 0.00896544267119595
527.68 0.0273828282351929
534.74 0.005194292944181
624.06 0.012920692317797
627.46 0.0046872200690177
670.46 0.00966075426727153
673.18 0.00533938917535204
870.86 0.00220214623919551
931.88 0.00249668217998382
933.68 0.00333814311920321
999.16 0.00799457203338501
1103.66 0.00147039188012951
};
\addplot [draw=purple11522131, fill=purple11522131, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
32.42 0.99999999979668
32.8 0.999999999784238
32.86 0.999999999811253
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.22 0.999999999806546
33.32 0.999999999807761
33.52 0.999999999809443
48.96 0.857013542697787
50.46 0.709188666183198
50.58 0.666769832565613
60.76 0.459088241371385
61.44 0.350452114391466
68.26 0.288839161428196
71.46 0.229983114300637
72.06 0.36082464216482
72.88 0.20393271986151
73.54 0.308652293655439
73.6 0.340640393131014
77.74 0.235544966894596
83.18 0.157622196348201
85.86 0.219071298043835
87 0.158170505353671
87.8 0.147345723147572
89.74 0.158924446716746
89.96 0.878518902472353
106.8 0.515728610230431
107.94 0.160238296334473
108.08 0.18518751559111
108.24 0.420990561999015
112.96 0.16423725858114
119.3 0.165320431942191
121.1 0.165931879614546
121.4 0.321283439802619
122.9 0.103799561941819
123.52 0.105689856218511
123.54 0.16701071167221
125.04 0.16708809389227
130.48 0.167833542193555
154.06 0.0778627801544556
174.88 0.0460775276240287
176.84 0.0503502665916493
179.44 0.0397825157224299
189.12 0.0412902252577953
194.12 0.0341570652607007
198.14 0.0687003057995589
219.84 0.0280073437356045
281.78 0.0274521787672049
303.1 0.0253143258938404
304.94 0.0224097632744356
325.68 0.0258068415587312
332.4 0.0251604832248979
344.9 0.025045960282952
350.12 0.0261480927027984
350.68 0.0254388591828299
354.12 0.0252242285708618
391.34 0.0234765480191671
394.14 0.0168973787130159
428.78 0.0219485277900936
436.52 0.0262508997212733
441.98 0.0219754757537947
462.58 0.0266585369095283
465.1 0.0266736377380999
472.16 0.0267677033051448
479.82 0.0268913483855246
489.12 0.0269728868955202
490.42 0.0270106495864003
502.86 0.0268173448135813
511.14 0.0186048679904556
517.32 0.0273227513032658
519.14 0.027313509898968
523.6 0.0273625966651678
534.34 0.0252183399445867
540.98 0.00558923008230333
550.3 0.00659625782316353
554.18 0.0205511309950678
568.38 0.00565130509576207
572.66 0.0195363662654747
594.08 0.00489074931177106
594.5 0.0155046874354411
613.52 0.00992240454306736
618.28 0.00917472292027666
628.42 0.00815132535698754
675.78 0.00522437973590881
695.28 0.00591349315041835
705.74 0.00596983723727568
779.66 0.00477986224325563
860.2 0.00527895290394453
905.84 0.00546349938788228
916.2 0.00422820972736008
950.76 0.00405083939721978
1078.88 0.00387161460864726
1099.72 0.00416131266154231
1112.96 0.003896734728369
1192.36 0.00388957820975332
};
\addplot [
  draw=saddlebrown1356716,
  fill=saddlebrown1356716,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
527.68 0.0273828282351928
543.44 0.0206197589702108
546.14 0.0199960407596653
546.32 0.0190494580103563
554.54 0.0178789651908424
557.02 0.0170047459002408
563.94 0.0159437325089741
569.84 0.0151802950427584
571.42 0.0139017729483819
580.94 0.0128718596963898
587.8 0.0119006151003939
604.56 0.0107316735305262
607.52 0.00995977456562595
612.32 0.00883213105532234
621.8 0.00793801586556377
634.48 0.00718829854140163
644.5 0.00661303019443451
656.28 0.00577232587704204
664.18 0.00529071515119532
673.34 0.00471679743403248
680.98 0.00431694993840502
693.52 0.00402307957651328
702.76 0.00385297672387864
710.04 0.0036411683594868
710.68 0.00342406336295795
712.5 0.00352041585787605
714.72 0.00335782227158843
718.26 0.00331524822533228
725.92 0.00325277475395145
727.64 0.00297047313599306
728.9 0.00312440344456086
731.96 0.00301132456649942
732.3 0.0031630453917349
732.32 0.00294340008228144
732.78 0.00308674284662165
735.84 0.00288445221539916
740.56 0.00285698988569658
748.3 0.00282256998617187
749.98 0.00276711058180146
750.36 0.00273737826458943
757.26 0.00269156226523191
761.68 0.00266563529910175
766.34 0.00261902225988932
772.38 0.00257210077962337
775 0.00254041350906791
783.64 0.0025019112082084
791.26 0.00245298391869523
804.58 0.00240547319137145
807.04 0.00236906302342152
812.96 0.00232348311573666
822.78 0.00227357433712471
829.7 0.00221648706256762
839.3 0.00215125378854426
854.52 0.00209827736272589
868.94 0.00203345529873997
884.32 0.00197665679957575
898.38 0.00191758976365112
915.34 0.00186552303606368
936.12 0.00181537045391688
959.72 0.00176547062463419
983.86 0.00171224802847546
1000.44 0.00166095598994307
1030.16 0.00160749384957793
1053.9 0.00155304565408314
1081.54 0.00149598233282043
1116.44 0.00143974647692138
1148.22 0.00137412446613368
1173.3 0.00132156974562009
1194.48 0.0012727086799958
};
\addplot [draw=black18, fill=black18, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
33.2 0.99999999980788
70.92 0.225107596237741
72.76 0.210878345665069
75.28 0.195996728090339
76.76 0.179821853828445
77.16 0.189186085647883
77.18 0.172395306621637
80.54 0.166532004779595
83.08 0.15640544420268
83.62 0.151899105043405
84.98 0.141061708217509
86.92 0.136756465291971
89.16 0.13193381931812
90.86 0.128364960917746
93.24 0.121023311846883
95.82 0.11683685395527
98.68 0.110696814739449
100.04 0.106652042608072
106.1 0.0990157514507826
108.6 0.0958037470928353
110.9 0.0916811967899963
114.26 0.0879352530105515
121.98 0.0804927779728151
125.08 0.0749744289469566
129.88 0.0701090250419114
137.36 0.0661427503318755
137.96 0.0616618798829065
138.56 0.0643162833449804
146.74 0.0575615410826055
151.42 0.0507584773680926
151.8 0.0533383833594549
157.42 0.0484748791368032
158.86 0.0455877654387877
170.26 0.0414058464345257
175.16 0.0405741100806877
177.94 0.0395937650887451
181.54 0.0377208862386256
187.42 0.0360065755157114
191.68 0.0347087760098523
201.56 0.032966410093777
212.46 0.031737875908739
221.92 0.0288795818996223
241.02 0.02691400780356
243.32 0.0265479408130891
258.66 0.0250513026575173
265.58 0.0243254374136645
280.32 0.0227434388289943
296.04 0.020549030642554
334.26 0.018114845910122
344.34 0.0165030050085225
367.48 0.0143470192697269
386.12 0.0128236669560975
406.78 0.0112895895958993
422.12 0.010454086909242
440.08 0.0100144397218935
468.9 0.008923752709477
493.18 0.00832944146110404
519.32 0.00753617880491297
520.54 0.00792968999973277
566.46 0.00702006986026507
580.9 0.00680971120716808
614.12 0.00627910046459291
615.16 0.00664703766996395
657.72 0.00583437512760543
679.26 0.00537013779222168
733 0.00491744624637688
800.96 0.00435805460058907
856.46 0.00374740730965687
965.58 0.00294345663994793
1033.16 0.00249308516463351
1124.1 0.00203993667239804
};
\addplot [draw=darkgray153, fill=darkgray153, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
33.2 0.99999999980788
94.2 0.146898781674562
98.58 0.131440060714341
102.94 0.118337936175393
109.12 0.108547674479112
110.96 0.102349619725666
117.88 0.0892750673675453
122.44 0.0841616726417896
130.9 0.0727116060914542
139.14 0.060773178882216
143.68 0.056597628011066
146.74 0.0526266439982455
153.22 0.0480471360960284
162.1 0.0423493168429771
164.68 0.0386195445590377
169.8 0.0366257177652276
173.34 0.0330550466856225
181.14 0.0301750607939932
187.74 0.0279630975921603
194.48 0.0263370315706119
209.46 0.0233350560267512
214.86 0.0213804439299003
228.42 0.0195288273293355
244.8 0.0182010849527372
253.56 0.0166205129067125
269.7 0.0155398507232313
273.08 0.0148008217120132
277.48 0.0142896387230598
279.34 0.0138327306032203
291.5 0.013332931856778
303.14 0.0126724564937917
307.24 0.012244288126889
319.36 0.0117233613682811
325.04 0.0113465086157211
333.82 0.011010812498001
340.54 0.0108889985449065
340.92 0.0105626597761737
347.44 0.0102452097619355
354.38 0.0100376512284405
364.4 0.00956336713965051
370.22 0.00946749186401524
375.22 0.00935585082677941
380.06 0.00911345428250314
385.22 0.00891087582637739
392.5 0.0082576189988107
404.62 0.00794268808103291
408.5 0.00761811826188275
414.36 0.00750572925557215
420.7 0.00737799760713919
431.94 0.00717973797223086
439.34 0.00709496012835279
446.18 0.00680961600383507
460.4 0.00665589394849501
469.2 0.00655442591898147
474.06 0.0064723519682569
480.88 0.00628200304794249
494.94 0.00607217154885291
505.66 0.00570217353975976
520.64 0.00540801800494306
537.18 0.00505334052160283
553.08 0.00484407380299492
585.38 0.00461406655821698
609.34 0.00441128979556557
619.54 0.00423650396543048
640.14 0.00397010239991094
671.98 0.00369193115109039
704.52 0.00348266400715053
725.04 0.00321538415349773
745.32 0.00302591878402954
778.02 0.00284903645424013
844.42 0.00266819421839824
845.92 0.00246863213295377
877.88 0.0022863686062408
911.22 0.00214779226486312
972.06 0.00197310734421594
1005.38 0.0018494568096292
1048.44 0.00170164075361647
1111.46 0.00156526357409355
1197 0.0014415442009507
};
\addplot [very thick, royalblue28108204]
table {%
33.2 0.967996332162016
44.8878787878788 0.492446143430125
56.5757575757576 0.297538379835009
68.2636363636364 0.199545140678946
79.9515151515152 0.143501053679194
91.6393939393939 0.108472295407294
103.327272727273 0.0851107062912926
115.015151515152 0.0687399070932763
126.70303030303 0.0568121693235734
138.390909090909 0.0478438942618811
150.078787878788 0.0409237058135923
161.766666666667 0.0354666255925734
173.454545454545 0.0310831462762422
185.142424242424 0.0275057139552456
196.830303030303 0.0245455625361676
208.518181818182 0.0220663823921856
220.206060606061 0.0199677178710278
231.893939393939 0.0181741918143809
243.581818181818 0.0166283312041654
255.269696969697 0.0152856808660273
266.957575757576 0.0141114072839894
278.645454545455 0.0130778945857951
290.333333333333 0.0121630144770174
302.021212121212 0.0113488623297868
313.709090909091 0.0106208210606687
325.39696969697 0.00996685900518982
337.084848484848 0.00937699716352011
348.772727272727 0.00884290061470941
360.460606060606 0.00835756204106233
372.148484848485 0.00791505433277627
383.836363636364 0.00751033553065178
395.524242424242 0.00713909380004466
407.212121212121 0.00679762329553245
418.9 0.00648272406146144
430.587878787879 0.00619162078085393
442.275757575758 0.0059218964133539
453.963636363636 0.00567143767598709
465.651515151515 0.00543839000525877
477.339393939394 0.00522112015683252
489.027272727273 0.00501818499350447
500.715151515151 0.00482830531495706
512.40303030303 0.00465034381677738
524.090909090909 0.00448328644827344
535.778787878788 0.00432622658113759
547.466666666667 0.00417835151324219
559.154545454546 0.0040389309207441
570.842424242424 0.00390730694245902
582.530303030303 0.00378288563712424
594.218181818182 0.00366512959974329
605.906060606061 0.00355355156003964
617.593939393939 0.00344770881594974
629.281818181818 0.00334719837946984
640.969696969697 0.00325165273213533
652.657575757576 0.00316073610382436
664.345454545455 0.00307414120212182
676.033333333333 0.00299158633069828
687.721212121212 0.00291281284448452
699.409090909091 0.00283758289719994
711.09696969697 0.00276567744330329
722.784848484848 0.00269689446189836
734.472727272727 0.00263104737472965
746.160606060606 0.00256796363428964
757.848484848485 0.00250748346135188
769.536363636364 0.0024494587140404
781.224242424242 0.00239375187292789
792.912121212121 0.00234023512868846
804.6 0.00228878956057217
816.287878787879 0.00223930439546205
827.975757575758 0.00219167633855973
839.663636363636 0.0021458089678533
851.351515151515 0.00210161218547859
863.039393939394 0.00205900171991375
874.727272727273 0.00201789867366633
886.415151515152 0.00197822911173756
898.10303030303 0.0019399236866931
909.790909090909 0.00190291729664541
921.478787878788 0.00186714877286887
933.166666666667 0.00183256059413277
944.854545454545 0.00179909862515767
956.542424242424 0.00176671187688139
968.230303030303 0.00173535228646884
979.918181818182 0.00170497451521818
991.606060606061 0.00167553576270885
1003.29393939394 0.00164699559570789
1014.98181818182 0.00161931579050217
1026.6696969697 0.00159246018745879
1038.35757575758 0.00156639455673493
1050.04545454545 0.00154108647416516
1061.73333333333 0.00151650520644854
1073.42121212121 0.00149262160484289
1085.10909090909 0.00146940800664862
1096.79696969697 0.00144683814383269
1108.48484848485 0.00142488705820345
1120.17272727273 0.00140353102260178
1131.86060606061 0.00138274746762245
1143.54848484848 0.00136251491342395
1155.23636363636 0.00134281290622412
1166.92424242424 0.00132362195911479
1178.61212121212 0.00130492349686092
1190.3 0.00128669980437829
};
\addplot [very thick, cadetblue80178158]
table {%
76.3 0.254021695934473
86.9335353535353 0.189070243167694
97.5670707070707 0.147082741976569
108.200606060606 0.118380208365422
118.834141414141 0.0978786236185576
129.467676767677 0.082707980365506
140.101212121212 0.0711515421722366
150.734747474747 0.0621324288401403
161.368282828283 0.0549477627889855
172.001818181818 0.0491230656145149
182.635353535354 0.0443286463954712
193.268888888889 0.0403296021428423
203.902424242424 0.0369548502866972
214.53595959596 0.0340773511395284
225.169494949495 0.0316011304728359
235.80303030303 0.0294525569622233
246.436565656566 0.0275743520853685
257.070101010101 0.0259213961817364
267.703636363636 0.0244577402901696
278.337171717172 0.0231544430010647
288.970707070707 0.0219879816721092
299.604242424242 0.0209390698972942
310.237777777778 0.019991766533981
320.871313131313 0.0191327967963438
331.504848484848 0.018351029517681
342.138383838384 0.0176370707446106
352.771919191919 0.0169829449167549
363.405454545455 0.01638184264702
374.03898989899 0.0158279196172171
384.672525252525 0.015316135046197
395.306060606061 0.0148421210446537
405.939595959596 0.0144020762623263
416.573131313131 0.0139926787792882
427.206666666667 0.0136110143460044
437.840202020202 0.0132545169441074
448.473737373737 0.0129209192974312
459.107272727273 0.0126082114652565
469.740808080808 0.0123146060363415
480.374343434343 0.0120385087418659
491.007878787879 0.0117784935390195
501.641414141414 0.0115332814002681
512.27494949495 0.0113017221880035
522.908484848485 0.0110827791091197
533.54202020202 0.0108755153356854
544.175555555556 0.0106790824513835
554.809090909091 0.0104927104426196
565.442626262626 0.0103156990011723
576.076161616162 0.0101474099442727
586.709696969697 0.00998726058987628
597.343232323232 0.00983471795103361
607.976767676768 0.00968929363479997
618.610303030303 0.00955053934892336
629.243838383838 0.00941804293432142
639.877373737374 0.00929142485365381
650.510909090909 0.00917033507657444
661.144444444444 0.0090544503108589
671.77797979798 0.00894347153584715
682.411515151515 0.00883712180074975
693.045050505051 0.00873514425553515
703.678585858586 0.00863730038649969
714.312121212121 0.00854336843235311
724.945656565657 0.00845314195983363
735.579191919192 0.00836642858058877
746.212727272727 0.00828304879339075
756.846262626263 0.00820283493776099
767.479797979798 0.00812563024680578
778.113333333333 0.00805128798855589
788.746868686869 0.00797967068639538
799.380404040404 0.00791064941028233
810.013939393939 0.00784410313143854
820.647474747475 0.00777991813403127
831.28101010101 0.00771798747810964
841.914545454545 0.0076582105087048
852.548080808081 0.00760049240656769
863.181616161616 0.00754474377651613
873.815151515151 0.00749088026979829
884.448686868687 0.00743882223726437
895.082222222222 0.0073884944104771
905.715757575758 0.00733982560819105
916.349292929293 0.00729274846589551
926.982828282828 0.00724719918635057
937.616363636364 0.00720311730925442
948.249898989899 0.0071604454983648
958.883434343434 0.00711912934456251
969.51696969697 0.00707911718349212
980.150505050505 0.00704035992654543
990.78404040404 0.00700281090407107
1001.41757575758 0.00696642571979853
1012.05111111111 0.00693116211555832
1022.68464646465 0.00689697984546495
1033.31818181818 0.00686384055880496
1043.95171717172 0.00683170769094023
1054.58525252525 0.00680054636159839
1065.21878787879 0.00677032327997721
1075.85232323232 0.0067410066561404
1086.48585858586 0.00671256611822626
1097.11939393939 0.00668497263503261
1107.75292929293 0.00665819844357757
1118.38646464646 0.00663221698126962
1129.02 0.00660700282235067
};
\addplot [very thick, chocolate21910927]
table {%
32.92 1.00166326302187
43.7355555555556 0.559577770635859
54.5511111111111 0.36066445254605
65.3666666666667 0.253997527855577
76.1822222222222 0.18995224026526
86.9977777777778 0.148339720187751
97.8133333333333 0.119681660172264
108.628888888889 0.0990429998059504
119.444444444444 0.0836444473950061
130.26 0.071821271898463
141.075555555556 0.0625254945161317
151.891111111111 0.055069788595171
162.706666666667 0.0489875983334545
173.522222222222 0.0439528271912863
184.337777777778 0.0397317378762823
195.153333333333 0.0361530808335394
205.968888888889 0.0330889502378256
216.784444444444 0.0304421720759079
227.6 0.0281377906416013
238.415555555556 0.0261171956407321
249.231111111111 0.0243339914056251
260.046666666667 0.0227510401388389
270.862222222222 0.0213383116828145
281.677777777778 0.0200712970862116
292.493333333333 0.0189298225969955
303.308888888889 0.0178971522159435
314.124444444444 0.0169593009923643
324.94 0.0161045041370129
335.755555555556 0.0153228026621962
346.571111111111 0.0146057170922271
357.386666666667 0.0139459883945138
368.202222222222 0.01333737069021
379.017777777778 0.0127744641936877
389.833333333333 0.0122525796588369
400.648888888889 0.0117676276879809
411.464444444444 0.0113160278000031
422.28 0.0108946333071379
433.095555555556 0.0105006689197878
443.911111111111 0.010131678660371
454.726666666667 0.00978548217423891
465.542222222222 0.00946013791704615
476.357777777778 0.00915391200203744
487.173333333333 0.00886525172852699
497.988888888889 0.00859276299995627
508.804444444444 0.00833519098799644
519.62 0.00809140351700455
530.435555555556 0.00786037673741303
541.251111111111 0.00764118273243248
552.066666666667 0.00743297876368671
562.882222222222 0.00723499791110541
573.697777777778 0.00704654090292144
584.513333333333 0.00686696896479745
595.328888888889 0.00669569754437787
606.144444444444 0.00653219079007004
616.96 0.00637595668150165
627.775555555555 0.00622654272460204
638.591111111111 0.00608353213718522
649.406666666667 0.00594654046173656
660.222222222222 0.00581521255119419
671.037777777778 0.00568921988117297
681.853333333333 0.0055682581485477
692.668888888889 0.00545204512179451
703.484444444444 0.00534031871314685
714.3 0.00523283524659187
725.115555555555 0.0051293678991233
735.931111111111 0.00502970529557139
746.746666666667 0.00493365023982276
757.562222222222 0.0048410185673902
768.377777777778 0.00475163810614172
779.193333333333 0.00466534773360008
790.008888888889 0.00458199652060907
800.824444444444 0.00450144295236776
811.64 0.00442355421888079
822.455555555556 0.00434820556778578
833.271111111111 0.0042752797133171
844.086666666667 0.00420466629586256
854.902222222222 0.0041362613871819
865.717777777778 0.00406996703689324
876.533333333333 0.00400569085630672
887.348888888889 0.00394334563610095
898.164444444444 0.00388284899470599
908.98 0.00382412305458188
919.795555555555 0.00376709414386964
930.611111111111 0.00371169252114708
941.426666666667 0.00365785212124887
952.242222222222 0.00360551032031196
963.057777777778 0.00355460771838738
973.873333333333 0.0035050879381197
984.688888888889 0.00345689743813878
995.504444444444 0.00340998533993649
1006.32 0.00336430326711593
1017.13555555556 0.00331980519600336
1027.95111111111 0.00327644731670571
1038.76666666667 0.00323418790377934
1049.58222222222 0.00319298719575053
1060.39777777778 0.00315280728279542
1071.21333333333 0.00311361200194801
1082.02888888889 0.00307536683925953
1092.84444444444 0.00303803883838203
1103.66 0.00300159651509396
};
\addplot [very thick, purple11522131]
table {%
32.42 1.05677724037341
44.1365656565657 0.668513752931391
55.8531313131313 0.469458996839072
67.569696969697 0.35182191495937
79.2862626262626 0.275655992612596
91.0028282828283 0.223091407426074
102.719393939394 0.185060797619599
114.43595959596 0.156525670682277
126.152525252525 0.134486668484359
137.869090909091 0.117059030748985
149.585656565657 0.103005495259512
161.302222222222 0.091484031232672
173.018787878788 0.0819039674680375
184.735353535354 0.0738401270079655
196.451919191919 0.0669795709203322
208.168484848485 0.0610874578017021
219.88505050505 0.0559845206899121
231.601616161616 0.051531829685185
243.318181818182 0.0476202516597099
255.034747474747 0.044163013216596
266.751313131313 0.0410903591837475
278.467878787879 0.0383456542162346
290.184444444444 0.0358824959918045
301.90101010101 0.0336625490281195
313.617575757576 0.0316538994420467
325.334141414141 0.0298297914036956
337.050707070707 0.0281676467407872
348.767272727273 0.0266482970027206
360.483838383838 0.0252553766358688
372.200404040404 0.0239748395363796
383.91696969697 0.0227945709511825
395.633535353535 0.0217040736964108
407.350101010101 0.0206942127648463
419.066666666667 0.0197570061520764
430.783232323232 0.0188854525255537
442.499797979798 0.0180733884574352
454.216363636364 0.0173153695285179
465.932929292929 0.0166065708205283
477.649494949495 0.0159427032437655
489.366060606061 0.0153199428666164
501.082626262626 0.0147348709740403
512.799191919192 0.0141844230216654
524.515757575757 0.0136658449988713
536.232323232323 0.0131766559893312
547.948888888889 0.012714615936948
559.665454545454 0.0122776978011189
571.38202020202 0.0118640634271037
583.098585858586 0.0114720425721433
594.815151515151 0.0111001146214144
606.531717171717 0.0107468926042617
618.248282828283 0.0104111091837886
629.964848484848 0.0100916043444949
641.681414141414 0.00978731454532583
653.39797979798 0.00949726314091878
665.114545454545 0.00922055190333982
676.831111111111 0.00895635350126612
688.547676767677 0.00870390481425183
700.264242424242 0.0084625009771153
711.980808080808 0.00823149006416787
723.697373737374 0.00801026833543204
735.413939393939 0.00779827597754382
747.130505050505 0.00759499328101212
758.847070707071 0.00739993720316915
770.563636363636 0.00721265827270039
782.280202020202 0.00703273779726596
793.996767676767 0.00685978534055884
805.713333333333 0.00669343643931198
817.429898989899 0.00653335053436534
829.146464646464 0.00637920909301898
840.86303030303 0.00623071390260189
852.579595959596 0.00608758551753491
864.296161616161 0.00594956184421402
876.012727272727 0.00581639684982592
887.729292929293 0.00568785938277034
899.445858585858 0.00556373209373237
911.162424242424 0.00544381044764876
922.87898989899 0.00532790181786868
934.595555555555 0.00521582465473929
946.312121212121 0.00510740772166694
958.028686868687 0.00500248939243
969.745252525252 0.00490091700416046
981.461818181818 0.00480254626098063
993.178383838384 0.00470724068378551
1004.89494949495 0.00461487110211057
1016.61151515151 0.00452531518442372
1028.32808080808 0.00443845700353685
1040.04464646465 0.00435418663414945
1051.76121212121 0.004272399779822
1063.47777777778 0.00419299742692997
1075.19434343434 0.00411588552337834
1086.91090909091 0.00404097468005975
1098.62747474747 0.00396817989322451
1110.34404040404 0.00389742028609459
1122.06060606061 0.00382861886820348
1133.77717171717 0.00376170231107721
1145.49373737374 0.00369660073899338
1157.2103030303 0.00363324753366402
1168.92686868687 0.00357157915178716
1180.64343434343 0.00351153495450153
1192.36 0.00345305704785977
};
\addplot [very thick, saddlebrown1356716]
table {%
527.68 0.0260041994926554
534.415353535353 0.0234393082274716
541.150707070707 0.0211944857444265
547.886060606061 0.019223555962854
554.621414141414 0.0174877981760466
561.356767676768 0.0159546277008594
568.092121212121 0.0145965288816501
574.827474747475 0.0133901888113648
581.562828282828 0.0123157913474877
588.298181818182 0.0113564396463055
595.033535353535 0.0104976821331453
601.768888888889 0.00972712203142531
608.504242424242 0.00903409463736047
615.239595959596 0.00840939971297246
621.974949494949 0.00784507887710316
628.710303030303 0.00733422985457015
635.445656565656 0.00687085101381702
642.18101010101 0.00644971087281262
648.916363636364 0.00606623825063799
655.651717171717 0.00571642954152723
662.387070707071 0.00539677023070525
669.122424242424 0.00510416828960576
675.857777777778 0.00483589750730228
682.593131313131 0.00458954915524212
689.328484848485 0.00436299065930537
696.063838383838 0.00415433017930441
702.799191919192 0.00396188618112536
709.534545454545 0.00378416123866442
716.269898989899 0.00361981942780749
723.005252525252 0.00346766677794298
729.740606060606 0.00332663433194445
736.47595959596 0.00319576343644534
743.211313131313 0.0030741929431851
749.946666666667 0.00296114805136163
756.68202020202 0.00285593056199841
763.417373737374 0.00275791034975189
770.152727272727 0.00266651788646266
776.888080808081 0.0025812376750664
783.623434343434 0.00250160247297334
790.358787878788 0.00242718820134733
797.094141414141 0.00235760945137548
803.829494949495 0.00229251551106918
810.564848484848 0.00223158684671346
817.300202020202 0.00217453198209486
824.035555555555 0.00212108472632971
830.770909090909 0.00207100170769279
837.506262626263 0.00202406017647886
844.241616161616 0.00198005604476523
850.97696969697 0.00193880213510394
857.712323232323 0.00190012661374574
864.447676767677 0.00186387158709255
871.18303030303 0.00182989184273811
877.918383838384 0.00179805371877069
884.653737373737 0.00176823408701144
891.389090909091 0.00174031943759888
898.124444444444 0.00171420505384543
904.859797979798 0.00168979426760345
911.595151515151 0.00166699778653157
918.330505050505 0.00164573308564957
925.065858585859 0.00162592385645111
931.801212121212 0.00160749950761105
938.536565656566 0.00159039471199492
945.271919191919 0.00157454899527595
952.007272727273 0.00155990636197849
958.742626262626 0.00154641495523188
965.47797979798 0.00153402674691728
972.213333333333 0.00152269725525077
978.948686868687 0.00151238528715934
985.68404040404 0.00150305270308621
992.419393939394 0.00149466420210981
999.154747474747 0.00148718712547895
1005.8901010101 0.0014805912768628
1012.62545454545 0.00147484875778727
1019.36080808081 0.00146993381688262
1026.09616161616 0.00146582271170732
1032.83151515152 0.00146249358203221
1039.56686868687 0.00145992633358185
1046.30222222222 0.00145810253132497
1053.03757575758 0.00145700530149769
1059.77292929293 0.00145661924161574
1066.50828282828 0.00145693033780871
1073.24363636364 0.00145792588886789
1079.97898989899 0.00145959443645862
1086.71434343434 0.00146192570099795
1093.4496969697 0.00146491052274534
1100.18505050505 0.00146854080769414
1106.9204040404 0.00147280947789128
1113.65575757576 0.00147771042584462
1120.39111111111 0.00148323847270759
1127.12646464646 0.00148938932996037
1133.86181818182 0.00149615956433
1140.59717171717 0.0015035465657156
1147.33252525253 0.00151154851790431
1154.06787878788 0.00152016437188379
1160.80323232323 0.0015293938215731
1167.53858585859 0.00153923728180782
1174.27393939394 0.00154969586843379
1181.00929292929 0.00156077138037058
1187.74464646465 0.00157246628352311
1194.48 0.00158478369642584
};
\addplot [very thick, black18]
table {%
33.2 0.843163829701064
44.2191919191919 0.490680202090722
55.2383838383838 0.325060571787242
66.2575757575758 0.233433515830803
77.2767676767677 0.177099890012661
88.2959595959596 0.139809187721506
99.3151515151515 0.113737973793127
110.334343434343 0.0947281241920832
121.353535353535 0.0803971533163429
132.372727272727 0.06929686133524
143.391919191919 0.060503912792272
154.411111111111 0.0534059608484673
165.430303030303 0.0475832502871485
176.449494949495 0.0427398273356162
187.468686868687 0.0386618994805059
198.487878787879 0.0351917268747714
209.507070707071 0.0322107441261635
220.526262626263 0.0296283528864424
231.545454545455 0.027374301569559
242.564646464646 0.0253933936197818
253.583838383838 0.0236417426474237
264.60303030303 0.022084076693592
275.622222222222 0.0206917675005903
286.641414141414 0.0194413693954221
297.660606060606 0.0183135219845542
308.679797979798 0.0172921162878813
319.69898989899 0.0163636541384317
330.718181818182 0.0155167510845414
341.737373737374 0.0147417470385414
352.756565656566 0.0140303986660873
363.775757575758 0.0133756343866789
374.794949494949 0.012771357765158
385.814141414141 0.012212288618924
396.833333333333 0.0116938337527605
407.852525252525 0.0112119811402146
418.871717171717 0.0107632127894029
429.890909090909 0.0103444325961926
440.910101010101 0.0099529062938244
451.929292929293 0.00958621122295468
462.948484848485 0.00924219411863496
473.967676767677 0.00891893547643028
484.986868686869 0.00861471934475473
496.006060606061 0.00832800761383189
507.025252525252 0.00805741804782009
518.044444444444 0.00780170544634696
529.063636363636 0.00755974543311381
540.082828282828 0.00733052045854711
551.10202020202 0.00711310767543328
562.121212121212 0.00690666840471987
573.140404040404 0.00671043895603284
584.159595959596 0.00652372260614133
595.178787878788 0.00634588257032673
606.19797979798 0.00617633582773489
617.217171717172 0.00601454768338216
628.236363636364 0.00586002696739984
639.255555555556 0.00571232178701604
650.274747474748 0.0055710157592348
661.293939393939 0.00543572466261674
672.313131313131 0.00530609345534793
683.332323232323 0.00518179361419213
694.351515151515 0.00506252075518754
705.370707070707 0.00494799250226652
716.389898989899 0.00483794657449974
727.409090909091 0.0047321390665242
738.428282828283 0.00463034290001494
749.447474747475 0.00453234642688868
760.466666666667 0.00443795216735977
771.485858585859 0.00434697566806307
782.50505050505 0.00425924446726738
793.524242424242 0.004174597155768
804.543434343434 0.00409288252340425
815.562626262626 0.00401395878232786
826.581818181818 0.00393769285917441
837.60101010101 0.00386395974918698
848.620202020202 0.00379264192612438
859.639393939394 0.00372362880247209
870.658585858586 0.00365681623507649
881.677777777778 0.00359210607185206
892.69696969697 0.00352940573567658
903.716161616162 0.00346862784200099
914.735353535354 0.00340968984706264
925.754545454545 0.0033525137239126
936.773737373737 0.00329702566375141
947.792929292929 0.00324315580032091
958.812121212121 0.00319083795532348
969.831313131313 0.00314000940304046
980.850505050505 0.00309061065249895
991.869696969697 0.00304258524569544
1002.88888888889 0.00299587957052665
1013.90808080808 0.00295044268720475
1024.92727272727 0.00290622616704856
1035.94646464646 0.00286318394264376
1046.96565656566 0.00282127216845753
1057.98484848485 0.00278044909107502
1069.00404040404 0.00274067492829976
1080.02323232323 0.00270191175642669
1091.04242424242 0.00266412340505722
1102.06161616162 0.00262727535888017
1113.08080808081 0.00259133466589167
1124.1 0.00255626985157207
};
\addplot [very thick, darkgray153]
table {%
33.2 1.25722136489288
44.9555555555556 0.624409113982235
56.7111111111111 0.371189684858908
68.4666666666667 0.245990706740083
80.2222222222222 0.17528261964652
91.9777777777778 0.131525405233192
103.733333333333 0.102578215706889
115.488888888889 0.0824303406122854
127.244444444444 0.0678352140065459
139 0.0569160936938179
150.755555555556 0.0485273787295694
162.511111111111 0.0419378249331872
174.266666666667 0.0366629267564573
186.022222222222 0.0323713396557991
197.777777777778 0.0288302193419009
209.533333333333 0.0258720329760892
221.288888888889 0.0233737209889455
233.044444444444 0.0212432245058849
244.8 0.0194105469191878
256.555555555556 0.0178216859447074
268.311111111111 0.0164344288687331
280.066666666667 0.0152153845375203
291.822222222222 0.0141378530040742
303.577777777778 0.0131802730019548
315.333333333333 0.0123250747073168
327.088888888889 0.0115578211342364
338.844444444444 0.0108665579805571
350.6 0.0102413159688034
362.355555555555 0.00967372608380784
374.111111111111 0.00915671931922782
385.866666666667 0.00868429033597049
397.622222222222 0.00825130992025722
409.377777777778 0.00785337503701463
421.133333333333 0.00748668809024264
432.888888888889 0.00714795905256809
444.644444444444 0.00683432563420238
456.4 0.00654328778086155
468.155555555556 0.00627265362834412
479.911111111111 0.00602049467422914
491.666666666667 0.00578510840861186
503.422222222222 0.00556498701482631
515.177777777778 0.00535879103594934
526.933333333333 0.00516532712420407
538.688888888889 0.00498352916343626
550.444444444444 0.00481244219096363
562.2 0.00465120865279062
573.955555555556 0.0044990566118424
585.711111111111 0.00435528959736613
597.466666666667 0.00421927783868682
609.222222222222 0.00409045067094377
620.977777777778 0.00396828993647753
632.733333333333 0.00385232423489946
644.488888888889 0.0037421238988963
656.244444444444 0.00363729659255159
668 0.00353748344523218
679.755555555556 0.00344235564755217
691.511111111111 0.00335161144710804
703.266666666667 0.00326497349099822
715.022222222222 0.00318218646993427
726.777777777778 0.00310301502528784
738.533333333333 0.00302724188591959
750.288888888889 0.00295466620627975
762.044444444444 0.00288510208119977
773.8 0.00281837721613184
785.555555555556 0.00275433173443156
797.311111111111 0.0026928171057028
809.066666666667 0.00263369518129666
820.822222222222 0.00257683732483399
832.577777777778 0.00252212362714953
844.333333333333 0.00246944219637239
856.088888888889 0.00241868851499473
867.844444444444 0.00236976485676459
879.6 0.00232257975709252
891.355555555555 0.00227704753140297
903.111111111111 0.00223308783650768
914.866666666667 0.00219062527064164
926.622222222222 0.00214958900829445
938.377777777778 0.00210991246640178
950.133333333333 0.00207153299883951
961.888888888889 0.00203439161649586
973.644444444444 0.00199843273048958
985.4 0.00196360391636019
997.155555555556 0.00192985569728428
1008.91111111111 0.00189714134457352
1020.66666666667 0.00186541669388848
1032.42222222222 0.00183463997576101
1044.17777777778 0.00180477165915855
1055.93333333333 0.00177577430694908
1067.68888888889 0.00174761244223701
1079.44444444444 0.00172025242463986
1091.2 0.00169366233566457
1102.95555555556 0.00166781187242189
1114.71111111111 0.00164267224898848
1126.46666666667 0.00161821610479028
1138.22222222222 0.00159441741943815
1149.97777777778 0.00157125143349852
1161.73333333333 0.00154869457472765
1173.48888888889 0.00152672438934071
1185.24444444444 0.00150531947792401
1197 0.00148445943563297
};
\addplot [draw=black, fill=black, mark=x, very thick, mark size=2.5pt, only marks]
table{%
x  y
131.28 0.167918891881762
527.68 0.0273828282351949
};


==> figures/quantitative_results/group_laplace_2.tex <==
\nextgroupplot[
ylabel shift = -0.2cm,
clip marker paths=true,
width=0.52\textwidth,
height=4.5cm,
title style={yshift=-0.2cm},
scaled x ticks=false,
xlabel style={yshift=0.1cm},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
title={Laplace's Equation - $6$ Refinements},
x grid style={darkgray176},
xlabel={Elements \(\displaystyle (\times 10^3)\)},
xmajorgrids,
xmin=-403.628, xmax=9206.588,
xtick style={color=black},
xtick={-2000,0,2000,4000,6000,8000,10000},
xticklabels={-2.0,0.0,2.0,4.0,6.0,8.0,10.0},
y grid style={darkgray176},
ylabel={\empty},
ymajorgrids,
ymin=1.43078625778226e-05, ymax=1.8415257818879,
ymode=log,
ytick style={color=black},
ytick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
}
% yticklabels=\empty,
]
\addplot [
  draw=royalblue28108204,
  fill=royalblue28108204,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
33.2 0.99999999980788
66.02 0.192025637079874
66.24 0.187754282622464
66.34 0.210435561772441
66.58 0.19890936695577
67.94 0.193531390033193
69.3 0.174770133837383
71.78 0.174365695494093
72.38 0.156949629591999
75.9 0.148918296502688
102.28 0.0983805572546707
119.54 0.0537816766034118
121.14 0.0459877371057981
126.16 0.0536801714025099
126.2 0.0660026589615362
132.22 0.0624297627197812
134.28 0.0599914039330322
136.88 0.0508885976010886
137.02 0.0477467752453722
139.1 0.0533310750783739
272.68 0.011161218156936
273.52 0.0111538292919025
293.74 0.0101423591666926
300.16 0.0112677465297255
300.4 0.0101433712368608
315.74 0.00917324202806342
343.36 0.00898039284460785
344.16 0.00780840545152171
345.66 0.0141429613906773
350.14 0.00931732162255995
350.94 0.0082821778200329
352.32 0.00738795269938686
388.5 0.00788040987157702
417.08 0.00644228100736605
427.84 0.00435113419832459
432.62 0.00741348157269585
446.48 0.00419211075954711
475.26 0.0055602980129416
525.5 0.00402110613752549
561 0.00415045532386424
586.34 0.00275212195688654
630.76 0.00279821751589418
633.38 0.00268855856423296
673.04 0.00280461263989624
687.12 0.00212741068296248
717.06 0.00227717171517922
776.66 0.00302452928241457
843.66 0.00180818039911108
933.94 0.00138855683299744
947.24 0.0011055181722984
1031.8 0.00134497991469994
1046.54 0.00133999721172291
1064.5 0.00105608379550473
1075.58 0.00106518142567715
1118.48 0.00110406463422299
1183.62 0.00114555677074573
1209.7 0.00104698097732296
1319.3 0.000622062873310763
1336.02 0.00108585681607456
1371.98 0.00107372383261761
1470.32 0.000970685989659171
1494.08 0.000593824432742029
1526.78 0.000760801816138272
1550.16 0.000775750897001304
1693.82 0.000704098849461141
1753.9 0.000592311284693081
1902.06 0.000555353983147898
1904.44 0.000540381800416667
1959.86 0.000551058094436498
2065.42 0.000448142978175028
2261.5 0.000277298372416601
2315.22 0.000465590189956223
2518.24 0.000245160825041142
2931.22 0.000218117485457911
3205.54 0.000178053359067072
3272.3 0.00014862340264744
3272.86 0.000162934804105929
3308.72 0.000212898311291264
3547.52 0.000143698849065868
3655.94 0.000126556279295253
3680.06 0.000151626994456722
3810.74 0.000148219231124926
3814.18 0.000121086738241704
3817.28 0.000133130536623686
4035.54 0.000135588923101501
4386.66 0.000130928531879776
4422.52 8.44822797284713e-05
4471.24 7.98373936580992e-05
4568.14 0.000111884502868355
4857.4 0.000127122847411118
5186.26 0.000115801642998642
5293.92 7.93398419333758e-05
6125.68 6.84487990434793e-05
6855.8 3.76676098626857e-05
7024.44 0.000111786638922668
7131.68 4.35655309200817e-05
7333.12 4.83932172488927e-05
7426.32 2.98619298101207e-05
7825.86 3.49159036300333e-05
8423.68 4.19108357379708e-05
};
\addplot [
  draw=cadetblue80178158,
  fill=cadetblue80178158,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
269.42 0.0272303318541551
272.38 0.0215977137330373
279.24 0.0162516717808451
283.26 0.0191443230460429
283.78 0.0193749293424317
287.46 0.0189385326891545
299.02 0.0243064973287749
305.88 0.028637757436734
308.56 0.0175920101292412
333.44 0.0159009466220338
472.92 0.00556119277744241
475.62 0.00529001285822559
510.74 0.0106270855010055
516.46 0.0204597195890836
520.4 0.00848185116164715
527.84 0.0108032058997219
535.68 0.00672643832235808
539.52 0.00582425314479223
550.58 0.00951400954749761
604.32 0.00613558297446528
677.74 0.0071844851773329
709.78 0.00762817321203376
726.3 0.00728491513844455
741.84 0.00927074952933055
751.08 0.00513134021424232
751.32 0.0148440487197465
768.36 0.399235053639226
807.48 0.0108265620792889
835.86 0.00979563012887476
856.3 0.0157451875434538
878.68 0.00546548489378337
885.34 0.0133596159845129
892.46 0.00962885303338184
907 0.00286763780992378
911.56 0.0128261695193435
913.28 0.00918311750268795
943.22 0.00251651347817735
961.66 0.0042055788663924
984.84 0.0104601463159832
1005.62 0.0110199942008356
1030.16 0.0105451279233217
1032.48 0.0105415645295325
1129.02 0.00291537514140832
1194.64 0.0030083418913392
1301.06 0.000821145131500648
1319.74 0.00087372153719304
1326.48 0.000757102659530126
1342.08 0.00190064515224483
1358.36 0.00727073468576773
1374.68 0.0107968538773586
1428.36 0.00733887818749248
1457.72 0.00355723291054542
1582.06 0.000435075356426895
1622.14 0.00278285560894437
1636.9 0.000688007119504234
1639.38 0.0024956653002775
1682.46 0.000467651039965788
1691.6 0.000896256575790227
1730.22 0.000646993220251929
1774.68 0.000874644716232583
1864.78 0.00199090507420633
1874.54 0.00241588823937115
1903.54 0.00732549731349817
1946.16 0.000957310755094496
2086.72 0.00615858923618284
2098.16 0.000856531532816897
2099.64 0.0544660230362162
2237.4 0.0186654952067104
2285.38 0.000959967370578621
2286.5 0.000795896897355156
2315.1 0.000393032138933562
2353.48 0.0002323076580011
2375.16 0.000217412904975599
2392.72 0.00617290064542923
2397.5 0.00107175938948574
2480.48 0.00040359613024162
2515.02 0.000924245639864907
2521.6 0.000282029134376849
2531.28 0.000162759191820814
2572.06 0.000310029979511982
2672.4 0.00142967923942809
2695.72 0.0244510099678341
2719.22 0.000210597375113824
2744.38 0.0068890684019686
2774.84 0.00127180875147284
2823.2 0.00108819772552587
2823.48 0.00556497129007377
2831.74 0.000194570165127203
2851.66 0.00153526229473184
2907.04 0.01241965731928
2925.94 0.000225162155015772
2966.28 0.000413352286956212
3228.08 0.000182922738215535
3275.86 0.00382832241408514
3296.52 0.00157554295936538
3365.2 0.000723874269730266
3392.46 0.000165649797824695
3405.36 0.00240339462080803
3510.92 0.000177093105564597
3699.98 0.000736475592561294
};
\addplot [
  draw=chocolate21910927,
  fill=chocolate21910927,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.2 0.99999999980788
33.58 0.986498106376962
50.62 0.682281746399152
56.32 0.675091619736275
65.62 0.260249346477582
115.6 0.0757925855534126
126.66 0.0599798317786378
127.42 0.17045487058599
131.28 0.167918891881757
140.88 0.0662508888619228
168.36 0.0745746899730482
174.34 0.03083485026722
175.84 0.0337750553683708
176.54 0.0324122972998927
189.32 0.0325943411088236
205.26 0.0249483838815312
206.98 0.0383061222154387
207.6 0.0350564665820563
214.7 0.0407980243371618
259 0.0203575342918624
295.04 0.0179067695748342
329 0.0116013971916544
333.68 0.00898421134448436
355.68 0.026039290880154
371.28 0.0105667822235345
401.22 0.00737634999987988
416.64 0.0077376532598953
490.34 0.00463666241079894
529.3 0.00480549858795774
555.78 0.0157089781434893
588.7 0.00315125994010182
612.78 0.0173071746476804
655.98 0.00469471975617978
661.22 0.0099398529423857
680.34 0.00663291466693789
684.66 0.0038635896322651
811.92 0.00376090448845621
934.88 0.0048069515628215
962.54 0.001762126006636
1073.08 0.00158105158402724
1079.06 0.00129678815179724
1269.02 0.00246545078917409
1353.4 0.00140971893687057
1579.76 0.00102881055503182
2627.12 0.000524752517792176
3084.36 0.00371071374144733
4614.22 0.767177231940209
4842.3 0.006650704597917
8769.76 5.0938774467089e-05
};
\addplot [draw=purple11522131, fill=purple11522131, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
108.08 0.18518751559111
123.2 0.102497766778339
154.8 0.0774324679854691
174.88 0.0460775276240287
176.84 0.0503502665916493
179.44 0.0397825157224299
189.12 0.0412902252577953
194.12 0.0341570652607007
210.56 0.0685941150462297
219.84 0.0280073437356045
281.78 0.0274521787672049
303.1 0.0253143258938404
304.94 0.0224097632744356
325.68 0.0258068415587312
332.4 0.0251604832248979
344.9 0.025045960282952
350.12 0.0261480927027984
350.68 0.0254388591828299
354.12 0.0252242285708618
391.34 0.0234765480191671
394.14 0.0168973787130159
428.78 0.0219485277900936
436.52 0.0262508997212733
441.98 0.0219754757537947
462.58 0.0266585369095283
465.1 0.0266736377380999
472.16 0.0267677033051448
479.82 0.0268913483855246
489.12 0.0269728868955202
490.42 0.0270106495864003
502.86 0.0268173448135813
511.14 0.0186048679904556
517.32 0.0273227513032658
519.14 0.027313509898968
523.6 0.0273625966651678
534.34 0.0252183399445867
540.98 0.00558923008230333
550.3 0.00659625782316353
568.38 0.00565130509576207
675.78 0.00522437973590881
860.2 0.00527895290394453
905.84 0.00546349938788228
916.2 0.00422820972736008
950.76 0.00405083939721978
1078.88 0.00387161460864726
1099.72 0.00416131266154231
1112.96 0.003896734728369
1192.36 0.00388957820975332
1285.16 0.00386028512044188
1377.8 0.00387330505245377
1402.48 0.00386011021484851
1479.5 0.00386288106812439
1646.84 0.00396190490260269
1762.24 0.00398192253631001
1951.96 0.00406715784330481
2065.98 0.00410984891040232
2067.36 0.0041110975384706
2076.52 0.00411202809827759
2082.06 0.00411445858406589
2107.88 0.00412081322700426
2115.4 0.00412206706974933
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2115.84 0.004122119539775
2157 0.00365007172631006
2305 0.00344520529533483
2332.08 0.00344078759201267
2375.34 0.00343765993267126
2481.1 0.00343350163787332
2511.8 0.00344590632265012
2635.98 0.00343525995903315
2648.94 0.00343520244232403
2742.98 0.00343681275090956
3083.52 0.00344180245328454
5618.06 0.0005037858593648
6834.3 0.000516901818534272
7002.16 0.000515591440067443
7542.02 0.000522291251523498
7574.38 0.000523409529473858
8041.18 0.000527716795948202
8098.4 0.000528420512048933
8231.82 0.000529301873221877
8334.2 0.000529992695438445
8392.78 0.000528705722443463
8437.1 0.000530969995588356
8497.34 0.000529385802937412
8519.06 0.000529477618295145
8519.6 0.000529479621339149
8519.68 0.000529479923316743
8519.68 0.000529479923316743
8519.68 0.000529479923316743
8519.68 0.000529479923316743
8519.68 0.000529479923316743
8519.68 0.000529479923316743
};
\addplot [draw=black18, fill=black18, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
33.2 0.99999999980788
88.64 0.125680514672274
91.5 0.118294262199929
94.52 0.111360533595086
96.14 0.106725353512633
98.58 0.103119734353714
103.06 0.0920270701419962
107.84 0.0874382667995979
110.34 0.0840578690433487
112.06 0.0819063628396549
118.72 0.0785058909350878
123.06 0.0736022837033418
126.68 0.0716836417845779
132 0.0657451723540767
137.76 0.0596782675018436
143.64 0.0580679255124789
148.12 0.0568209200976028
149.28 0.0526566573695782
157.18 0.0496354851374305
162.14 0.0470269741864306
164.1 0.0438324322706926
170.88 0.0413667246160725
176.26 0.0385935532408533
182.98 0.0379612184616221
199.44 0.0353126414974565
210.28 0.0338979511184986
210.56 0.0307214649916558
216.26 0.0324239075815054
223.9 0.0291543299857388
234.9 0.0263132213236466
252.38 0.0242364800578708
253.54 0.0234394801400863
269.76 0.0217295758753702
295.34 0.0188660611016614
315.38 0.0170380613173319
323.94 0.0156358975792213
349.56 0.0141192405041145
369.5 0.0133969285389175
379.18 0.0129387256311939
391.08 0.0115800204372365
422.64 0.0104787364157876
452.8 0.00908554928035431
483.5 0.00848009143201333
503.88 0.00785317559500864
524.46 0.00711380402426492
543.74 0.00688002782970892
583.8 0.00636286481067349
625.26 0.00556262283644963
704.3 0.00479801712792097
752.2 0.0043239983636887
830.9 0.00369470870841305
882.84 0.00336664641022855
958.26 0.0026425836094685
1040.58 0.00221633114560798
1139.82 0.0020212746511361
1168.78 0.00185958163003969
1274.98 0.00160563027220137
1301.2 0.00151671914290485
1337.14 0.00141699625112001
1523.42 0.00122831643281512
1589.8 0.00112993357859804
1650.66 0.00103339348943775
1851.22 0.000943236337688224
1994.92 0.000785700984363763
2179.2 0.00063560474806975
2446.28 0.000514306079466475
2776.76 0.000418512089981816
3092.5 0.000313564585174223
3420.78 0.000253979759546727
3775.1 0.00021457201042522
4148.94 0.000182220756669369
4470.86 0.000155751796096679
4913.06 0.000135441441948871
5517.64 0.000118252766499964
5943.22 0.00010331229779313
6927.74 7.68401464396048e-05
7143.36 6.27320236485976e-05
7962.72 4.37678671503627e-05
8616.48 3.2389924011099e-05
8716.1 2.44247115793406e-05
};
\addplot [draw=darkgray153, fill=darkgray153, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
33.2 0.99999999980788
129.4 0.0663281242132411
139.2 0.0566783999327457
148.18 0.0501549279619793
155.2 0.0441955515673794
161.38 0.0392396284506437
168.56 0.0351177233288931
179.26 0.0321632096462975
191.44 0.0291922080094791
201.88 0.0257129433131064
206.96 0.0240616856890378
218.36 0.0218814264953215
226.78 0.0198738962060499
229.76 0.0184886227864552
232.54 0.017544629040791
244.06 0.016193163281883
260.1 0.0142550263792862
263.02 0.0146585639771191
277.7 0.0132314445219726
286.62 0.0128183124434369
311.52 0.0112347877970438
337.06 0.0100424655489091
358.56 0.00930911803076962
384.74 0.00833310934763894
411.74 0.00740380051317467
434.24 0.00668148393974867
473.96 0.00581582300610365
489.64 0.0054622039348092
511.24 0.00496781588083645
549.3 0.00432248035679294
571.22 0.00397733024891469
600.76 0.00366081269663052
644.68 0.00314347686101439
679.28 0.00277426317852751
727.52 0.00246320396526854
763.9 0.00226388146708856
792.4 0.00204724285517656
840.4 0.00185838446822926
892.58 0.00167499908885197
938.66 0.00150921862985876
969.56 0.00143536182088382
997.08 0.00133426478323686
1025.14 0.00125017132307145
1083.2 0.00115757292955204
1119.96 0.00107197414723644
1188.78 0.00097133126559016
1258.76 0.000884083732685383
1315.62 0.000823211456522832
1351.16 0.000779399062224193
1427.22 0.00071010925815554
1483.22 0.000644856299500747
1559.1 0.000577119616828608
1680.32 0.000523937243395019
1758.1 0.000487938981647013
1869.94 0.000425897871398799
1968.86 0.000398613710393876
2156.5 0.000331300006357371
2218.68 0.000300320933854168
2335.16 0.000265943117656326
2493.12 0.000243444576195654
2668.88 0.000214437519480435
2749.74 0.000198732077728896
2895.32 0.000180336586558322
3095.52 0.000163083416125375
3145.64 0.000150268322679534
3226.58 0.000138449235220512
3375.7 0.00012845683396457
3419.42 0.000124904952310855
3579.84 0.000115878576227366
3777.72 0.000105968070232127
3839.36 9.93527801593471e-05
4041.1 9.21067240017025e-05
4150.14 8.5301722042584e-05
4337.78 7.92564470426533e-05
4583.82 7.34049707574555e-05
4805.1 6.86511449157824e-05
4956.18 6.38726170725381e-05
5127.32 5.7792532904222e-05
5510.74 5.2676888299253e-05
5852.06 4.82860546394672e-05
6142.76 4.42147392224028e-05
6334.84 4.03107117241403e-05
6647.74 3.66677932965414e-05
7205.82 3.22586835150764e-05
7893.16 2.89882924813232e-05
8463.52 2.53774238230858e-05
};
\addplot [
  draw=saddlebrown1356716,
  fill=saddlebrown1356716,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
527.68 0.0273828282351928
569.04 0.0199753675805781
574.56 0.0193445985921392
576.08 0.0183108132331301
590.6 0.0170635213386491
602.04 0.0161620487963937
608.54 0.0151330230000694
616.12 0.0143377556551488
629.26 0.0130438182244757
643.48 0.0120297859015205
654.84 0.0110116194089781
678.48 0.00976533288336428
689.02 0.0089616184302245
703.04 0.00779980103326453
720.9 0.0068746226689987
743.62 0.00610954759813924
759.36 0.00550384065749145
783.9 0.00464253909931192
798.18 0.00414367441703194
824.56 0.00355503694376715
840.32 0.00311984186438066
853.48 0.00281393826809092
862.22 0.00262692989228494
885.12 0.00234462497129731
891.1 0.0022573682454946
902.26 0.00219156235310356
905.36 0.00214690793112011
914.22 0.00208910205241493
933.5 0.00203147357766722
940.42 0.00195271439957186
949.64 0.00189154680796149
952.64 0.00192717789984529
952.94 0.0018431676239087
954.02 0.00181984277340927
954.18 0.00179527415138289
960.34 0.00175433703722455
974.02 0.0017317526925832
979.9 0.00170150789158333
980.98 0.00166219851266311
984.82 0.00164405381554371
999.96 0.00159763046704373
1005.26 0.00158021337088693
1009.58 0.0015475674799449
1024.88 0.00151005050902187
1035.7 0.00148170690318046
1045.2 0.00144642036352346
1062.5 0.0013996010197035
1078.92 0.00136091606576115
1100.72 0.00132778661223378
1118.92 0.00129277604864663
1143.92 0.00125003438126067
1156.06 0.00121767429240028
1175.78 0.00117457556551981
1205.62 0.0011313488597606
1236.42 0.00108199808881586
1265.92 0.00103719523095472
1284.06 0.000992266723013719
1319.92 0.000953940507862098
1367.14 0.000910686757892115
1402.14 0.000872262503476731
1437.8 0.000833456478963398
1491.44 0.000792053016387579
1535.8 0.000756815336331547
1580.74 0.000716944822533076
1624.26 0.000678480139615166
1664.84 0.000640771035573084
1730.76 0.00059965265484273
1778.42 0.000567015550602318
1826.36 0.000534130214250673
1881.14 0.000495397707276826
1943.78 0.000465283201470044
2007.64 0.000435880364332287
2065.48 0.000404829282760783
2133.9 0.000381166788164811
2222.62 0.000363067100951838
2299.1 0.000343391720442722
2372.88 0.000322819723853552
2446.28 0.000301986947901375
2530.12 0.000281866215234887
2608.84 0.000262432641638972
2697.74 0.000244036064151947
2797.08 0.000227696753112263
2897.66 0.000212516710698387
3017.7 0.000197837492563389
3154.22 0.000185012614318678
3237.48 0.000174132702389207
3340.72 0.000162546041551502
3468.06 0.00015265517937529
3572.14 0.000142956185569058
3705.6 0.000133354987791289
3831.06 0.000124355895948581
3988.26 0.000115787541170214
4133.62 0.000108977971256893
4298.6 0.000102360103224335
4458.02 9.40387220539506e-05
4636.2 8.73559796548526e-05
4827.7 8.14495023531128e-05
4969.98 7.54127862375705e-05
5132.58 7.10074220920435e-05
5332.26 6.67416023325312e-05
};
\addplot [very thick, royalblue28108204]
table {%
33.2 0.768307097410559
117.952323232323 0.0655528152284666
202.704646464646 0.0237580354800053
287.45696969697 0.0124870260072905
372.209292929293 0.00780479568951742
456.961616161616 0.005393249821569
541.713939393939 0.0039788439505589
626.466262626263 0.00307356538761968
711.218585858586 0.00245658649843563
795.970909090909 0.00201569378480701
880.723232323232 0.00168875235646584
965.475555555556 0.0014389980199516
1050.22787878788 0.00124349815308843
1134.9802020202 0.00108731790179615
1219.73252525253 0.00096037584993323
1304.48484848485 0.000855657343651045
1389.23717171717 0.000768153191003962
1473.9894949495 0.000694204927217097
1558.74181818182 0.000631087485766523
1643.49414141414 0.000576735504044905
1728.24646464646 0.000529559269503291
1812.99878787879 0.000488318162452493
1897.75111111111 0.000452031887137082
1982.50343434343 0.00041991708560997
2067.25575757576 0.000391341339586739
2152.00808080808 0.000365789297238136
2236.7604040404 0.000342837392778069
2321.51272727273 0.000322134746334975
2406.26505050505 0.000303388569615963
2491.01737373737 0.000286352897831766
2575.7696969697 0.000270819805615981
2660.52202020202 0.000256612497881441
2745.27434343434 0.000243579830019528
2830.02666666667 0.000231591927878086
2914.77898989899 0.000220536661287407
2999.53131313131 0.000210316785414579
3084.28363636364 0.000200847608617949
3169.03595959596 0.000192055078354265
3253.78828282828 0.000183874201267038
3338.54060606061 0.00017624773211028
3423.29292929293 0.000169125080239046
3508.04525252525 0.000162461393176722
3592.79757575758 0.000156216785081031
3677.5498989899 0.000150355684384541
3762.30222222222 0.000144846279928749
3847.05454545455 0.000139660048876204
3931.80686868687 0.000134771352821145
4016.55919191919 0.000130157091013117
4101.31151515151 0.000125796401601892
4186.06383838384 0.000121670403414206
4270.81616161616 0.000117761972066444
4355.56848484849 0.000114055545266822
4440.32080808081 0.000110536953015544
4525.07313131313 0.000107193269111094
4609.82545454545 0.000104012680945548
4694.57777777778 0.000100984375045899
4779.3301010101 9.80984362108636e-05
4864.08242424242 9.53457584188115e-05
4948.83474747475 9.27179659543232e-05
5033.58707070707 9.02073434284324e-05
5118.33939393939 8.78067735585278e-05
5203.09171717172 8.55096817346325e-05
5287.84404040404 8.33099865345633e-05
5372.59636363636 8.120205546542e-05
5457.34868686869 7.91806653065108e-05
5542.10101010101 7.72409665119793e-05
5626.85333333333 7.53784512023894e-05
5711.60565656566 7.35889243353207e-05
5796.35797979798 7.1868477697163e-05
5881.1103030303 7.02134664031782e-05
5965.86262626263 6.86204876315655e-05
6050.61494949495 6.70863613506964e-05
6135.36727272727 6.56081128276234e-05
6220.1195959596 6.41829567310824e-05
6304.87191919192 6.28082826640573e-05
6389.62424242424 6.14816419799963e-05
6474.37656565657 6.02007357533893e-05
6559.12888888889 5.89634037899443e-05
6643.88121212121 5.77676145743382e-05
6728.63353535354 5.66114560646842e-05
6813.38585858586 5.54931272527004e-05
6898.13818181818 5.44109304172108e-05
6982.89050505051 5.33632640062502e-05
7067.64282828283 5.23486160898011e-05
7152.39515151515 5.13655583311511e-05
7237.14747474747 5.04127404301689e-05
7321.8997979798 4.94888849964903e-05
7406.65212121212 4.85927828147826e-05
7491.40444444444 4.77232884679838e-05
7576.15676767677 4.68793162877262e-05
7660.90909090909 4.60598366041122e-05
7745.66141414141 4.52638722696653e-05
7830.41373737374 4.44904954346371e-05
7915.16606060606 4.37388245529875e-05
7999.91838383838 4.30080216002485e-05
8084.67070707071 4.22972894862029e-05
8169.42303030303 4.16058696468396e-05
8254.17535353535 4.09330398014434e-05
8338.92767676768 4.02781118619177e-05
8423.68 3.96404299825716e-05
};
\addplot [very thick, cadetblue80178158]
table {%
269.42 0.021587955660092
304.072121212121 0.019633774770367
338.724242424242 0.0179281538480511
373.376363636364 0.0164330858989763
408.028484848485 0.0151163639029582
442.680606060606 0.013951152465122
477.332727272727 0.0129152119339617
511.984848484848 0.0119901097216724
546.63696969697 0.0111605254227838
581.289090909091 0.0104136718306225
615.941212121212 0.009738824224911
650.593333333333 0.00912694167901297
685.245454545455 0.00857036342621435
719.897575757576 0.0080625652944435
754.549696969697 0.0075979638137263
789.201818181818 0.00717175806075933
823.853939393939 0.00677980139541884
858.506060606061 0.00641849693551166
893.158181818182 0.0060847119521194
927.810303030303 0.00577570741067552
962.462424242424 0.00548907969255889
997.114545454545 0.00522271215976291
1031.76666666667 0.00497473471245299
1066.41878787879 0.00474348986835035
1101.07090909091 0.00452750418887459
1135.72303030303 0.00432546410898599
1170.37515151515 0.00413619541030559
1205.02727272727 0.00395864572150755
1239.67939393939 0.0037918695446938
1274.33151515152 0.00363501539800085
1308.98363636364 0.00348731473806553
1343.63575757576 0.00334807238505752
1378.28787878788 0.00321665822076374
1412.94 0.00309249996901174
1447.59212121212 0.00297507689936121
1482.24424242424 0.00286391432090168
1516.89636363636 0.00275857875428982
1551.54848484848 0.00265867368773128
1586.20060606061 0.002563835837162
1620.85272727273 0.00247373184297647
1655.50484848485 0.00238805534573318
1690.15696969697 0.00230652439170411
1724.80909090909 0.00222887912621532
1759.46121212121 0.00215487973868731
1794.11333333333 0.00208430462831772
1828.76545454545 0.00201694876361233
1863.41757575758 0.001952622212591
1898.0696969697 0.00189114882357856
1932.72181818182 0.00183236503912311
1967.37393939394 0.00177611882783806
2002.02606060606 0.00172226872089767
2036.67818181818 0.00167068294157925
2071.3303030303 0.00162123861767966
2105.98242424242 0.00157382106787227
2140.63454545455 0.00152832315414439
2175.28666666667 0.001484644693386
2209.93878787879 0.00144269192201076
2244.59090909091 0.00140237700819573
2279.24303030303 0.00136361760694261
2313.89515151515 0.00132633645370211
2348.54727272727 0.00129046099277515
2383.19939393939 0.00125592303711942
2417.85151515151 0.00122265845655432
2452.50363636364 0.00119060689167838
2487.15575757576 0.00115971149109673
2521.80787878788 0.00112991866980655
2556.46 0.00110117788681025
2591.11212121212 0.00107344144022236
2625.76424242424 0.00104666427831089
2660.41636363636 0.00102080382506884
2695.06848484848 0.000995819819049618
2729.72060606061 0.000971674164323544
2764.37272727273 0.000948330792522103
2799.02484848485 0.000925755535035356
2833.67696969697 0.00090391600451551
2868.32909090909 0.000882781484918777
2902.98121212121 0.00086232282938819
2937.63333333333 0.000842512365343732
2972.28545454545 0.000823323806203255
3006.93757575758 0.000804732169209168
3041.5896969697 0.000786713698882281
3076.24181818182 0.000769245795666048
3110.89393939394 0.000752306949362358
3145.54606060606 0.000735876676994226
3180.19818181818 0.00071993546476163
3214.8503030303 0.000704464713785033
3249.50242424242 0.000689446689356362
3284.15454545455 0.000674864473440515
3318.80666666667 0.00066070192019144
3353.45878787879 0.000646943614265942
3388.11090909091 0.000633574831735791
3422.76303030303 0.000620581503414615
3457.41515151515 0.000607950180430497
3492.06727272727 0.000595668001888431
3526.71939393939 0.000583722664478867
3561.37151515151 0.000572102393899643
3596.02363636364 0.000560795917968635
3630.67575757576 0.000549792441313846
3665.32787878788 0.000539081621536001
3699.98 0.000528653546746595
};
\addplot [very thick, chocolate21910927]
table {%
33.2 1.07875574027478
121.448080808081 0.0700137802215456
209.696161616162 0.0276458437836219
297.944242424242 0.0163065159621878
386.192323232323 0.0114349050488914
474.440404040404 0.00881365406971445
562.688484848485 0.00720425943305682
650.936565656566 0.00612674073722537
739.184646464646 0.00535992003026423
827.432727272727 0.00478896436406432
915.680808080808 0.00434880385436633
1003.92888888889 0.00400001214391218
1092.17696969697 0.00371740065116262
1180.42505050505 0.00348417047286442
1268.67313131313 0.00328871256918561
1356.92121212121 0.00312276093769794
1445.16929292929 0.00298027796332541
1533.41737373737 0.00285675563008815
1621.66545454545 0.00274876288792958
1709.91353535354 0.00265364401007905
1798.16161616162 0.00256931249358489
1886.4096969697 0.00249410709589583
1974.65777777778 0.00242668927539529
2062.90585858586 0.00236596882678676
2151.15393939394 0.00231104909476139
2239.40202020202 0.00226118602463796
2327.6501010101 0.0022157571502639
2415.89818181818 0.00217423782363043
2504.14626262626 0.00213618279298855
2592.39434343434 0.00210121178013684
2680.64242424242 0.00206899808212376
2768.8905050505 0.00203925948436417
2857.13858585859 0.00201175095757742
2945.38666666667 0.00198625874393568
3033.63474747475 0.00196259553430813
3121.88282828283 0.00194059650927423
3210.13090909091 0.00192011606903561
3298.37898989899 0.0019010251166014
3386.62707070707 0.00188320878824566
3474.87515151515 0.00186656454778535
3563.12323232323 0.00185100057852919
3651.37131313131 0.00183643442012226
3739.61939393939 0.0018227918079231
3827.86747474747 0.00181000568071016
3916.11555555556 0.00179801532895025
4004.36363636364 0.0017867656609687
4092.61171717172 0.00177620656843548
4180.8597979798 0.00176629237585254
4269.10787878788 0.00175698136136405
4357.35595959596 0.00174823533834981
4445.60404040404 0.00174001928900313
4533.85212121212 0.00173230104251856
4622.1002020202 0.00172505099168602
4710.34828282828 0.00171824184265299
4798.59636363636 0.00171184839341678
4886.84444444444 0.00170584733727426
4975.09252525252 0.00170021708801131
5063.34060606061 0.00169493762407971
5151.58868686869 0.00168999034939992
5239.83676767677 0.00168535796875756
5328.08484848485 0.00168102437604037
5416.33292929293 0.00167697455379899
5504.58101010101 0.00167319448281578
5592.82909090909 0.00166967106053798
5681.07717171717 0.00166639202737817
5769.32525252525 0.00166334590001121
5857.57333333333 0.00166052191090509
5945.82141414141 0.00165790995341668
6034.06949494949 0.00165550053186413
6122.31757575758 0.00165328471605763
6210.56565656566 0.00165125409983098
6298.81373737374 0.0016494007631694
6387.06181818182 0.0016477172375748
6475.3098989899 0.00164619647435048
6563.55797979798 0.00164483181552199
6651.80606060606 0.00164361696714216
6740.05414141414 0.00164254597475526
6828.30222222222 0.00164161320081943
6916.5503030303 0.00164081330390723
7004.79838383838 0.00164014121952325
7093.04646464646 0.00163959214239393
7181.29454545454 0.00163916151009933
7269.54262626263 0.00163884498792995
7357.79070707071 0.00163863845486266
7446.03878787879 0.00163853799056062
7534.28686868687 0.00163853986331096
7622.53494949495 0.00163864051882219
7710.78303030303 0.00163883656981076
7799.03111111111 0.00163912478631251
7887.27919191919 0.00163950208666109
7975.52727272727 0.00163996552908008
8063.77535353535 0.00164051230384082
8152.02343434343 0.001641139725942
8240.27151515151 0.00164184522827094
8328.5195959596 0.00164262635520996
8416.76767676768 0.00164348075665444
8505.01575757576 0.00164440618241193
8593.26383838384 0.00164540047695432
8681.51191919192 0.00164646157449735
8769.76 0.00164758749438382
};
\addplot [very thick, purple11522131]
table {%
108.08 0.0895185170649146
193.045656565657 0.0487836066821809
278.011313131313 0.0329285584073989
362.97696969697 0.024567247969211
447.942626262626 0.0194351596184134
532.908282828283 0.0159806930640571
617.87393939394 0.0135058901091305
702.839595959596 0.0116512063990235
787.805252525253 0.010212976771416
872.770909090909 0.00906740193657323
957.736565656566 0.00813500561170207
1042.70222222222 0.00736249210771913
1127.66787878788 0.00671282496735105
1212.63353535354 0.00615949038813987
1297.59919191919 0.00568302391612333
1382.56484848485 0.00526882435632647
1467.53050505051 0.00490573156119189
1552.49616161616 0.00458507433704899
1637.46181818182 0.00430001695381501
1722.42747474747 0.00404510063079355
1807.39313131313 0.0038159154790785
1892.35878787879 0.00360886164750061
1977.32444444444 0.00342097266245566
2062.2901010101 0.00324978289715514
2147.25575757576 0.00309322685414857
2232.22141414141 0.00294956171641279
2317.18707070707 0.00281730714387302
2402.15272727273 0.00269519800742618
2487.11838383838 0.00258214693781309
2572.08404040404 0.00247721439775009
2657.0496969697 0.00237958457630708
2742.01535353535 0.00228854582944738
2826.98101010101 0.00220347469993652
2911.94666666667 0.00212382277738554
2996.91232323232 0.00204910582830723
3081.87797979798 0.00197889475292926
3166.84363636364 0.00191280802152319
3251.80929292929 0.00185050531627934
3336.77494949495 0.00179168216111049
3421.74060606061 0.00173606536542839
3506.70626262626 0.00168340914200128
3591.67191919192 0.0016334917857526
3676.63757575758 0.00158611282150216
3761.60323232323 0.0015410905454572
3846.56888888889 0.00149825989869681
3931.53454545455 0.00145747062169152
4016.5002020202 0.00141858564762416
4101.46585858586 0.00138147969935998
4186.43151515152 0.00134603806069018
4271.39717171717 0.00131215549720477
4356.36282828283 0.0012797353060438
4441.32848484849 0.0012486884769919
4526.29414141414 0.00121893295004799
4611.2597979798 0.00119039295682235
4696.22545454546 0.00116299843496786
4781.19111111111 0.00113668450640716
4866.15676767677 0.0011113910114254
4951.12242424243 0.00108706209180203
5036.08808080808 0.001063645817089
5121.05373737374 0.00104109384893612
5206.01939393939 0.00101936113903941
5290.98505050505 0.000998405656864911
5375.95070707071 0.000978188143793844
5460.91636363636 0.000958671890758828
5545.88202020202 0.000939822536805088
5630.84767676768 0.000921607886325218
5715.81333333333 0.000903997742987736
5800.77898989899 0.000886963758615183
5885.74464646465 0.000870479295472199
5970.7103030303 0.000854519300601821
6055.67595959596 0.000839060191003663
6140.64161616162 0.000824079748583172
6225.60727272727 0.000809557023920024
6310.57292929293 0.000795472248007838
6395.53858585859 0.000781806751209009
6480.50424242424 0.000768542888749052
6565.4698989899 0.000755663972145963
6650.43555555556 0.00074315420603288
6735.40121212121 0.000730998629887973
6820.36686868687 0.000719183064234705
6905.33252525253 0.000707694060919345
6990.29818181818 0.00069651885711149
7075.26383838384 0.000685645332708039
7160.2294949495 0.000675061970851789
7245.19515151515 0.000664757821303549
7330.16080808081 0.000654722466431177
7415.12646464647 0.000644945989601095
7500.09212121212 0.000635418945777607
7585.05777777778 0.000626132334153047
7670.02343434343 0.000617077572647838
7754.98909090909 0.000608246474133835
7839.95474747475 0.000599631224247299
7924.9204040404 0.000591224360669517
8009.88606060606 0.000583018753763623
8094.85171717172 0.000575007588465712
8179.81737373737 0.000567184347336966
8264.78303030303 0.000559542794691316
8349.74868686869 0.000552076961720264
8434.71434343434 0.000544781132542927
8519.68 0.000537649831115191
};
\addplot [very thick, black18]
table {%
33.2 0.522781230194577
120.906060606061 0.0783834873783186
208.612121212121 0.0333765540917374
296.318181818182 0.0189522820872485
384.024242424242 0.0123726334776837
471.730303030303 0.00877677766103672
559.436363636364 0.00658022761200427
647.142424242424 0.00513271302733287
734.848484848485 0.00412470106522072
822.554545454546 0.00339263269636509
910.260606060606 0.00284308165633538
997.966666666667 0.00241935443313055
1085.67272727273 0.00208534124287676
1173.37878787879 0.00181711180706639
1261.08484848485 0.00159827304553899
1348.79090909091 0.00141727505215694
1436.49696969697 0.00126578132663018
1524.20303030303 0.00113764716752194
1611.90909090909 0.00102825929251329
1699.61515151515 0.000934097334166926
1787.32121212121 0.000852435682887536
1875.02727272727 0.000781136443186013
1962.73333333333 0.000718502925273741
2050.43939393939 0.000663174199130828
2138.14545454545 0.000614048028138933
2225.85151515151 0.000570223752199596
2313.55757575758 0.000530959412710235
2401.26363636364 0.00049563918944729
2488.9696969697 0.00046374840138605
2576.67575757576 0.000434854122547739
2664.38181818182 0.000408590012480059
2752.08787878788 0.000384644342860706
2839.79393939394 0.000362750471086682
2927.5 0.000342679204047567
3015.20606060606 0.000324232634174876
3102.91212121212 0.000307239131228308
3190.61818181818 0.000291549247997875
3278.32424242424 0.000277032353689618
3366.0303030303 0.000263573850482376
3453.73636363636 0.000251072860312922
3541.44242424242 0.00023944029302233
3629.14848484848 0.000228597225492085
3716.85454545455 0.000218473535706482
3804.56060606061 0.000209006746819635
3892.26666666667 0.000200141045036024
3979.97272727273 0.000191826441995551
4067.67878787879 0.000184018057809785
4155.38484848485 0.000176675505244525
4243.09090909091 0.000169762359027401
4330.79696969697 0.000163245697064078
4418.50303030303 0.000157095702615282
4506.20909090909 0.000151285318330329
4593.91515151515 0.000145789944537185
4681.62121212121 0.000140587175421832
4769.32727272727 0.000135656567743824
4857.03333333333 0.000130979437572488
4944.73939393939 0.000126538681222428
5032.44545454545 0.000122318617144403
5120.15151515152 0.000118304846009647
5207.85757575758 0.000114484126629223
5295.56363636364 0.000110844265689038
5383.2696969697 0.000107374019566775
5470.97575757576 0.000104063006738346
5558.68181818182 0.000100901629486079
5646.38787878788 9.78810037946177e-05
5734.09393939394 9.49928964686601e-05
5821.8 9.22296686331724e-05
5909.50606060606 8.95842248850469e-05
5997.21212121212 8.70499674581839e-05
6084.91818181818 8.46207548440078e-05
6172.62424242424 8.2290864378426e-05
6260.3303030303 8.00549583658912e-05
6348.03636363636 7.79080533628855e-05
6435.74242424242 7.58454922879713e-05
6523.44848484848 7.38629190645622e-05
6611.15454545454 7.19562555365168e-05
6698.86060606061 7.01216804263459e-05
6786.56666666667 6.83556101317447e-05
6874.27272727273 6.66546811788994e-05
6961.97878787879 6.50157341709721e-05
7049.68484848485 6.34357990877056e-05
7137.39090909091 6.19120818075325e-05
7225.09696969697 6.04419517372166e-05
7312.80303030303 5.90229304460746e-05
7400.50909090909 5.7652681212497e-05
7488.21515151515 5.63289993999185e-05
7575.92121212121 5.50498035877666e-05
7663.62727272727 5.38131273903731e-05
7751.33333333333 5.2617111903449e-05
7839.03939393939 5.14599987236399e-05
7926.74545454545 5.03401234919423e-05
8014.45151515151 4.92559099164756e-05
8102.15757575758 4.82058642343186e-05
8189.86363636364 4.71885700758896e-05
8277.5696969697 4.62026836987394e-05
8365.27575757576 4.52469295606647e-05
8452.98181818182 4.43200962047814e-05
8540.68787878788 4.34210324316574e-05
8628.39393939394 4.2548643735821e-05
8716.1 4.17018889859611e-05
};
\addplot [very thick, darkgray153]
table {%
33.2 0.81182053213339
118.354747474747 0.0733006368095973
203.509494949495 0.0263520291493571
288.664242424242 0.0136337837701197
373.81898989899 0.00837772916635324
458.973737373737 0.00569285837317061
544.128484848485 0.00413277887098602
629.283232323232 0.003143884806044
714.43797979798 0.00247642305927133
799.592727272727 0.00200399173947109
884.747474747475 0.00165692059981762
969.902222222222 0.00139418936751723
1055.05696969697 0.00119034085174615
1140.21171717172 0.00102888196325941
1225.36646464646 0.000898737460960972
1310.52121212121 0.000792241297177217
1395.67595959596 0.000703947434462756
1480.83070707071 0.000629898737288646
1565.98545454545 0.000567162594066866
1651.1402020202 0.000513527445462487
1736.29494949495 0.000467299432823784
1821.4496969697 0.000427163070614815
1906.60444444444 0.000392083868398678
1991.75919191919 0.000361239044165331
2076.91393939394 0.000333967421776298
2162.06868686869 0.000309732664614985
2247.22343434343 0.000288095931393343
2332.37818181818 0.000268695288001356
2417.53292929293 0.000251230029906454
2502.68767676768 0.000235448618636004
2587.84242424242 0.000221139309077989
2672.99717171717 0.000208122801768505
2758.15191919192 0.000196246434340149
2843.30666666667 0.000185379553768852
2928.46141414141 0.00017540980238169
3013.61616161616 0.000166240116742238
3098.77090909091 0.000157786286945567
3183.92565656566 0.000149974959631011
3269.0804040404 0.000142741994697487
3354.23515151515 0.000136031105767987
3439.3898989899 0.00012979272965885
3524.54464646465 0.000123983081727286
3609.69939393939 0.000118563362909439
3694.85414141414 0.000113499091185619
3780.00888888889 0.000108759535608201
3865.16363636364 0.000104317235262917
3950.31838383838 0.000100147588876252
4035.47313131313 9.62285034334808e-05
4120.62787878788 9.25400922872869e-05
4205.78262626263 8.90644149329689e-05
4290.93737373737 8.57852519927565e-05
4376.09212121212 8.26879100578092e-05
4461.24686868687 7.97590519357438e-05
4546.40161616162 7.69865485857916e-05
4631.55636363636 7.43593496256592e-05
4716.71111111111 7.18673697896477e-05
4801.86585858586 6.95013891269252e-05
4887.02060606061 6.72529650683018e-05
4972.17535353535 6.51143547722718e-05
5057.3301010101 6.30784463969204e-05
5142.48484848485 6.11386981418045e-05
5227.6395959596 5.92890840698736e-05
5312.79434343434 5.75240458593871e-05
5397.94909090909 5.58384497539899e-05
5483.10383838384 5.42275480793425e-05
5568.25858585859 5.2686944779862e-05
5653.41333333333 5.12125645017294e-05
5738.56808080808 4.98006248103272e-05
5823.72282828283 4.84476111833929e-05
5908.87757575757 4.71502544667768e-05
5994.03232323232 4.59055105189336e-05
6079.18707070707 4.47105418041269e-05
6164.34181818182 4.35627007235817e-05
6249.49656565656 4.2459514499164e-05
6334.65131313131 4.13986714461564e-05
6419.80606060606 4.03780084908441e-05
6504.96080808081 3.9395499805283e-05
6590.11555555556 3.84492464461893e-05
6675.2703030303 3.75374668976163e-05
6760.42505050505 3.6658488428242e-05
6845.5797979798 3.58107391838881e-05
6930.73454545454 3.49927409444982e-05
7015.88929292929 3.42031024823883e-05
7101.04404040404 3.34405134652782e-05
7186.19878787879 3.27037388535163e-05
7271.35353535353 3.19916137461503e-05
7356.50828282828 3.13030386351264e-05
7441.66303030303 3.0636975031016e-05
7526.81777777778 2.99924414273313e-05
7611.97252525252 2.93685095737369e-05
7697.12727272727 2.87643010313762e-05
7782.28202020202 2.81789839861138e-05
7867.43676767677 2.76117702978092e-05
7952.59151515151 2.7061912765813e-05
8037.74626262626 2.65287025927244e-05
8122.90101010101 2.60114670301149e-05
8208.05575757576 2.55095671914201e-05
8293.21050505051 2.50223960185385e-05
8378.36525252525 2.45493763898895e-05
8463.52 2.40899593587706e-05
};
\addplot [very thick, saddlebrown1356716]
table {%
527.68 0.0204671540339114
576.211111111111 0.0143913598887822
624.742222222222 0.0105200168851043
673.273333333333 0.00794237585652515
721.804444444444 0.00616158902365322
770.335555555556 0.00489211760170549
818.866666666667 0.00396243046955861
867.397777777778 0.00326548108335065
915.928888888889 0.00273221556001934
964.46 0.00231677578348645
1012.99111111111 0.00198791624404395
1061.52222222222 0.00172385626476419
1110.05333333333 0.00150909960763035
1158.58444444444 0.00133241668029578
1207.11555555556 0.00118553338393754
1255.64666666667 0.00106226051075773
1304.17777777778 0.0009579041938585
1352.70888888889 0.000868859454546761
1401.24 0.000792325340225134
1449.77111111111 0.000726102240336101
1498.30222222222 0.000668445649953659
1546.83333333333 0.00061795929147607
1595.36444444444 0.000573516061840672
1643.89555555556 0.000534198906934887
1692.42666666667 0.000499256139059724
1740.95777777778 0.000468067340485915
1789.48888888889 0.000440117107861279
1838.02 0.000414974661475363
1886.55111111111 0.000392277882035744
1935.08222222222 0.00037172071902755
1983.61333333333 0.000353043187666395
2032.14444444444 0.000336023368714338
2080.67555555556 0.000320470969334683
2129.20666666667 0.000306222109079386
2177.73777777778 0.000293135073717654
2226.26888888889 0.000281086838430404
2274.8 0.000269970206233081
2323.33111111111 0.000259691441153701
2371.86222222222 0.000250168301429291
2420.39333333333 0.000241328397787752
2468.92444444444 0.000233107817216399
2517.45555555556 0.000225449964562676
2565.98666666667 0.000218304583669136
2614.51777777778 0.000211626927114463
2663.04888888889 0.000205377049467329
2711.58 0.00019951920360305
2760.11111111111 0.000194021323345185
2808.64222222222 0.00018885457867645
2857.17333333333 0.000183992992168978
2905.70444444444 0.000179413107233455
2954.23555555556 0.000175093700372619
3002.76666666667 0.000171015530919997
3051.29777777778 0.000167161122806946
3099.82888888889 0.000163514573775098
3148.36 0.000160061388173182
3196.89111111111 0.000156788330075339
3245.42222222222 0.000153683293955439
3293.95333333333 0.000150735190566676
3342.48444444444 0.000147933846022817
3391.01555555556 0.000145269912368699
3439.54666666667 0.000142734788172721
3488.07777777778 0.000140320547880873
3536.60888888889 0.000138019878846992
3585.14 0.000135826025102383
3633.67111111111 0.000133732737054384
3682.20222222222 0.000131734226411113
3730.73333333333 0.000129825125721848
3779.26444444444 0.000128000452001328
3827.79555555556 0.00012625557397408
3876.32666666667 0.000124586182533217
3924.85777777778 0.000122988264058449
3973.38888888889 0.000121458076281545
4021.92 0.000119992126425158
4070.45111111111 0.000118587151373609
4118.98222222222 0.000117240099662638
4167.51333333333 0.000115948115099898
4216.04444444444 0.000114708521849575
4264.57555555556 0.000113518810833412
4313.10666666667 0.000112376627316939
4361.63777777778 0.000111279759564242
4410.16888888889 0.000110226128457375
4458.7 0.000109213777987695
4507.23111111111 0.000108240866536347
4555.76222222222 0.000107305658869836
4604.29333333333 0.000106406518784347
4652.82444444444 0.000105541902339345
4701.35555555556 0.000104710351626999
4749.88666666667 0.000103910489029435
4798.41777777778 0.00010314101192053
4846.94888888889 0.000102400687773312
4895.48 0.000101688349637766
4944.01111111111 0.00010100289195727
4992.54222222222 0.000100343266694944
5041.07333333333 9.97084797438437e-05
5089.60444444444 9.90975875974703e-05
5138.13555555556 9.8509694259125e-05
5186.66666666667 9.79439483707224e-05
5235.19777777778 9.73995405433439e-05
5283.72888888889 9.68757008734699e-05
5332.26 9.63716966302043e-05
};
\addplot [draw=black, fill=black, mark=x, very thick, mark size=2.5pt, only marks]
table{%
x  y
131.28 0.167918891881762
527.68 0.0273828282351949
2115.84 0.00412211953977583
8519.68 0.00052947992331703
};

==> figures/quantitative_results/group_main_1.tex <==
\nextgroupplot[
ylabel shift = -0.2cm,
clip marker paths=true,
width=0.52\textwidth,
title style={yshift=-0.2cm},
height=4.5cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
title={Poisson's Equation},
x grid style={darkgray176},
xlabel={\empty},
xmajorgrids,
xmin=-425.719, xmax=9421.899,
xtick style={color=black},
xtick={-2000,0,2000,4000,6000,8000,10000},
xticklabels={-2.0,0.0,2.0,4.0,6.0,8.0,10.0},
y grid style={darkgray176},
ylabel={Squared Error},
ymajorgrids,
ymin=3.22979249486793e-06, ymax=1.84089349960545,
ymode=log,
ytick style={color=black},
ytick={1e-07,1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
}
]
\addplot [
  draw=royalblue28108204,
  fill=royalblue28108204,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
219.22 0.0116380025783674
236.58 0.00893751131252496
255.06 0.00757221773421185
266.3 0.00695152587324572
277.02 0.00870449843080493
289.06 0.00650849332548639
301.82 0.00650772537377039
309.02 0.00632830538267971
313.48 0.00852456067483164
317.48 0.00503420224308783
366.78 0.00472734343816265
384.24 0.00384945126787151
427.52 0.00440570193112838
431.14 0.00387196288409598
433.8 0.0031068838328975
438.92 0.0033561305566538
446.06 0.00325148782214415
485 0.00270934352590588
524.5 0.0019590317268996
530.98 0.0024847849713976
530.98 0.0024462804500235
542.2 0.00339373662958677
568.26 0.00191195330793864
569.1 0.00200759214947172
579.8 0.00192121084682089
587.66 0.00166535004820132
612.06 0.00170099739413765
628 0.00142557999535175
636.98 0.00193167521782833
648.04 0.00147630841918046
648.78 0.00196488850395651
684.76 0.00192456325257735
704.12 0.00152017798836435
708.02 0.00171515266408961
724.56 0.00106290863523144
740.7 0.00145038634314574
740.82 0.00126611233262213
754.68 0.0010958404611985
776.14 0.00136681288549904
861 0.00122261947029662
866.82 0.0012376456173406
951.18 0.000684639740045543
978.82 0.000682995459645206
1030.58 0.000639142132617508
1031.2 0.000608987227553708
1080.16 0.000534351174466062
1116.56 0.000522936657826564
1126.22 0.00047220578013082
1173.32 0.000587407673606018
1183.24 0.000496992672901857
1212.6 0.000433759599768057
1270.84 0.000477030829124065
1271.28 0.00057574970357699
1312.64 0.000295338105933881
1334.88 0.0003688460635094
1390.92 0.000632823129081481
1414.42 0.000439822660083419
1465.2 0.000380405825070989
1546.18 0.000259777992401812
1645.64 0.000189432782231567
1650.1 0.00040730379394757
1712.26 0.000225696747843442
1799.62 0.000205137266591349
1800.64 0.000149688394684308
1820.82 0.00022968203197516
1908.42 0.000134858938308452
1925.1 0.000231468966668099
2020.12 0.000123482420852495
2156.38 0.000114435638078513
2168.78 0.000132258579214635
2169 0.000101440195225082
2212 0.000202015930911123
2238.3 0.000100444720362762
2307.32 0.00010430451268494
2321.26 0.000101348576943888
2363.12 7.85396281013735e-05
2399.82 8.97496755911525e-05
2432.68 0.000175103698214891
2457.16 9.48685731254995e-05
2655.7 7.07642905549767e-05
2715.22 5.85765922707877e-05
3044.4 5.85685554721719e-05
3414.76 4.01750628140733e-05
3545.46 3.80019302781983e-05
3591.66 3.62548169075136e-05
3997.22 3.19018762058348e-05
4033.6 2.70246768067793e-05
4075.94 2.55319826966762e-05
4148.74 2.90210310242148e-05
4304.56 2.36833753484687e-05
4311.96 4.28165553247746e-05
4611.22 2.13677683411378e-05
5764.26 1.3085878413959e-05
6013.74 1.0832458588431e-05
6168.52 9.73742044189171e-06
6591.82 8.02970379055727e-06
6800.42 8.43665609892419e-06
6819.78 8.29434337198603e-06
7381.26 8.13257734004449e-06
7648.78 6.34432528857979e-06
};
\addplot [
  draw=cadetblue80178158,
  fill=cadetblue80178158,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
238.86 0.0314591256860586
259.2 0.0279614216442924
266.94 0.0440459298859297
270.78 0.0318815823464054
275.54 0.0593514293437776
292.74 0.0207354951700831
293.06 0.0221127116170605
307.06 0.0209106646236632
330.7 0.0702922818937551
350.14 0.0807482460346126
387.32 0.0620047069674773
426.5 0.00592632357712872
441.78 0.00526383493362311
449.52 0.00894098739715834
502.08 0.0128625751437315
527.28 0.00764885638127966
564.38 0.0278710432660707
581.08 0.00737865073205254
607.64 0.0116848347806724
657.88 0.0259621669592313
679.92 0.00755933491914977
695 0.00257071214077956
695.84 0.00395982101856514
702.54 0.0352949317001577
710.8 0.00739388781093521
765.8 0.00489009062296662
780.24 0.0120847799816269
789.02 0.00435340001031618
797.66 0.0791101360827437
870.48 0.215947865448271
877.5 0.202251458564746
953.76 0.00785133509905537
959.74 0.00230121519966155
963.22 0.00206243086349683
964.68 0.0083785913521835
1000.26 0.00346978020975467
1009.96 0.004142049657295
1047.06 0.00225157380159124
1122.86 0.003062103305598
1139.62 0.0020778500532229
1194.2 0.149376206797811
1203.38 0.00109219342001367
1237.52 0.017414815893132
1269.76 0.00153445767684243
1308.66 0.0101006962225929
1343.88 0.00195426204490739
1403.68 0.186316022036712
1474.82 0.00518823390213346
1483.06 0.00137966614553141
1508.22 0.00241542593084506
1533.24 0.108028873012002
1558.36 0.00154318317939186
1623.28 0.00324453968222031
1652.94 0.00306113530930337
1683.24 0.00136663132183301
1769.66 0.00043475425513794
1780.54 0.000525754510912481
1972.86 0.000937671471083318
1977.3 0.00144378189022144
2010.66 0.000830648873741841
2054.24 0.00866340439454498
2158.24 0.000664382562999057
2213.06 0.000443453811901927
2247.66 0.00487431109654702
2270.74 0.00172876918014416
2334.56 0.000310206885374613
2362.8 0.263314397040719
2473.06 0.00119230634636316
2481.1 0.000386263868361426
2492.44 0.000349575358333937
2507.76 0.00122087231252026
2526.96 0.00072060660227723
2528.42 0.000359101194848207
2681.3 0.00184721059179259
2719.26 0.0056335828642175
2783.24 0.000464571417157986
2793.82 0.000547802481503746
2812.56 0.122094542705312
2814.86 0.000552381231239201
2914.52 0.000395045921821014
2958.5 0.026449141273229
2974 0.00147822884589543
2979.64 0.0154154293281526
3023.04 0.00117847278133127
3044.12 0.00771705726110193
3145.88 0.000208994471589525
3162.34 0.00085605260280606
3183.74 0.0238842006531611
3285.24 0.000110283822470742
3285.78 0.000164999251045578
3304.3 0.000293792721768415
3309.32 0.000517710651832717
3351.3 0.000455257895227682
3373.9 0.000130315097348245
3462.92 0.0001628222984189
3705.6 0.000490453853139452
3714.04 0.000242224384089039
3748.38 0.0332845233781071
3834.84 0.000446808641735386
4033.74 0.00301583029691757
};
\addplot [
  draw=chocolate21910927,
  fill=chocolate21910927,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
21.9 0.999999998927878
21.9 0.999999998927878
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.92 0.999999998950274
21.94 0.999999998905941
21.94 0.999999998905941
21.94 0.999999998905941
21.94 0.999999998905941
22 0.999999998889839
22.02 0.999999998899304
22.16 0.999999998640609
22.28 0.999999998477158
26.5 0.970894204249672
32.62 0.924277946638112
34.96 0.862638850036096
91.4 0.720312311243077
94.9 0.18919499810567
108.74 0.71958749216895
134.98 0.0689210131272957
136.1 0.0613824673087774
155.44 0.0559306313583098
208.3 0.197146125458646
249.98 0.0499246702086478
271.24 0.0325903579711196
274.72 0.0511839347070228
283.88 0.043017706650582
308.14 0.288765844789137
329.14 0.0162289718257283
338.64 0.034337015545152
357.98 0.0101646670694072
386.82 0.0167657064564419
395.32 0.0042305451504377
403.3 0.0119398370592536
430.36 0.0289122109821289
531.96 0.11696073594285
595.12 0.58453985126498
642.3 0.00386796707321375
670.92 0.00302893160661771
695.68 0.00347257940790675
722.02 0.0391289662856242
762.26 0.00451677919851355
1152.26 0.0261976517911636
1233.2 0.000998733802377771
1272.96 0.000876420935487872
1282.64 0.00102417788068937
1315.36 0.000594576789097483
1410.32 0.00146055096768862
1658.3 0.0267799322922428
1817.54 0.222864808756589
1978.66 0.000274269869038731
2059.9 0.00791404372976221
2070.98 0.000261190457505995
2305.2 0.225290493210452
3213.16 0.000133900698026789
3434.82 0.000663721741809451
4206.7 0.000806185856602349
4447.52 0.000113588426911867
4668.8 0.000258317240468995
5045.36 4.79021802088747e-05
7591.98 3.04719971098142e-05
};
\addplot [draw=purple11522131, fill=purple11522131, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
78.58 0.301493427330464
85.08 0.274455743146065
85.76 0.247059957310875
104.82 0.127743695311313
116.6 0.135439329155988
118.2 0.174983189580105
120.4 0.0964925082987315
121.34 0.0988675248837244
135.02 0.112585768954093
197.68 0.0829814200198853
210.46 0.0645671680607277
223.72 0.0607998674259802
241.1 0.0504275656964269
297.98 0.0553802062154436
311.14 0.0404930406669039
323.64 0.022991687600625
333.94 0.0274936611138742
341.18 0.0269801010301793
341.2 0.028156653231875
342.48 0.00992160065898382
343.86 0.0267192329551306
346.56 0.0261208939579781
349.9 0.0251530914362062
351.26 0.0227907233444659
352.64 0.0239397173789617
355.92 0.0191090303397534
364.18 0.0218794329430158
370.24 0.0200638785751326
376.04 0.0136155573179307
381.9 0.0146785342366676
385.72 0.012640642012926
409 0.0129078349935975
418.96 0.00933051668986954
447.7 0.00934748444519734
452.28 0.0229373947300776
493.02 0.0056858045394716
499.32 0.00694086566029311
552.38 0.00895209879479779
572.84 0.00505305561248642
786.28 0.00258348532329224
833.92 0.00320550253911646
1257.9 0.00215555030491081
1339.34 0.00195086299350352
1353.52 0.00209068490575845
1356.5 0.00222798967646156
1396.46 0.00190324922233753
1421.5 0.00176630035985534
1422.22 0.00180824419903394
1425.32 0.001896163401944
1426.54 0.00176777019284238
1429.28 0.00170450464911716
1429.56 0.00189968336381655
1432.82 0.00177489483284763
1449.28 0.00189240844296632
1449.38 0.00189070300363587
1450.16 0.00193782213005509
1450.24 0.00189066552594398
1456.6 0.00190102776276496
1456.6 0.00190102776276496
1462.96 0.00198042805162412
1469.72 0.00162821515839203
1482.54 0.00132975900752616
1516.94 0.00106385341758505
1527.66 0.00105963343820681
1574.24 0.000997338909699857
1613.18 0.000647274604876434
1892.02 0.000604202070923351
1919.8 0.000576682497257652
1930.46 0.000710916067721463
2102.78 0.000469878926949001
2190.92 0.00081450106318767
2593.9 0.000243552880772975
3084.76 0.000263576696379211
3435.3 0.000184887847662381
3657.84 0.000203971119068862
3703.24 0.000186005272034085
3759.92 0.000197947946581525
3996.78 0.000188218954708874
4612.32 0.000214224514655938
5706.3 0.000144931275103409
5716.12 0.000155178357462367
5718.68 0.000144788209431815
5744.66 0.000144619952836946
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
5765.12 0.000144604747120997
};
\addplot [draw=black18, fill=black18, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
21.92 0.999999998950274
83.82 0.0565991403312627
84.92 0.0588434607820434
87.46 0.0545513186266436
89.44 0.0531291257532859
91.3 0.0515217060177
93.44 0.0480001628274194
96.28 0.0467487104402012
100.36 0.0433061758426616
102.3 0.0415798392741656
106.2 0.038275903318379
107.12 0.0372273805784123
110.02 0.0357377313643206
113.5 0.0319765669036278
115.38 0.0296578466886223
120.22 0.0284679207307645
123.52 0.0267085079418755
127.8 0.0251518540082812
129.9 0.0248574705995461
136.5 0.0209990308167946
139.42 0.0199226295055767
141.48 0.0198756524374638
142.1 0.0197127637668238
144.48 0.0191718935347858
149.58 0.0183330737846724
156.82 0.016898848442373
167.62 0.0156431375315336
167.9 0.0153476420456348
173.88 0.0136691014180857
174.22 0.0147322899942479
182 0.0130232029511979
190.2 0.0119863084446229
202.6 0.0111271027480034
210.64 0.0102835108948271
215.74 0.00946573785573982
223.3 0.00935835078227575
234.66 0.00876949811989275
243.76 0.00794194352009218
249.54 0.00731416749373406
254.44 0.00712263453479527
266.76 0.00631241799950617
280.28 0.00591988306616931
303.3 0.00528315768049147
314.52 0.00490564968309633
333.12 0.00442007209387173
354.68 0.00387193325893414
361.4 0.00371106066501458
384.2 0.00300969495379285
387.46 0.00318275076293748
421.82 0.00259540854325304
441.9 0.00237988095775454
449.8 0.00229588028434392
471.36 0.00200396605681757
484.58 0.00182979486232863
533.58 0.00169527536071066
556.12 0.00150706174146262
579.36 0.00150071729081547
605.72 0.00137742631748754
653.74 0.00120926624525868
701.24 0.00109419178867071
760.14 0.00091264464581015
808.02 0.000832556955903132
859.1 0.000747053380373828
888.1 0.000692876630678483
1011.82 0.000595294323974944
1060.48 0.000510602303872567
1108.76 0.00047774453235278
1250.74 0.000407819374192714
1392.44 0.000330743620421011
1462.76 0.000276544739610269
1504.58 0.000249372526617893
1650.76 0.000203598112706266
1810.98 0.000169667478610816
2048.04 0.000140076164755548
2159.52 0.000120980786924505
2339.48 0.000106310019037566
2638.86 8.57536496349864e-05
2908.8 6.88814297530126e-05
3134.48 6.04724152185696e-05
3466.7 5.05035384212832e-05
4017.1 3.9037987620245e-05
4404.1 3.16366332585035e-05
4973.16 2.39541099394721e-05
5396.44 1.97349819656197e-05
6214.76 1.4498315180921e-05
7342.48 1.07893422272306e-05
8052.28 7.80335850902706e-06
};
\addplot [draw=darkgray153, fill=darkgray153, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
21.92 0.999999998950274
112.1 0.0303243408055568
121.94 0.0276176454252955
125.02 0.0259477996440306
127.98 0.0244287341728597
138.98 0.0227191753539499
143.6 0.020910043928064
148.64 0.0206439652679976
155.34 0.0196985048965192
159.38 0.018596093274776
163.04 0.0175493257955033
173.26 0.016473342312274
184.38 0.0162006011390902
189.82 0.015450059393199
200.12 0.0146389860622553
210.08 0.0136365820202889
212.12 0.0137341483938617
218.28 0.0134631137044205
223.08 0.0127641472302505
232.76 0.012307991229748
239.16 0.0115034420838717
248.16 0.0112811193908862
259.42 0.0107052707594736
295.02 0.00996943853327848
315.92 0.00934406359066508
319.6 0.00881669699253116
343.7 0.00871252964265616
371.16 0.00839024171553709
391.2 0.00793169608711516
396.18 0.00751484779745654
399.22 0.00681808320575125
436.02 0.00649267245273593
471.9 0.00621478437348911
521.14 0.00582989924711537
565.12 0.00570107859311501
622.1 0.00520474619919274
638.1 0.00506894387509509
649.18 0.00478703465169344
720.84 0.00442442533962123
789.56 0.00412619132689798
807.8 0.00397758535516771
884.5 0.00355011380476904
897.94 0.00343187975951783
900.8 0.00315986307399483
1003.52 0.00304836434880253
1047.6 0.00274246060829574
1150.08 0.00245705872922855
1192.4 0.00234140291374883
1208.36 0.00224216602812112
1283.26 0.00204533432594027
1414.4 0.00187099364683792
1479.3 0.00177157620603225
1532.08 0.00160584644786739
1677.04 0.00140319692242571
1743.56 0.00134329557397193
1780.1 0.00123054360060732
1866.06 0.00110971226628307
2056.6 0.000986271100410831
2216.46 0.000910590142508534
2387.08 0.000740586744135399
2650.56 0.000671638593555898
2685.78 0.000623070461710295
2863.26 0.000561448059636026
2988.82 0.000507482424440779
3181.46 0.000442796433540224
3376.28 0.00038785815595569
3571.42 0.000324153929771946
3817.98 0.000282257887838828
3888.68 0.000260771272496118
4047.44 0.000235620426098432
4347.12 0.000211041124908258
4677.46 0.000166394105666857
4890.32 0.000150551223206391
5284.12 0.000126332217339954
5652.04 0.000107981520467349
6214.2 8.25597002555252e-05
6445.84 7.16315559937878e-05
6915.98 6.13875970270764e-05
7242.06 5.31338013209708e-05
7650 4.49797649208315e-05
7997.06 3.85029184051354e-05
8366.84 3.45654105103186e-05
};
\addplot [
  draw=saddlebrown1356716,
  fill=saddlebrown1356716,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
351.36 0.0259470568426135
424.78 0.00932584828733208
430 0.00871409822286043
432.9 0.00765906975946302
435.62 0.00724690570691994
447.9 0.00694617455805699
461.08 0.00632115483471587
470.06 0.0061098007545293
489.18 0.00572775513817063
502.8 0.00543050338169425
531.94 0.00507370072263522
539.4 0.00473767518661581
563.94 0.00446869544912157
593.34 0.00393751246044451
630.24 0.00360041213744293
651.9 0.00335968242838088
667.64 0.00308164656033296
697.98 0.00285585163917606
751.54 0.00264686469786277
782.02 0.00253747275344309
828.18 0.00231160538943217
862.7 0.00200277154871525
910.22 0.00183540369769237
939.38 0.00176632212946235
965.44 0.00156967277894731
1025.7 0.00142082445381516
1096.1 0.00127457991642592
1133.32 0.00118572128652756
1227.88 0.00107500778600639
1278.42 0.0010443276155184
1288.72 0.000978921635742221
1378.34 0.000917210502572047
1392.68 0.0008921582037726
1448.98 0.000826411273939311
1455.56 0.000785323339770194
1510.14 0.000744352728044646
1572.3 0.000710315407438729
1613.16 0.00068083415211576
1634.9 0.000651483249550822
1689.78 0.000617482855499086
1823.26 0.000591893045434779
1865.44 0.000562543029194233
1976.94 0.000537038663552404
2003.3 0.000505353158115542
2043.8 0.000478304111776504
2071.48 0.000453906402098779
2135.88 0.000439543436736492
2177.14 0.000416172756268122
2225.02 0.000393887788024111
2349.2 0.000374526585907536
2407.9 0.00036459437929653
2539.78 0.000343184120521825
2623.46 0.000330660666260436
2698.26 0.000319360738810362
2853.62 0.000300605143331689
2949.36 0.000288519182456857
3120.5 0.000276625356045883
3278.58 0.000263386658651786
3433.66 0.000248319920322957
3506.04 0.000236549656664321
3630.82 0.00022696628636019
3709.02 0.000213877379050273
3870.94 0.000200166905231589
3992.1 0.000193156032078103
4296.7 0.000170100086985167
4302.06 0.00018133531780408
4555.88 0.0001601867644446
4684.72 0.000151811161019907
4929.24 0.000142345422047352
5063.38 0.000135516332472281
5234.24 0.000126415898692477
5437.96 0.000119865724061041
5528.6 0.000113300665004034
5699.12 0.000107559023988025
5925.72 0.000100357468654651
6186.72 9.49377140833932e-05
6343.1 8.87199523412338e-05
6605.28 8.38636699308428e-05
6834.42 7.858059334281e-05
6985.8 7.3204392919636e-05
7234.7 6.81103278539808e-05
7450.26 6.42815752805545e-05
7708.22 6.13769970515243e-05
7904.6 5.83514931244077e-05
8186.16 5.42609465339326e-05
8398.18 5.12519049536946e-05
8559.14 4.83525137048323e-05
8974.28 4.53478390058807e-05
};
\addplot [very thick, royalblue28108204]
table {%
219.22 0.011036362330508
294.266060606061 0.00683752177615596
369.312121212121 0.00464144864349475
444.358181818182 0.00334666716525019
519.404242424242 0.0025193038327363
594.450303030303 0.00195898836228103
669.496363636364 0.00156242272863255
744.542424242424 0.00127184853740656
819.588484848485 0.00105288309708372
894.634545454545 0.000884011430865333
969.680606060606 0.000751210162546177
1044.72666666667 0.000645022898528129
1119.77272727273 0.000558886634562944
1194.81878787879 0.000488132454642395
1269.86484848485 0.000429366813814566
1344.91090909091 0.000380076270852898
1419.95696969697 0.000338367971794018
1495.00303030303 0.0003027951072934
1570.04909090909 0.000272236981973959
1645.09515151515 0.000245815016365929
1720.14121212121 0.000222832893735278
1795.18727272727 0.000202733241627402
1870.23333333333 0.000185065832838411
1945.27939393939 0.000169463938324359
2020.32545454545 0.000155626532140522
2095.37151515152 0.000143304752953709
2170.41757575758 0.00013229149937599
2245.46363636364 0.000122413358503866
2320.5096969697 0.00011352428972744
2395.55575757576 0.00010550064185257
2470.60181818182 9.82371921850629e-05
2545.64787878788 9.16439755603686e-05
2620.69393939394 8.56437288176314e-05
2695.74 8.01698183332399e-05
2770.78606060606 7.51645493600184e-05
2845.83212121212 7.05777791330937e-05
2920.87818181818 6.63657731597201e-05
2995.92424242424 6.24902573397632e-05
3070.9703030303 5.89176286642295e-05
3146.01636363636 5.56182950054424e-05
3221.06242424242 5.25661205236171e-05
3296.10848484848 4.97379578968152e-05
3371.15454545455 4.71132522503113e-05
3446.20060606061 4.46737045530535e-05
3521.24666666667 4.24029845402706e-05
3596.29272727273 4.02864850465218e-05
3671.33878787879 3.83111110946094e-05
3746.38484848485 3.64650982610337e-05
3821.43090909091 3.47378557882919e-05
3896.47696969697 3.31198306849694e-05
3971.52303030303 3.16023896826275e-05
4046.56909090909 3.01777164323574e-05
4121.61515151515 2.88387217459749e-05
4196.66121212121 2.75789650348172e-05
4271.70727272727 2.63925853870252e-05
4346.75333333333 2.52742409632466e-05
4421.79939393939 2.42190555898078e-05
4496.84545454546 2.32225715948118e-05
4571.89151515152 2.22807080720926e-05
4646.93757575758 2.13897238752291e-05
4721.98363636364 2.05461847426933e-05
4797.0296969697 1.97469340388092e-05
4872.07575757576 1.89890666660709e-05
4947.12181818182 1.8269905764614e-05
5022.16787878788 1.75869818659648e-05
5097.21393939394 1.69380142120492e-05
5172.26 1.63208939879861e-05
5247.30606060606 1.57336692494166e-05
5322.35212121212 1.51745313528374e-05
5397.39818181818 1.46418027212986e-05
5472.44424242424 1.41339257984621e-05
5547.4903030303 1.3649453061884e-05
5622.53636363636 1.31870379818742e-05
5697.58242424242 1.2745426825751e-05
5772.62848484848 1.23234512190284e-05
5847.67454545455 1.19200213852963e-05
5922.72060606061 1.15341199954871e-05
5997.76666666667 1.1164796565038e-05
6072.81272727273 1.08111623443141e-05
6147.85878787879 1.04723856536745e-05
6222.90484848485 1.0147687619861e-05
6297.95090909091 9.83633827504848e-06
6372.99696969697 9.53765298401601e-06
6448.04303030303 9.25098916853041e-06
6523.08909090909 8.97574330125288e-06
6598.13515151515 8.71134814433109e-06
6673.18121212121 8.45727021036785e-06
6748.22727272727 8.21300742570822e-06
6823.27333333333 7.97808697798452e-06
6898.31939393939 7.75206333164318e-06
6973.36545454545 7.53451639676642e-06
7048.41151515152 7.32504983792122e-06
7123.45757575758 7.12328951103846e-06
7198.50363636364 6.92888201746202e-06
7273.5496969697 6.74149336532551e-06
7348.59575757576 6.56080772932964e-06
7423.64181818182 6.38652630081431e-06
7498.68787878788 6.21836622075785e-06
7573.73393939394 6.05605958900093e-06
7648.78 5.89935254359227e-06
};
\addplot [very thick, cadetblue80178158]
table {%
238.86 0.0371374481061499
277.192121212121 0.0322000316184874
315.524242424242 0.0282624616721036
353.856363636364 0.0250580922872224
392.188484848485 0.0224064835106428
430.520606060606 0.0201812887720372
468.852727272727 0.0182914747845647
507.184848484848 0.016669844278446
545.51696969697 0.0152657537975013
583.849090909091 0.0140403420348959
622.181212121212 0.0129633147503883
660.513333333333 0.0120107250241012
698.845454545454 0.0111634074274614
737.177575757576 0.0104058522094566
775.509696969697 0.00972538193957077
813.841818181818 0.00911154005704565
852.173939393939 0.00855563045879386
890.506060606061 0.00805036643012686
928.838181818182 0.00758959986164248
967.170303030303 0.00716811018461701
1005.50242424242 0.00678143825649987
1043.83454545455 0.00642575445201471
1082.16666666667 0.00609775304768537
1120.49878787879 0.00579456700770791
1158.83090909091 0.00551369873762725
1197.16303030303 0.00525296343738564
1235.49515151515 0.00501044247138204
1273.82727272727 0.00478444475907143
1312.15939393939 0.0045734746303699
1350.49151515152 0.00437620492455909
1388.82363636364 0.00419145436721583
1427.15575757576 0.0040181684569062
1465.48787878788 0.00385540324650919
1503.82 0.00370231152374397
1542.15212121212 0.0035581309896647
1580.48424242424 0.00342217410845265
1618.81636363636 0.00329381936120919
1657.14848484848 0.00317250368399148
1695.48060606061 0.00305771590859552
1733.81272727273 0.00294899105554222
1772.14484848485 0.00284590535387844
1810.47696969697 0.00274807188294508
1848.80909090909 0.00265513674810783
1887.14121212121 0.00256677571631694
1925.47333333333 0.0024826912488297
1963.80545454545 0.00240260987794709
2002.13757575758 0.00232627988254352
2040.4696969697 0.00225346922379642
2078.80181818182 0.0021839637080805
2117.13393939394 0.00211756534866958
2155.46606060606 0.00205409090183766
2193.79818181818 0.00199337055629402
2232.1303030303 0.00193524675772654
2270.46242424242 0.00187957315264525
2308.79454545455 0.00182621363778243
2347.12666666667 0.00177504150307335
2385.45878787879 0.00172593865775849
2423.79090909091 0.00167879493045382
2462.12303030303 0.00163350743516096
2500.45515151515 0.00158997999616274
2538.78727272727 0.00154812262559225
2577.11939393939 0.00150785104819604
2615.45151515152 0.0014690862684486
2653.78363636364 0.00143175417573071
2692.11575757576 0.00139578518376931
2730.44787878788 0.00136111390096089
2768.78 0.00132767882857287
2807.11212121212 0.00129542208414423
2845.44424242424 0.00126428914769447
2883.77636363636 0.0012342286286035
2922.10848484848 0.00120519205124912
2960.44060606061 0.00117713365768683
2998.77272727273 0.00115001022583179
3037.10484848485 0.00112378090175885
3075.43696969697 0.0010984070448744
3113.76909090909 0.00107385208483706
3152.10121212121 0.00105008138921367
3190.43333333333 0.00102706214095502
3228.76545454545 0.00100476322486284
3267.09757575758 0.000983155122298061
3305.4296969697 0.000962209813450126
3343.76181818182 0.000941900686550061
3382.09393939394 0.00092220245346633
3420.42606060606 0.000903091071173305
3458.75818181818 0.000884543668627683
3497.0903030303 0.000866538478629445
3535.42242424242 0.000849054774280971
3573.75454545455 0.000832072809691459
3612.08666666667 0.000815573764604143
3650.41878787879 0.000799539692651157
3688.75090909091 0.000783953472965809
3727.08303030303 0.000768798764904497
3765.41515151515 0.000754059965651053
3803.74727272727 0.000739722170494791
3842.07939393939 0.000725771135590503
3880.41151515151 0.000712193243024061
3918.74363636364 0.000698975468021236
3957.07575757576 0.00068610534815025
3995.40787878788 0.000673570954380143
4033.74 0.000661360863867796
};
\addplot [very thick, chocolate21910927]
table {%
21.9 1.0078570427758
98.3654545454546 0.2191050322673
174.830909090909 0.103686045815564
251.296363636364 0.0617251706835256
327.761818181818 0.0412646564516899
404.227272727273 0.0296207811034494
480.692727272727 0.0223193659311728
557.158181818182 0.0174232049026206
633.623636363636 0.0139736957749938
710.089090909091 0.0114492767714463
786.554545454546 0.00954521391587949
863.02 0.00807326725451775
939.485454545455 0.00691183157566669
1015.95090909091 0.00597939843250849
1092.41636363636 0.00521962002514998
1168.88181818182 0.00459250384210468
1245.34727272727 0.00406901417330281
1321.81272727273 0.00362764933933606
1398.27818181818 0.0032522074678756
1474.74363636364 0.00293029043161332
1551.20909090909 0.00265227924085705
1627.67454545455 0.00241061810260261
1704.14 0.0021993050831932
1780.60545454545 0.00201352383119329
1857.07090909091 0.00184937335174151
1933.53636363636 0.00170366705468494
2010.00181818182 0.00157378147649931
2086.46727272727 0.00145754110887291
2162.93272727273 0.00135312980232053
2239.39818181818 0.00125902195620536
2315.86363636364 0.00117392859876608
2392.32909090909 0.00109675478400001
2468.79454545455 0.00102656566940986
2545.26 0.000962559310194387
2621.72545454545 0.000904044692029398
2698.19090909091 0.000850423880746343
2774.65636363636 0.00080117743043952
2851.12181818182 0.000755852387835003
2927.58727272727 0.000714052378396769
3004.05272727273 0.000675429371582583
3080.51818181818 0.000639676808172313
3156.98363636364 0.000606523838382434
3233.44909090909 0.000575730470443258
3309.91454545455 0.000547083469046607
3386.38 0.000520392874236015
3462.84545454545 0.000495489035898439
3539.31090909091 0.000472220078521697
3615.77636363636 0.000450449726437509
3692.24181818182 0.000430055432238308
3768.70727272727 0.000410926761097904
3845.17272727273 0.000392963991851128
3921.63818181818 0.000376076902290521
3998.10363636364 0.000360183711527083
4074.56909090909 0.000345210156677772
4151.03454545454 0.000331088684775047
4227.5 0.000317757743793077
4303.96545454545 0.000305161159170793
4380.43090909091 0.000293247584278782
4456.89636363636 0.000281970015001416
4533.36181818182 0.000271285360048972
4609.82727272727 0.000261154059826313
4686.29272727273 0.000251539747705227
4762.75818181818 0.000242408948409414
4839.22363636364 0.000233730808951008
4915.68909090909 0.000225476858177422
4992.15454545454 0.000217620791515058
5068.62 0.000210138277946928
5145.08545454545 0.000203006786646667
5221.55090909091 0.000196205431022106
5298.01636363636 0.000189714828205715
5374.48181818182 0.000183516972274177
5450.94727272727 0.000177595119690793
5527.41272727273 0.000171933685647355
5603.87818181818 0.000166518150140791
5680.34363636364 0.000161334972757693
5756.80909090909 0.000156371515259816
5833.27454545455 0.000151615971168234
5909.74 0.000147057301635264
5986.20545454545 0.000142685176973253
6062.67090909091 0.000138489923279466
6139.13636363636 0.000134462473657898
6215.60181818182 0.000130594323593043
6292.06727272727 0.000126877490078347
6368.53272727273 0.000123304474144248
6444.99818181818 0.000119868226467895
6521.46363636364 0.00011656211577962
6597.92909090909 0.000113379899810427
6674.39454545455 0.000110315698550695
6750.86 0.000107363969613341
6827.32545454545 0.000104519485515184
6903.79090909091 0.000101777312708554
6980.25636363636 9.91327922114865e-05
7056.72181818182 9.65815216994116e-05
7133.18727272727 9.41193389343082e-05
7209.65272727273 9.17423064189557e-05
7286.11818181818 8.94466971743869e-05
7362.58363636364 8.72289815480577e-05
7439.04909090909 8.50858149686914e-05
7515.51454545455 8.30140265713605e-05
7591.98 8.10106086232193e-05
};
\addplot [very thick, purple11522131]
table {%
78.58 0.326366197778146
136.019797979798 0.114904585930215
193.459595959596 0.0591928259361639
250.899393939394 0.0364060990579827
308.339191919192 0.0248142212219854
365.77898989899 0.0180866836016719
423.218787878788 0.013820663503719
480.658585858586 0.010937541390112
538.098383838384 0.00889305587153157
595.538181818182 0.00738774147931236
652.97797979798 0.0062454354965921
710.417777777778 0.0053568423572965
767.857575757576 0.00465114148972796
825.297373737374 0.00408075383888628
882.737171717172 0.00361272262496554
940.17696969697 0.00322361392283262
997.616767676768 0.00289638266952223
1055.05656565657 0.00261838226659018
1112.49636363636 0.0023800637364572
1169.93616161616 0.0021741038286741
1227.37595959596 0.00199480740712344
1284.81575757576 0.00183768956365928
1342.25555555556 0.00169917810852568
1399.69535353535 0.00157639829311947
1457.13515151515 0.00146701472036622
1514.57494949495 0.00136911367741607
1572.01474747475 0.00128111446795355
1629.45454545455 0.00120170183479506
1686.89434343434 0.00112977391434277
1744.33414141414 0.00106440176281152
1801.77393939394 0.0010047975969685
1859.21373737374 0.000950289663494821
1916.65353535354 0.000900302197488431
1974.09333333333 0.000854339322275723
2031.53313131313 0.000811972026526085
2088.97292929293 0.000772827562481692
2146.41272727273 0.000736580762756145
2203.85252525253 0.000702946887778833
2261.29232323232 0.000671675702209853
2318.73212121212 0.000642546544072073
2376.17191919192 0.000615364200350834
2433.61171717172 0.000589955441307265
2491.05151515152 0.000566166095590236
2548.49131313131 0.000543858571511084
2605.93111111111 0.000522909748119033
2663.37090909091 0.00050320917414397
2720.81070707071 0.000484657524329757
2778.25050505051 0.000467165271826443
2835.6903030303 0.000450651542646948
2893.1301010101 0.000435043124109204
2950.5698989899 0.000420273603976131
3008.0096969697 0.000406282620903847
3065.44949494949 0.000393015209993712
3122.88929292929 0.000380421229856704
3180.32909090909 0.000368454859750987
3237.76888888889 0.000357074157132807
3295.20868686869 0.000346240667437425
3352.64848484848 0.000335919079136169
3410.08828282828 0.000326076918142894
3467.52808080808 0.000316684276504141
3524.96787878788 0.000307713571031175
3582.40767676768 0.000299139328142719
3639.84747474747 0.000290937991703576
3697.28727272727 0.000283087751082422
3754.72707070707 0.000275568387024628
3812.16686868687 0.000268361133253742
3869.60666666667 0.000261448551986861
3927.04646464646 0.000254814421782037
3984.48626262626 0.000248443636335862
4041.92606060606 0.000242322113021638
4099.36585858586 0.000236436710107235
4156.80565656566 0.000230775151720356
4214.24545454545 0.000225325959740368
4271.68525252525 0.000220078391892723
4329.12505050505 0.000215022385406243
4386.56484848485 0.000210148505667059
4444.00464646465 0.000205447899367154
4501.44444444444 0.000200912251701726
4558.88424242424 0.000196533747218818
4616.32404040404 0.000192305033967953
4673.76383838384 0.000188219190632639
4731.20363636364 0.000184269696365136
4788.64343434343 0.000180450403071528
4846.08323232323 0.000176755509921354
4903.52303030303 0.000173179539879235
4960.96282828283 0.000169717318076524
5018.40262626263 0.000166363951859274
5075.84242424242 0.000163114812365074
5133.28222222222 0.000159965517495777
5190.72202020202 0.000156911916166062
5248.16181818182 0.000153950073719282
5305.60161616162 0.000151076258412391
5363.04141414141 0.000148286928880929
5420.48121212121 0.000145578722503368
5477.92101010101 0.000142948444591506
5535.36080808081 0.000140393058340296
5592.80060606061 0.000137909675476477
5650.2404040404 0.000135495547550813
5707.6802020202 0.000133148057823578
5765.12 0.000130864713697377
};
\addplot [very thick, black18]
table {%
21.92 0.745760476176531
103.034747474747 0.0396785097882239
184.149494949495 0.0131675798439805
265.264242424242 0.00657838032881512
346.37898989899 0.0039596624681078
427.493737373737 0.00265287832767291
508.608484848485 0.00190560684885747
589.723232323232 0.00143752957030421
670.83797979798 0.00112453234414446
751.952727272727 0.000904673723834232
833.067474747475 0.000744186137994275
914.182222222222 0.000623365086806442
995.29696969697 0.000530073088147395
1076.41171717172 0.000456496647610199
1157.52646464646 0.000397417990058547
1238.64121212121 0.000349243109653531
1319.75595959596 0.000309429904353558
1400.87070707071 0.000276138506884105
1481.98545454545 0.000248010261143613
1563.1002020202 0.00022402391152576
1644.21494949495 0.000203399617598049
1725.3296969697 0.000185533425780117
1806.44444444444 0.000169951621978594
1887.55919191919 0.000156278351538785
1968.67393939394 0.000144212270889631
2049.78868686869 0.00013350945923178
2130.90343434343 0.00012397074086221
2212.01818181818 0.000115432161973327
2293.13292929293 0.000107757754721406
2374.24767676768 0.00010083398086952
2455.36242424242 9.45654232577453e-05
2536.47717171717 8.88714144270448e-05
2617.59191919192 8.36833761880114e-05
2698.70666666667 7.89427036065277e-05
2779.82141414141 7.45990695508014e-05
2860.93616161616 7.06090567951744e-05
2942.05090909091 6.69350472127221e-05
3023.16565656566 6.35443142123843e-05
3104.2804040404 6.04082769509944e-05
3185.39515151515 5.75018841416809e-05
3266.5098989899 5.48031023128173e-05
3347.62464646465 5.22924887358506e-05
3428.73939393939 4.99528333615831e-05
3509.85414141414 4.77688572925796e-05
3590.96888888889 4.57269578017693e-05
3672.08363636364 4.38149918521857e-05
3753.19838383838 4.20220916055569e-05
3834.31313131313 4.03385066222236e-05
3915.42787878788 3.87554684227797e-05
3996.54262626263 3.72650738570099e-05
4077.65737373737 3.58601843495409e-05
4158.77212121212 3.45343385960646e-05
4239.88686868687 3.3281676693667e-05
4321.00161616162 3.20968740229782e-05
4402.11636363636 3.09750834735637e-05
4483.23111111111 2.99118848290421e-05
4564.34585858586 2.89032403141849e-05
4645.46060606061 2.79454554601615e-05
4726.57535353535 2.7035144572035e-05
4807.6901010101 2.6169200189352e-05
4888.80484848485 2.53447660199906e-05
4969.9195959596 2.45592129024252e-05
5051.03434343434 2.38101174147204e-05
5132.14909090909 2.30952428018988e-05
5213.26383838384 2.24125219385089e-05
5294.37858585859 2.176004208158e-05
5375.49333333333 2.1136031201831e-05
5456.60808080808 2.05388457088884e-05
5537.72282828283 1.99669594101456e-05
5618.83757575758 1.94189535633787e-05
5699.95232323232 1.88935079008466e-05
5781.06707070707 1.83893925177871e-05
5862.18181818182 1.79054605313322e-05
5943.29656565657 1.74406414272193e-05
6024.41131313131 1.69939350215239e-05
6105.52606060606 1.65644059731943e-05
6186.64080808081 1.61511787906279e-05
6267.75555555556 1.57534332820286e-05
6348.8703030303 1.53704004049755e-05
6429.98505050505 1.50013584756058e-05
6511.0997979798 1.46456297021903e-05
6592.21454545455 1.43025770117142e-05
6673.32929292929 1.39716011414551e-05
6754.44404040404 1.36521379705332e-05
6835.55878787879 1.33436560690349e-05
6916.67353535354 1.30456544446416e-05
6997.78828282828 1.27576604687547e-05
7078.90303030303 1.24792279659375e-05
7160.01777777778 1.22099354521176e-05
7241.13252525253 1.19493845084396e-05
7322.24727272727 1.16971982789449e-05
7403.36202020202 1.14530200814023e-05
7484.47676767677 1.12165121216403e-05
7565.59151515152 1.0987354302648e-05
7646.70626262626 1.07652431205334e-05
7727.82101010101 1.05498906401621e-05
7808.93575757576 1.03410235439647e-05
7890.05050505051 1.01383822479887e-05
7971.16525252525 9.94172007981098e-06
8052.28 9.75080251340353e-06
};
\addplot [very thick, darkgray153]
table {%
21.92 0.146882334693568
106.212121212121 0.0377570359541847
190.504242424242 0.0200592911062981
274.796363636364 0.0130185398513157
359.088484848485 0.00933038108310853
443.380606060606 0.00710217672212892
527.672727272727 0.00563105011777276
611.964848484849 0.00459866148198295
696.25696969697 0.0038410397551521
780.549090909091 0.00326567873615227
864.841212121212 0.00281670977415752
949.133333333333 0.00245855148174466
1033.42545454545 0.00216755632676998
1117.71757575758 0.00192744805358024
1202.0096969697 0.00172669077855243
1286.30181818182 0.00155690216059791
1370.59393939394 0.00141185928744008
1454.88606060606 0.00128685532432443
1539.17818181818 0.00117827128172234
1623.4703030303 0.00108328386698797
1707.76242424242 0.000999661795557557
1792.05454545455 0.000925621004275404
1876.34666666667 0.000859719935773945
1960.63878787879 0.000800782612761184
2044.93090909091 0.000747841322656307
2129.22303030303 0.000700093360298846
2213.51515151515 0.000656867994244165
2297.80727272727 0.000617600966444292
2382.09939393939 0.000581814610475548
2466.39151515152 0.000549102207140356
2550.68363636364 0.0005191155689123
2634.97575757576 0.000491555108385211
2719.26787878788 0.000466161834799995
2803.56 0.000442710859625239
2887.85212121212 0.000421006092445482
2972.14424242424 0.000400875882600225
3056.43636363636 0.000382169417420798
3140.72848484849 0.000364753729652821
3225.02060606061 0.000348511198359764
3309.31272727273 0.000333337451877758
3393.60484848485 0.000319139600113109
3477.89696969697 0.000305834738012905
3562.18909090909 0.000293348673404707
3646.48121212121 0.000281614841341781
3730.77333333333 0.000270573374164977
3815.06545454545 0.00026017030212218
3899.35757575758 0.000250356863890503
3983.6496969697 0.000241088909968521
4067.94181818182 0.000232326384832949
4152.23393939394 0.000224032876130579
4236.52606060606 0.000216175221114376
4320.81818181818 0.00020872316211988
4405.1103030303 0.00020164904418341
4489.40242424242 0.000194927548981252
4573.69454545455 0.00018853546016215
4657.98666666667 0.000182451455888239
4742.27878787879 0.000176655925019595
4826.57090909091 0.000171130803896768
4910.86303030303 0.000165859431111928
4995.15515151515 0.000160826418026858
5079.44727272727 0.000156017533106831
5163.73939393939 0.000151419598402851
5248.03151515152 0.000147020396738711
5332.32363636364 0.000142808588350249
5416.61575757576 0.00013877363588737
5500.90787878788 0.000134905736829186
5585.2 0.000131195762482762
5669.49212121212 0.000127635202839294
5753.78424242424 0.000124216116650817
5838.07636363636 0.000120931086167679
5922.36848484849 0.000117773176043897
6006.66060606061 0.000114735895975618
6090.95272727273 0.00011181316668845
6175.24484848485 0.000108999288933521
6259.53696969697 0.000106288915190644
6343.82909090909 0.000103677023810684
6428.12121212121 0.00010115889535878
6512.41333333333 9.87300909460752e-05
6596.70545454545 9.63864323604363e-05
6680.99757575758 9.41239838268101e-05
6765.2896969697 9.19390352456533e-05
6849.58181818182 8.98280867735871e-05
6933.87393939394 8.77878346243787e-05
7018.16606060606 8.58151579806953e-05
7102.45818181818 8.39071069180599e-05
7186.7503030303 8.20608912521999e-05
7271.04242424243 8.02738702296829e-05
7355.33454545455 7.85435429894816e-05
7439.62666666667 7.68675397300619e-05
7523.91878787879 7.52436135227612e-05
7608.21090909091 7.36696327177978e-05
7692.50303030303 7.21435738942155e-05
7776.79515151515 7.06635153095421e-05
7861.08727272727 6.92276308089551e-05
7945.37939393939 6.78341841573622e-05
8029.67151515152 6.64815237610577e-05
8113.96363636364 6.51680777485568e-05
8198.25575757576 6.38923493828534e-05
8282.54787878788 6.26529127797503e-05
8366.84 6.14484089090734e-05
};
\addplot [very thick, saddlebrown1356716]
table {%
351.36 0.0117766429172202
438.460202020202 0.00759317722857615
525.560404040404 0.00534467657548856
612.660606060606 0.00399283315853852
699.760808080808 0.0031138673038541
786.86101010101 0.00250835558681953
873.961212121212 0.00207228392125772
961.061414141414 0.00174699816463692
1048.16161616162 0.00149733157455739
1135.26181818182 0.00130112997170669
1222.36202020202 0.00114385562728247
1309.46222222222 0.00101563666890812
1396.56242424242 0.000909571492959973
1483.66262626263 0.000820712494640504
1570.76282828283 0.0007454345515208
1657.86303030303 0.000681030097843669
1744.96323232323 0.000625442255920725
1832.06343434343 0.000577084632466934
1919.16363636364 0.000534716977044624
2006.26383838384 0.000497357707942642
2093.36404040404 0.000464221290771711
2180.46424242424 0.000434672694280994
2267.56444444444 0.000408193786183473
2354.66464646465 0.000384358210432917
2441.76484848485 0.0003628123771948
2528.86505050505 0.000343260917409352
2615.96525252525 0.000325455438518883
2703.06545454545 0.000309185749012658
2790.16565656566 0.000294272948883233
2877.26585858586 0.000280563944227881
2964.36606060606 0.000267927058812611
3051.46626262626 0.000256248497843141
3138.56646464646 0.000245429479125909
3225.66666666667 0.000235383890831687
3312.76686868687 0.000226036367726144
3399.86707070707 0.000217320702163003
3486.96727272727 0.00020917852457072
3574.06747474747 0.000201558202185111
3661.16767676768 0.000194413915525348
3748.26787878788 0.000187704880403681
3835.36808080808 0.000181394689702836
3922.46828282828 0.000175450754194008
4009.56848484848 0.000169843825632886
4096.66868686869 0.000164547588508399
4183.76888888889 0.000159538309315351
4270.86909090909 0.000154794534219063
4357.96929292929 0.000150296827585636
4445.06949494949 0.00014602754514845
4532.1696969697 0.000141970636634117
4619.2698989899 0.000138111473529149
4706.3701010101 0.000134436698371001
4793.4703030303 0.000130934092524507
4880.5705050505 0.000127592459881108
4967.67070707071 0.000124401524312868
5054.77090909091 0.00012135183904126
5141.87111111111 0.000118434706354287
5228.97131313131 0.000115642106334517
5316.07151515152 0.000112966633452819
5403.17171717172 0.000110401440044569
5490.27191919192 0.000107940185821862
5577.37212121212 0.000105576992691159
5664.47232323232 0.000103306404244295
5751.57252525252 0.000101123349374641
5838.67272727273 9.90231095418648e-05
5925.77292929293 9.70012892701154e-05
6012.87313131313 9.5053789517094e-05
6099.97333333333 9.31767835968373e-05
6187.07353535353 9.13666953780909e-05
6274.17373737374 8.96201795139762e-05
6361.27393939394 8.79341034878873e-05
6448.37414141414 8.63055312860079e-05
6535.47434343434 8.47317085289062e-05
6622.57454545454 8.32100489139492e-05
6709.67474747475 8.17381218371129e-05
6796.77494949495 8.03136410774687e-05
6883.87515151515 7.89344544405432e-05
6970.97535353535 7.75985342680805e-05
7058.07555555556 7.63039687317036e-05
7145.17575757576 7.50489538367524e-05
7232.27595959596 7.38317860703345e-05
7319.37616161616 7.2650855634471e-05
7406.47636363636 7.15046402112988e-05
7493.57656565657 7.03916992126557e-05
7580.67676767677 6.93106684711703e-05
7667.77696969697 6.82602553342137e-05
7754.87717171717 6.72392341258675e-05
7841.97737373737 6.62464419454257e-05
7929.07757575758 6.52807747739762e-05
8016.17777777778 6.43411838632886e-05
8103.27797979798 6.34266723836653e-05
8190.37818181818 6.25362923095585e-05
8277.47838383838 6.16691415237157e-05
8364.57858585859 6.082436112235e-05
8451.67878787879 6.00011329054048e-05
8538.77898989899 5.91986770374028e-05
8625.87919191919 5.84162498656374e-05
8712.97939393939 5.76531418836209e-05
8800.0795959596 5.69086758287461e-05
8887.1797979798 5.61822049040548e-05
8974.28 5.54731111148661e-05
};
\addplot [draw=black, fill=black, mark=x, very thick, mark size=2.5pt, only marks]
table{%
x  y
87.6 0.272343533408822
351.36 0.0259470568426133
1450.24 0.00189066552594397
5765.12 0.000144604747120979
};

==> figures/quantitative_results/group_main_2.tex <==
\nextgroupplot[
ylabel shift = -0.2cm,
clip marker paths=true,
width=0.52\textwidth,
title style={yshift=-0.2cm},
height=4.5cm,
scaled x ticks=false,
legend cell align={left},
log basis y={10},
tick align=outside,
tick pos=left,
title={Stokes Flow},
x grid style={darkgray176},
xlabel={\empty},
xmajorgrids,
xmin=-463.591, xmax=10471.751,
xtick style={color=black},
xtick={-2000,0,2000,4000,6000,8000,10000,12000},
xticklabels={-2.0,0.0,2.0,4.0,6.0,8.0,10.0},
y grid style={darkgray176},
ylabel={\empty},
ymajorgrids,
ymin=1.6e-06, ymax=5.80121683938417,
ymode=log,
ytick style={color=black},
ytick={1e-07,1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
}
]
\addplot [
  draw=royalblue28108204,
  fill=royalblue28108204,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
33.32 0.99999999993243
64.9 0.666977763968923
66.08 0.635200308961035
86.82 0.517850176002978
88.82 0.374976579489248
98.84 0.419507290728568
100.74 0.279794211912164
110.28 0.243180058293518
120.82 0.249052559613513
137.86 0.243830183923945
167.38 0.11497313665077
184.02 0.0946478603008035
185.58 0.0766329151425849
186.94 0.0929574456978693
190.78 0.0928610183064781
207.42 0.07650488298002
215.92 0.068450159279531
219.8 0.0560930488663731
251.92 0.0540741113459127
260.34 0.0657158980558838
427.86 0.0212762898323966
466.72 0.0130220571261205
472.4 0.0134263055355547
507.38 0.0118937963113513
519.02 0.0102284857447289
532.12 0.0102964907150482
532.9 0.0101877977372454
569.64 0.00899852770935653
575.98 0.00936246157546711
629.26 0.00728486705853312
709.08 0.00546556138663469
747.88 0.0053858701353386
757.34 0.00517595114103844
788.02 0.00526634888305671
810.34 0.00326217110482706
813.78 0.00503419851874908
826.26 0.00400798192190147
856.96 0.00358552537667551
884.22 0.00265400082500551
963.38 0.00442710897670244
1233.04 0.00174160115323288
1292.8 0.00147386576335486
1335.42 0.00150782761627882
1390.92 0.00153955451941804
1414.88 0.00165781005470579
1425.28 0.00161784481214953
1513.66 0.00134093644849511
1518.08 0.000905956289642722
1578.84 0.00183265743602863
1666.52 0.000993603798976317
1674.04 0.00137677609884964
1744.74 0.00106324857350244
1775.28 0.000956593881169706
1819.24 0.000987741614176905
1976.62 0.000626792409374693
2007.8 0.000646910688078179
2032.16 0.000708539458630236
2037.08 0.000789949816186746
2072.84 0.000585065700614331
2420.6 0.000514173066155448
2546.62 0.000438594430440026
2592.16 0.0003985628063108
2690.38 0.00024446744319101
2778.42 0.000413080672833224
2806.2 0.000550928473237413
2862.56 0.000401828653959693
2927.6 0.000394520567224911
3099.48 0.000313141998401
3120.06 0.000427384119284796
3134.84 0.000387849077907572
3188.04 0.000269625693669212
3253.92 0.000330992400317024
3401 0.000179500515022188
3698.88 0.000221601338241685
3815.3 0.000273886276260763
3967.28 0.000182777868137399
4027.8 0.000215647442748303
4041.24 0.000215334856108229
4088.78 0.000253184382417688
4283.88 0.000156779332946312
4334.78 0.000101470637991631
4490.02 0.000140981656240678
4553.96 0.000128797870552244
4634.76 0.000160459649939724
4664.26 0.000157204988142736
4691.68 0.000135168479899333
4745.78 0.000183694640674875
5283.58 0.00013790216724299
5330.02 0.000123822546176216
5596.48 0.000110367045701949
5686.98 0.000162465875179084
5827.46 0.000102794190697769
5963.04 0.000112108412701103
6018.3 0.000125814871796998
6392.58 8.76255905610294e-05
6612.14 8.41482690310943e-05
6686.74 0.000109614484982677
6815.02 9.70545732143426e-05
7603.3 9.32092866335062e-05
8624.18 7.17550805847686e-05
};
\addplot [
  draw=cadetblue80178158,
  fill=cadetblue80178158,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
212.68 0.141161309802721
218.24 0.144914823313613
220.12 0.147405079531887
220.52 0.158061864430087
222.1 0.117502378723376
222.62 0.133136382836979
223.04 0.119809397658282
225.28 0.119547987583072
233.54 0.103147040665571
262.02 0.0921593777876243
419.58 0.0460017634615905
425.4 0.0566215115298248
427.24 0.189244844249684
440.98 0.162638757314811
456.28 0.0631301851594839
462.02 0.366735353099643
492.06 0.303222072976536
502.84 0.278588033564185
511.06 0.184332007876049
518.4 0.232980827002057
582.66 0.0245080214799082
623.64 0.0234765069990089
628.62 0.0427675190302023
647.2 0.0646323016394516
664 0.222878989655775
682.3 0.0610732136611745
709.6 0.296444103050641
716.58 0.225083949729485
787.18 0.256662099711898
790.84 0.452856310323446
818.74 0.022773667002188
845.24 0.0644229837888212
847.54 0.0332041144464586
849.12 0.0145686045584429
916.64 0.0104885251147687
937.96 0.0571041540851467
947.9 0.150981578406017
1061.78 0.700002064986374
1063.68 0.058991176490658
1087.26 0.036662605022818
1100.96 0.0183468121189743
1156.92 0.0464715741889192
1239.62 0.145144551287296
1252.92 0.0079276267353224
1269.14 0.00413753215053044
1376.1 0.0147251108931351
1411.18 0.10841606440662
1424.64 0.0366291314578664
1438.98 0.00622947520037921
1452.16 0.411294646243272
1452.44 0.124578651637079
1458.8 0.402330578273486
1607.56 0.00579692736360486
1616.8 0.0820078220204681
1621.56 0.52942580770408
1639.24 0.0205394419165977
1735.2 0.295558506925669
1758.82 0.0602288299047352
1771.24 0.00100300859378613
1801.62 0.298550585837659
1812.46 0.0822073926510049
1822.96 0.041553919091109
1857.78 0.0453364142322788
1913.24 0.00455953226803892
2053.8 0.0233983625241656
2135.74 0.101942194667086
2138.84 0.00118478162779771
2349.72 0.364609281878828
2507.18 0.00345491140031748
2517.24 0.0068287498277297
2565.7 0.131433956485401
2622.9 0.0359205833833174
2651.84 0.12185068709643
2692.4 0.0179082220300424
2706 0.015158070787432
2726.54 0.0190407815835674
2746.36 0.00614311437348769
2801.46 0.536544199018495
2848.5 0.00128053699013464
2968.5 0.000655036679913426
3023.1 0.00319857229097586
3035.96 0.00523747686235817
3084.34 0.0386938308392024
3136.68 0.144692655509973
3139.64 0.0272173407579503
3169.78 0.000292743031407813
3239.72 0.00193097325175942
3376.8 0.000229122018758869
3417 0.051366534348802
3470.76 0.000467737703506004
3504.94 0.492913084536132
3590.8 0.00019734471181974
3763.24 0.27880162805468
4047.24 0.0576008833654537
};
\addplot [
  draw=chocolate21910927,
  fill=chocolate21910927,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
33.32 0.99999999993243
40.48 0.965026660037682
42.76 0.927491937833549
57.16 0.855340330354061
88.68 0.398857170963125
92.7 0.402209678100435
96.72 0.341617217820627
96.98 0.341606924700947
97.4 0.841841290211218
99.2 0.322377675509229
100.42 0.644159334119353
102.44 0.358841948566543
108.04 0.358083796411934
111.1 0.349488113658497
111.2 0.294633260491426
115.12 0.556853454084594
117 0.379644807172639
120.18 0.230223720810367
126.88 0.179502399534121
128.66 0.299068890377258
134.56 0.146292186050167
138.24 0.281426849299568
142.76 0.408181793517418
152.82 0.234021272354643
155.92 0.280277334774423
157.18 0.260915633242948
157.4 0.15456448994111
177.22 0.155770375358357
197.28 0.171838842129486
214.06 0.288282246059032
284.88 0.0928807224280245
295.08 0.334969992123274
313.4 0.0813321575443725
322.44 0.0353386623557122
343.26 0.504467235757207
387.64 0.0383052425702906
427.44 0.0561068973721813
461.42 0.0280580990740894
496.92 0.0221860864738903
678.86 0.0248145737065543
833.86 0.0447544404722053
958.88 0.0255000019290038
1157.88 0.00971178941375959
1228.78 0.0868704874434512
1442.66 0.0123815482821
1535.24 0.00726870785126631
1585.44 0.00426211569899615
1767.16 0.00249915081250904
1861.8 0.00407641293184567
2397.68 0.217826574613612
2574.16 0.00290985838346044
2737.8 0.00139560855304792
3388.78 0.00104790312301728
3738.8 0.00189051312584091
3868.46 0.125932188948265
4274.82 0.000384193212818031
4671.5 4.62139754350684e-05
6267.68 0.0739536157632153
7211.96 0.000121499627355619
};
\addplot [draw=purple11522131, fill=purple11522131, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
106.14 0.337284022144869
110.6 0.281135081149962
119.66 0.225900456451338
124.44 0.213442048603741
141.32 0.224930233191503
149.2 0.149150093593963
152.4 0.138972023813627
154.98 0.14949004184497
162.92 0.125852140035756
164.1 0.104814047072827
169.62 0.119526397438051
170.8 0.142223380037791
177.48 0.10586498636639
181.82 0.0973710551381316
203.78 0.0813590209840755
268.18 0.0632902308317845
297.94 0.0710874498188464
314.22 0.0694828135326359
369.7 0.066397149894993
384.26 0.0429109465004642
395.04 0.0386218974176012
431.14 0.0556176911830775
447.24 0.0236859109934983
455.68 0.0228362043922797
495.54 0.0194411115974153
529.54 0.0187138347848624
537.8 0.0186796942755036
538.16 0.018679054051407
538.2 0.0186737146248341
538.46 0.0186739357788629
538.84 0.0186743133178174
538.86 0.0186747221465037
539.08 0.0186742107425926
539.48 0.0186739443331654
539.66 0.0186734957811141
539.76 0.0186735194602359
539.84 0.0186736271050766
539.84 0.0186736271050766
539.84 0.0186736271050766
539.84 0.0186736271050766
2032.14 0.00268575018899509
2077.06 0.00271381606374106
2130.52 0.00257297133587573
2137.96 0.00257080291138441
2141.52 0.00257017694555869
2142.48 0.00257017472715489
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2142.72 0.00257009146393778
2149.86 0.00245793628686584
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2168.32 0.00236342113728311
2216.06 0.00237468107403588
8224.54 0.000344086283845686
8356.84 0.000344113207047856
8465.24 0.000345146026413259
8522.18 0.000344014526916937
8535.94 0.000339333984000819
8538.68 0.000339273307889225
8542.56 0.000339260873381374
8542.88 0.000339260075007642
8545.28 0.000339260110199661
8545.28 0.00034399845060651
8545.28 0.00034399845060651
8545.28 0.00034399845060651
8545.28 0.00034399845060651
8545.28 0.00034399845060651
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.00034399845060651
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8545.28 0.000339260110199661
8569.92 0.000342394194699086
};
\addplot [draw=black18, fill=black18, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
33.32 0.99999999993243
79.2 0.313290015698351
81.78 0.298510778394713
84.2 0.285567710562864
89.08 0.267723642806768
93.66 0.250886639645568
96.48 0.236336591707205
97.2 0.22726394158047
100.44 0.216161472328285
102.56 0.203605694174568
107.2 0.188605913922366
110.68 0.181819737438348
116.08 0.169716015394027
120.46 0.159775214813491
123.58 0.150149313682023
129.34 0.140751842528456
134.84 0.131304463472635
142.7 0.120431513028771
147.86 0.111674878730031
153.1 0.10081095603898
158.56 0.0917303672094131
164.66 0.0854139987012634
169.26 0.0825254016133525
172.42 0.0772905127673143
181.78 0.0674848297636666
188.38 0.0628287870744633
202.46 0.0574239071343047
209.44 0.0522125428604364
212.5 0.0500676615547574
222.96 0.045622690953337
227.5 0.0446061011853539
234.96 0.0418042268135939
247.42 0.0378246081105872
256.16 0.0333202712141075
274.98 0.0293351904411876
283.44 0.0265466501010813
305.14 0.0233719692102123
316.7 0.0208588289911115
327.26 0.0192995178081072
341.86 0.0175668454408558
354.06 0.0152126388576651
362.9 0.0146456424829107
386.54 0.0127194322112509
411.6 0.0109770514402562
433.32 0.0099877001741897
470.2 0.00845874016260052
491.4 0.00730891299563646
500.86 0.00687391055483915
518.52 0.00632525999454047
543.08 0.00568182575927838
585.66 0.00475785535072724
620.7 0.00429618071528121
678.54 0.00337914433314152
690.88 0.00315244140847832
726.44 0.00281813132392087
754.98 0.00250704397276236
809.32 0.00202764372613981
851.84 0.00179969455400896
918.68 0.00154625268425684
974.4 0.00134877786625103
1066.04 0.00110174792251866
1122.16 0.00096103903476494
1199.82 0.000841799956408325
1290.24 0.000648673210868458
1439.22 0.000509178811531739
1563.34 0.000406915898390704
1710.14 0.000337696923957356
1861.76 0.000255776074191667
1927.68 0.000227018070996779
2099.78 0.000183108176472213
2207.68 0.00014894824129836
2326.82 0.000124810185055736
2681.64 9.27077029431287e-05
2965.38 7.10998809411142e-05
3338.02 5.12677250595534e-05
3840.06 3.5195775618e-05
4007.66 3.08125294200742e-05
4451.04 2.47359285326982e-05
5049.72 2.02187997343735e-05
5630.96 1.80272173928162e-05
5958.3 1.68998440462418e-05
6654.34 1.58023456617402e-05
7013.36 1.5276984591226e-05
7364.78 1.46546723253157e-05
7833.18 1.42468349013418e-05
8285.56 1.37772562606166e-05
8446.2 1.34598778010029e-05
8939.24 1.31128484854949e-05
9656.04 1.28344776008324e-05
};
\addplot [draw=darkgray153, fill=darkgray153, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
33.32 0.99999999993243
105.42 0.247118644458441
114.74 0.214346336393461
122.32 0.191999051567789
130.28 0.170569282186969
141 0.152915432542835
149.94 0.133732557664312
158.82 0.119285811980666
164.54 0.110094615062489
181.56 0.0960143933652425
189.8 0.0837341991581893
204.68 0.0735622848769895
222.56 0.0623756775170083
233.5 0.0564774966326862
245.68 0.0490065693155629
268.72 0.040928122923616
284.92 0.0381651346778226
305.16 0.033556581466464
319.12 0.0289356488412
341.14 0.0249598372323457
365.04 0.0229461277961976
383.26 0.020453203295573
398.6 0.0174657114216166
420.4 0.0154806238098585
450.38 0.0136309607921804
478.76 0.0123072889614865
518.24 0.0100357246317909
535.32 0.00880447168196816
564.4 0.00763253163515431
596.86 0.00618835922164414
621.26 0.00556818778285868
631.84 0.00508169342462315
669.12 0.0045784383822463
686.62 0.0042923083035675
721.26 0.00378321383411664
751.54 0.00340809325348401
770.06 0.00306579057798471
802.96 0.00279510776054876
833.02 0.00248736960613335
878.38 0.00229960032240644
896.08 0.0021393181316482
911.42 0.00199388239048411
939.74 0.00177585108486935
965.92 0.00162495768742985
995.62 0.00143346373622897
1022.3 0.0012710786722768
1051.7 0.00113360634174779
1072.92 0.00107651194224652
1100.34 0.00100074658915409
1122.52 0.000925161658485865
1163.86 0.00085362806010163
1193.62 0.000796740438271907
1243.72 0.000717724491279931
1268.18 0.00068220170509496
1297.74 0.000633521366622839
1340.88 0.000566344023381284
1373.3 0.00053066231925001
1404.74 0.000490827550111423
1417.68 0.000466845179028422
1446.04 0.000441535497544286
1487.98 0.000399932477979647
1519.08 0.000379144055373508
1536.34 0.000356886356104473
1550.64 0.000340295808795138
1599.58 0.000292158702509164
1601.62 0.00031556144741093
1619.52 0.000273364166111787
1656.08 0.000258915783966589
1681 0.000242409098538926
1720.96 0.000227540531757515
1736.88 0.000213958387532877
1766.26 0.000201220285341197
1814.96 0.000192221361894142
1828.36 0.000179527339749031
1901.18 0.000164947610529362
1909.08 0.000154348492045384
1983.74 0.000144951788145188
2002.44 0.000134964748468264
2035.22 0.000123953188081648
2081 0.000113585881170964
2120.34 0.000106077293695542
2204.82 9.97710195436937e-05
2278.48 9.0988860187697e-05
2356.98 8.47715320623551e-05
2446.72 7.84450082905669e-05
2562.48 7.19383961056387e-05
2694.04 6.33995394684987e-05
2871.44 5.65735309842211e-05
3051.64 4.99283479838731e-05
3291.3 4.47288329519996e-05
3558.7 3.79390422489001e-05
3946.26 3.33446895664832e-05
4377.9 2.85833214355245e-05
4983.3 2.44946411141301e-05
5831.32 2.01974279053764e-05
7202.64 1.73921109515726e-05
9090.88 1.47044674093071e-05
};
\addplot [
  draw=saddlebrown1356716,
  fill=saddlebrown1356716,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
539.84 0.0186736271050518
606.24 0.0108608982394807
609.36 0.0103192510037162
627 0.00959776532605086
627.02 0.00922272179804538
636.06 0.00887959315383357
646.84 0.00857724114679822
649.34 0.00834097016503149
664.96 0.00764390199861746
669.56 0.00734001502753147
669.6 0.00672570608167206
685.54 0.00623057814496022
702.04 0.00571177484377207
710.78 0.00540542139776457
731.54 0.00498514606290271
755.16 0.00462073116261687
767.88 0.00427736189161273
776 0.00394429304281944
794.46 0.00369577177389543
821.82 0.00331572250852714
835.58 0.00309849349837278
848.04 0.0029582294522501
862.38 0.00279981849211517
897.06 0.00251169127128743
923.24 0.00232141314530173
939.22 0.00215688235976693
963.24 0.00191343288615196
990.94 0.00181793593939912
995.74 0.00169273133844848
1012.42 0.00162994212882767
1026.72 0.00152739443838268
1058.18 0.00141223421777113
1078.32 0.00132049892457523
1122.68 0.00123666858792669
1141.66 0.00119622429957497
1158.36 0.00112744090915787
1173.6 0.00109588624593356
1202.56 0.00101168268825819
1239.24 0.000953417772767446
1260.36 0.000771744188327509
1295 0.000719214564733268
1329.78 0.000619703362651716
1362.04 0.000562646572637406
1391.54 0.000520259111701669
1469.12 0.000430247253337524
1530.14 0.000382736579815759
1571.34 0.000365815383160123
1638.76 0.000327375100594789
1690.64 0.000280095078731507
1798.9 0.000233918980696023
1874.7 0.000217549892640933
1939.68 0.00020590202404019
2020.44 0.000189820459609546
2086.74 0.000178779664717027
2158.88 0.000165785844331108
2245.28 0.000151008066446839
2330.12 0.000139772655032041
2402.46 0.000131803214853782
2505.84 0.00011884872220902
2605.52 0.000111040989542906
2643.06 0.000101272219826724
2742.84 9.23232728233797e-05
2834.94 8.58167097600741e-05
2961.08 7.86667177472738e-05
3054.5 7.25085626609579e-05
3211.22 6.73766306434927e-05
3316.76 6.42063163255727e-05
3435.96 6.02583007218825e-05
3557.6 5.7147235377696e-05
3648.72 5.44115261332398e-05
3757.34 5.19830284305301e-05
3949.86 4.8903453631002e-05
4091.88 4.64412758603086e-05
4163.8 4.35929660769621e-05
4329.14 4.16935787086509e-05
4465.22 3.95297371769741e-05
4611.84 3.67153648010848e-05
4697.18 3.45008029561099e-05
4936.98 3.32054743027027e-05
5130.08 3.19305906497091e-05
5322.8 3.06152848830235e-05
5408.74 2.94981240680514e-05
5581.26 2.81813484980669e-05
5706.74 2.69032657442365e-05
5940.24 2.54893072167299e-05
6148.92 2.43116624171292e-05
6514.68 2.34311513080224e-05
6639.92 2.24316673533458e-05
6839.06 2.17124867571997e-05
7013.78 2.0979540743764e-05
7455.04 2.03154233694942e-05
7733.12 1.95295056471078e-05
7833.16 1.89199799891612e-05
7902.14 1.83018951184245e-05
8133.78 1.78797734758565e-05
8580.22 1.74748633531429e-05
8771.24 1.70264332707341e-05
9115.82 1.6588698280279e-05
9547.42 1.62730359594875e-05
9829.54 1.59575197631017e-05
};
\addplot [very thick, royalblue28108204]
table {%
33.32 2.79651864210356
120.096363636364 0.202153138651844
206.872727272727 0.0676248443603522
293.649090909091 0.0336053957766751
380.425454545455 0.0201030563272302
467.201818181818 0.0133958732673822
553.978181818182 0.00957942674105368
640.754545454546 0.00719996984999401
727.530909090909 0.00561548697336104
814.307272727273 0.00450659873474778
901.083636363636 0.00369978011616308
987.86 0.00309410740745331
1074.63636363636 0.00262760937239683
1161.41272727273 0.00226050974663374
1248.18909090909 0.00196631937048079
1334.96545454545 0.00172683910238822
1421.74181818182 0.00152922686686916
1508.51818181818 0.0013642085104631
1595.29454545455 0.0012249494402461
1682.07090909091 0.0011063220207642
1768.84727272727 0.00100441759966496
1855.62363636364 0.000916214015549343
1942.4 0.000839344406333196
2029.17636363636 0.000771933497498979
2115.95272727273 0.000712479748100142
2202.72909090909 0.000659769229499975
2289.50545454545 0.000612811827027393
2376.28181818182 0.000570793383076044
2463.05818181818 0.000533039382675547
2549.83454545455 0.000498987103345303
2636.61090909091 0.000468164045267637
2723.38727272727 0.000440171072318944
2810.16363636364 0.00041466912263322
2896.94 0.000391368649502074
2983.71636363636 0.000370021169179388
3070.49272727273 0.000350412447967729
3157.26909090909 0.000332356974654245
3244.04545454545 0.000315693448134751
3330.82181818182 0.000300281072358321
3417.59818181818 0.000285996497448969
3504.37454545455 0.000272731281193565
3591.15090909091 0.00026038977200977
3677.92727272727 0.000248887335174991
3764.70363636364 0.000238148860071327
3851.48 0.000228107498628881
3938.25636363636 0.00021870359487859
4025.03272727273 0.000209883773186845
4111.80909090909 0.000201600158811452
4198.58545454545 0.000193809709249155
4285.36181818182 0.000186473638711082
4372.13818181818 0.000179556921171715
4458.91454545455 0.00017302785994938
4545.69090909091 0.000166857713815465
4632.46727272727 0.00016102037129196
4719.24363636364 0.000155492066157592
4806.02 0.000150251128301108
4892.79636363636 0.000145277764982793
4979.57272727273 0.000140553868329142
5066.34909090909 0.00013606284552033
5153.12545454545 0.000131789468659253
5239.90181818182 0.000127719741753661
5326.67818181818 0.000123840782614299
5413.45454545455 0.000120140717784668
5500.23090909091 0.000116608588881975
5587.00727272727 0.000113234268952311
5673.78363636364 0.000110008387632796
5760.56 0.00010692226407494
5847.33636363636 0.000103967846721266
5934.11272727273 0.000101137659145183
6020.88909090909 9.84247512651708e-05
6107.66545454545 9.58226553313278e-05
6194.44181818182 9.33253461571882e-05
6281.21818181818 9.09272051344104e-05
6367.99454545455 8.86229876239115e-05
6454.77090909091 8.64077933655397e-05
6541.54727272727 8.4277039590581e-05
6628.32363636364 8.22264365580714e-05
6715.1 8.02519652679641e-05
6801.87636363636 7.83498571321453e-05
6888.65272727273 7.6516575408836e-05
6975.42909090909 7.47487982273901e-05
7062.20545454545 7.30434030493924e-05
7148.98181818182 7.13974524285718e-05
7235.75818181818 6.98081809467021e-05
7322.53454545455 6.8272983215589e-05
7409.31090909091 6.6789402846682e-05
7496.08727272727 6.5355122299976e-05
7582.86363636364 6.39679535328491e-05
7669.64 6.2625829377461e-05
7756.41636363636 6.13267955824348e-05
7843.19272727273 6.00690034608562e-05
7929.96909090909 5.8850703092271e-05
8016.74545454545 5.76702370313872e-05
8103.52181818182 5.65260344806873e-05
8190.29818181818 5.54166058881901e-05
8277.07454545454 5.43405379352137e-05
8363.85090909091 5.3296488882219e-05
8450.62727272727 5.22831842437478e-05
8537.40363636364 5.12994127660635e-05
8624.18 5.0344022683481e-05
};
\addplot [very thick, cadetblue80178158]
table {%
212.68 0.12642539400091
251.412929292929 0.129557619385279
290.145858585859 0.129924104686594
328.878787878788 0.12847140082075
367.611717171717 0.125835979189109
406.344646464646 0.1224492505581
445.077575757576 0.118605815837878
483.810505050505 0.114507926359639
522.543434343434 0.110294753050805
561.276363636364 0.106061908578061
600.009292929293 0.101874643827286
638.742222222222 0.0977768829113778
677.475151515152 0.0937974819785649
716.208080808081 0.0899546107897153
754.94101010101 0.0862588487354026
793.673939393939 0.08271539010306
832.406868686869 0.0793256255090292
871.139797979798 0.0760882821686404
909.872727272727 0.073000249453685
948.605656565657 0.0700571781921215
987.338585858586 0.0672539161874494
1026.07151515152 0.0645848244792677
1064.80444444444 0.062044006328486
1103.53737373737 0.0596254720728104
1142.2703030303 0.0573232567137483
1181.00323232323 0.0551315025914607
1219.73616161616 0.0530445162502211
1258.46909090909 0.0510568062312278
1297.20202020202 0.0491631067980278
1335.93494949495 0.0473583913253429
1374.66787878788 0.0456378781390696
1413.40080808081 0.0439970308941521
1452.13373737374 0.0424315550536112
1490.86666666667 0.04093739163977
1529.5995959596 0.0395107091338567
1568.33252525253 0.0381478941778847
1607.06545454545 0.0368455415648168
1645.79838383838 0.0356004438759995
1684.53131313131 0.034409581028681
1723.26424242424 0.0332701099235915
1761.99717171717 0.0321793543274539
1800.7301010101 0.0311347950836523
1839.46303030303 0.0301340607129162
1878.19595959596 0.0291749184423483
1916.92888888889 0.0282552656835747
1955.66181818182 0.0273731219678269
1994.39474747475 0.0265266213362806
2033.12767676768 0.0257140051771645
2071.86060606061 0.0249336154963648
2110.59353535354 0.0241838886050067
2149.32646464646 0.0234633492054123
2188.05939393939 0.0227706048556309
2226.79232323232 0.0221043407921858
2265.52525252525 0.0214633150906098
2304.25818181818 0.0208463541436237
2342.99111111111 0.0202523484373382
2381.72404040404 0.0196802486065645
2420.45696969697 0.0191290617511281
2459.1898989899 0.0185978479959711
2497.92282828283 0.0180857172787423
2536.65575757576 0.0175918263495063
2575.38868686869 0.0171153759681283
2614.12161616162 0.016655608285791
2652.85454545455 0.0162118043979761
2691.58747474747 0.0157832820570784
2730.3204040404 0.0153693935336192
2769.05333333333 0.0149695236157818
2807.78626262626 0.0145830877377035
2846.51919191919 0.0142095302276311
2885.25212121212 0.0138483226676713
2923.98505050505 0.0134989623574575
2962.71797979798 0.0131609708746024
3001.45090909091 0.0128338927253127
3040.18383838384 0.0125172940790205
3078.91676767677 0.0122107615813264
3117.6496969697 0.0119139012399565
3156.38262626263 0.0116263373788188
3195.11555555556 0.0113477116555935
3233.84848484848 0.0110776821386212
3272.58141414141 0.0108159224391531
3311.31434343434 0.0105621208953077
3350.04727272727 0.0103159798043401
3388.7802020202 0.0100772147000667
3427.51313131313 0.00984555367251307
3466.24606060606 0.00962073672705845
3504.97898989899 0.00940251518053901
3543.71191919192 0.00919065109195146
3582.44484848485 0.00898491672555994
3621.17777777778 0.00878509404436164
3659.91070707071 0.00859097423200627
3698.64363636364 0.00840235724139619
3737.37656565657 0.00821905136831222
3776.10949494949 0.00804087284852413
3814.84242424242 0.00786764547694767
3853.57535353535 0.00769920024750562
3892.30828282828 0.00753537501244141
3931.04121212121 0.00737601415991449
3969.77414141414 0.00722096830878575
4008.50707070707 0.00707009401957185
4047.24 0.00692325352061329
};
\addplot [very thick, chocolate21910927]
table {%
33.32 1.02687739323829
105.831515151515 0.348534583109097
178.34303030303 0.196846074733399
250.854545454545 0.131746660334439
323.366060606061 0.0963166453749804
395.877575757576 0.0743850900517243
468.389090909091 0.0596513159395407
540.900606060606 0.0491724732650113
613.412121212121 0.0413990848972089
685.923636363636 0.0354422281637398
758.435151515152 0.0307578173139712
830.946666666667 0.0269954938615563
903.458181818182 0.023920224046572
975.969696969697 0.0213689280414502
1048.48121212121 0.0192252014334859
1120.99272727273 0.017403927116005
1193.50424242424 0.0158415569198497
1266.01575757576 0.0144897772171633
1338.52727272727 0.01331126556116
1411.03878787879 0.0122767790405382
1483.5503030303 0.0113631135650155
1556.06181818182 0.0105516462807163
1628.57333333333 0.00982727669583705
1701.08484848485 0.00917764560661912
1773.59636363636 0.00859255090269847
1846.10787878788 0.00806350507570774
1918.61939393939 0.00758339616637354
1991.13090909091 0.00714622519960822
2063.64242424242 0.0067469008546155
2136.15393939394 0.00638107743514683
2208.66545454545 0.00604502593173041
2281.17696969697 0.00573553061364238
2353.68848484849 0.00544980548999421
2426.2 0.00518542636151088
2498.71151515152 0.00494027519989075
2571.22303030303 0.00471249434484506
2643.73454545455 0.00450044857286191
2716.24606060606 0.0043026935176603
2788.75757575758 0.0041179492466126
2861.26909090909 0.0039450780462643
2933.78060606061 0.00378306566241807
3006.29212121212 0.00363100538993493
3078.80363636364 0.00348808452465496
3151.31515151515 0.00335357278225296
3223.82666666667 0.00322681236210895
3296.33818181818 0.00310720939268191
3368.8496969697 0.0029942265416885
3441.36121212121 0.00288737661209874
3513.87272727273 0.00278621697548475
3586.38424242424 0.00269034471908123
3658.89575757576 0.00259939240319113
3731.40727272727 0.00251302434220034
3803.91878787879 0.00243093333616264
3876.4303030303 0.00235283779124017
3948.94181818182 0.00227847917668361
4021.45333333333 0.00220761977386348
4093.96484848485 0.00214004067940646
4166.47636363636 0.00207554002997622
4238.98787878788 0.00201393142085334
4311.49939393939 0.00195504249436277
4384.01090909091 0.00189871367749362
4456.52242424242 0.00184479705085288
4529.03393939394 0.00179315533347615
4601.54545454545 0.00174366097005011
4674.05696969697 0.00169619530884028
4746.56848484849 0.00165064786010879
4819.08 0.00160691562608952
4891.59151515152 0.00156490249469269
4964.10303030303 0.00152451869006648
5036.61454545455 0.00148568027396898
5109.12606060606 0.00144830869262183
5181.63757575758 0.00141233036433956
5254.14909090909 0.00137767630377243
5326.66060606061 0.00134428177907454
5399.17212121212 0.00131208599872328
5471.68363636364 0.00128103182508013
5544.19515151515 0.00125106551210104
5616.70666666667 0.00122213646488544
5689.21818181818 0.00119419701899971
5761.7296969697 0.00116720223772872
5834.24121212121 0.00114110972560183
5906.75272727273 0.00111587945670982
5979.26424242424 0.00109147361648054
6051.77575757576 0.00106785645571477
6124.28727272727 0.00104499415580358
6196.79878787879 0.00102285470415381
6269.3103030303 0.0010014077789437
6341.82181818182 0.000980624642414479
6414.33333333333 0.000960478041979781
6486.84484848485 0.000940942118501863
6559.35636363636 0.000921992321144531
6631.86787878788 0.0009036053282668
6704.37939393939 0.000885758973870248
6776.89090909091 0.000868432179156861
6849.40242424242 0.000851604888793792
6921.91393939394 0.000835258011517032
6994.42545454546 0.00081937336473819
7066.93696969697 0.000803933622847689
7139.44848484849 0.000788922268933874
7211.96 0.000774323549661436
};
\addplot [very thick, purple11522131]
table {%
106.14 0.28353489737048
191.632727272727 0.106952622091929
277.125454545455 0.058829207588513
362.618181818182 0.0382546045281553
448.110909090909 0.0273463563144605
533.603636363636 0.0207758089611439
619.096363636364 0.0164678449055995
704.589090909091 0.0134671378738368
790.081818181818 0.0112799489425781
875.574545454546 0.0096284274167716
961.067272727273 0.00834564118048794
1046.56 0.00732595172836613
1132.05272727273 0.00649962288373495
1217.54545454545 0.00581897539861275
1303.03818181818 0.00525043124014301
1388.53090909091 0.00476973685257999
1474.02363636364 0.00435898584942818
1559.51636363636 0.00400470248796604
1645.00909090909 0.00369657284528505
1730.50181818182 0.00342658380125898
1815.99454545455 0.00318842582870211
1901.48727272727 0.00297707059100798
1986.98 0.00278846689126041
2072.47272727273 0.00261931831595941
2157.96545454545 0.00246691826656544
2243.45818181818 0.00232902595129698
2328.95090909091 0.00220377204044793
2414.44363636364 0.00208958609256111
2499.93636363636 0.00198514015617948
2585.42909090909 0.00188930452694782
2670.92181818182 0.00180111273544002
2756.41454545455 0.00171973361348186
2841.90727272727 0.00164444883809966
2927.4 0.00157463475039514
3012.89272727273 0.00150974753731601
3098.38545454545 0.00144931107864412
3183.87818181818 0.00139290692110122
3269.37090909091 0.00134016596133809
3354.86363636364 0.00129076151036597
3440.35636363636 0.00124440348130877
3525.84909090909 0.00120083349567418
3611.34181818182 0.00115982074464772
3696.83454545455 0.00112115847412534
3782.32727272727 0.0010846609874819
3867.82 0.00105016108003449
3953.31272727273 0.00101750783501161
4038.80545454545 0.000986564723497368
4124.29818181818 0.000957207960979367
4209.79090909091 0.000929325081324971
4295.28363636364 0.000902813695653326
4380.77636363636 0.000877580408979059
4466.26909090909 0.000853539871926673
4551.76181818182 0.00083061394844683
4637.25454545455 0.000808730983460346
4722.74727272727 0.000787825156834436
4808.24 0.000767835912154765
4893.73272727273 0.000748707450473593
4979.22545454546 0.00073038828065029
5064.71818181818 0.000712830819105938
5150.21090909091 0.000695991032828532
5235.70363636364 0.000679828120322432
5321.19636363636 0.000664304225921825
5406.68909090909 0.000649384183504653
5492.18181818182 0.000635035286168928
5577.67454545455 0.000621227078882074
5663.16727272727 0.000607931171498189
5748.66 0.000595121069868026
5834.15272727273 0.000582772023050384
5919.64545454546 0.000570860884878418
6005.13818181818 0.000559365988346069
6090.63090909091 0.00054826703146328
6176.12363636364 0.000537544973387817
6261.61636363636 0.000527181939780163
6347.10909090909 0.000517161136448707
6432.60181818182 0.000507466770457961
6518.09454545455 0.00049808397796496
6603.58727272727 0.000488998758129872
6689.08 0.000480197912518093
6774.57272727273 0.000471668989473604
6860.06545454546 0.000463400232998578
6945.55818181818 0.000455380535722933
7031.05090909091 0.000447599395590587
7116.54363636364 0.000440046875927343
7202.03636363636 0.000432713568589164
7287.52909090909 0.000425590559919668
7373.02181818182 0.000418669399272422
7458.51454545455 0.000411942069877471
7544.00727272727 0.000405400961852766
7629.5 0.000399038847180188
7714.99272727273 0.000392848856482852
7800.48545454546 0.000386824457455584
7885.97818181818 0.000380959434814158
7971.47090909091 0.000375247871641095
8056.96363636364 0.000369684132016905
8142.45636363636 0.000364262844835516
8227.94909090909 0.000358978888711652
8313.44181818182 0.000353827377895917
8398.93454545455 0.000348803649120696
8484.42727272727 0.000343903249306523
8569.92 0.000339121924064563
};
\addplot [very thick, black18]
table {%
33.32 2.38773010881717
130.519191919192 0.128456433365304
227.718383838384 0.0377599242622377
324.917575757576 0.0171044007147552
422.116767676768 0.00950013936110667
519.31595959596 0.00594583078399538
616.515151515152 0.0040257427868359
713.714343434344 0.00288206231011765
810.913535353536 0.00215106054593345
908.112727272727 0.00165820084001336
1005.31191919192 0.00131169240426903
1102.51111111111 0.00105971812527053
1199.7103030303 0.000871326806495659
1296.90949494949 0.000727157663816716
1394.10868686869 0.000614625410974588
1491.30787878788 0.00052527856258275
1588.50707070707 0.000453281029046548
1685.70626262626 0.000394504017580932
1782.90545454545 0.000345963989426125
1880.10464646465 0.000305464231677061
1977.30383838384 0.000271360174388585
2074.50303030303 0.000242402093037211
2171.70222222222 0.000217627450751364
2268.90141414141 0.000196285815918935
2366.10060606061 0.000177785600020466
2463.2997979798 0.000161655685656033
2560.49898989899 0.000147517389043767
2657.69818181818 0.000135063706900864
2754.89737373737 0.000124043771215783
2852.09656565657 0.000114251076351254
2949.29575757576 0.000105514471853645
3046.49494949495 9.76912058010604e-05
3143.69414141414 9.06615043712169e-05
3240.89333333333 8.43243135404639e-05
3338.09252525253 7.85939279320873e-05
3435.29171717172 7.33973026759887e-05
3532.49090909091 6.86718953245422e-05
3629.6901010101 6.43639222184442e-05
3726.88929292929 6.04269412074618e-05
3824.08848484849 5.68206930753579e-05
3921.28767676768 5.35101493382365e-05
4018.48686868687 5.04647256563007e-05
4115.68606060606 4.76576289034626e-05
4212.88525252525 4.50653126862199e-05
4310.08444444444 4.26670213083216e-05
4407.28363636364 4.04444062189948e-05
4504.48282828283 3.83812021392447e-05
4601.68202020202 3.64629525408279e-05
4698.88121212121 3.46767761117783e-05
4796.0804040404 3.30111673983385e-05
4893.2795959596 3.14558260551152e-05
4990.47878787879 3.00015101313401e-05
5087.67797979798 2.8639909623708e-05
5184.87717171717 2.7363537175791e-05
5282.07636363636 2.61656333319435e-05
5379.27555555556 2.50400841844261e-05
5476.47474747475 2.39813496054312e-05
5573.67393939394 2.29844005459605e-05
5670.87313131313 2.20446641230705e-05
5768.07232323232 2.11579754154328e-05
5865.27151515152 2.03205350520543e-05
5962.47070707071 1.95288718164936e-05
6059.6698989899 1.87798096038968e-05
6156.86909090909 1.80704381646527e-05
6254.06828282828 1.73980871496219e-05
6351.26747474748 1.67603030403929e-05
6448.46666666667 1.61548286059504e-05
6545.66585858586 1.55795845763054e-05
6642.86505050505 1.50326532654406e-05
6740.06424242424 1.45122639115701e-05
6837.26343434343 1.4016779533182e-05
6934.46262626263 1.35446851254322e-05
7031.66181818182 1.30945770438697e-05
7128.86101010101 1.26651534417581e-05
7226.0602020202 1.22552056438953e-05
7323.25939393939 1.18636103541997e-05
7420.45858585859 1.14893226067859e-05
7517.65777777778 1.11313693810454e-05
7614.85696969697 1.07888438106406e-05
7712.05616161616 1.04608999244954e-05
7809.25535353535 1.01467478649981e-05
7906.45454545455 9.84564953487205e-06
8003.65373737374 9.55691462962477e-06
8100.85292929293 9.27989701727862e-06
8198.05212121212 9.01399143128994e-06
8295.25131313131 8.75863044626749e-06
8392.45050505051 8.5132817093597e-06
8489.6496969697 8.27744540306281e-06
8586.84888888889 8.05065191774386e-06
8684.04808080808 7.83245971442572e-06
8781.24727272727 7.62245336037927e-06
8878.44646464647 7.42024172183882e-06
8975.64565656566 7.22545629973278e-06
9072.84484848485 7.03774969572439e-06
9170.04404040404 6.85679419710608e-06
9267.24323232323 6.68228047020703e-06
9364.44242424242 6.51391635296911e-06
9461.64161616162 6.35142573823774e-06
9558.84080808081 6.19454754011228e-06
9656.04 6.04303473641642e-06
};
\addplot [very thick, darkgray153]
table {%
33.32 3.44278941745958
124.810505050505 0.202031953041108
216.30101010101 0.0570305178233965
307.791515151515 0.0246830678084634
399.28202020202 0.0131341045248432
490.772525252525 0.00790247961199322
582.26303030303 0.00516013712445453
673.753535353535 0.00357261141012064
765.24404040404 0.00258485767434777
856.734545454545 0.00193559637970189
948.22505050505 0.00148997173814771
1039.71555555556 0.00117322911868188
1131.20606060606 0.000941495371845894
1222.69656565657 0.000767789137016117
1314.18707070707 0.000634856847909506
1405.67757575758 0.000531294236674707
1497.16808080808 0.000449345880636371
1588.65858585859 0.000383605818658656
1680.14909090909 0.000330223242348308
1771.6395959596 0.000286402033103313
1863.1301010101 0.000250076921385517
1954.62060606061 0.000219698912167768
2046.11111111111 0.000194090064026275
2137.60161616162 0.000172343312697923
2229.09212121212 0.000153752163625518
2320.58262626263 0.000137760566519165
2412.07313131313 0.000123926662129765
2503.56363636364 0.000111896214708857
2595.05414141414 0.000101382905089808
2686.54464646465 9.21535481957038e-05
2778.03515151515 8.40168888220162e-05
2869.52565656566 7.68150272735443e-05
2961.01616161616 7.04167983720074e-05
3052.50666666667 6.47126157510864e-05
3143.99717171717 5.96104254973097e-05
3235.48767676768 5.50325069490203e-05
3326.97818181818 5.09129257032314e-05
3418.46868686869 4.71954925904397e-05
3509.95919191919 4.38321180021605e-05
3601.4496969697 4.07814772444975e-05
3692.9402020202 3.80079221544928e-05
3784.43070707071 3.54805888914115e-05
3875.92121212121 3.317266290717e-05
3967.41171717172 3.10607705440715e-05
4058.90222222222 2.91244731798985e-05
4150.39272727273 2.73458448329692e-05
4241.88323232323 2.57091180149102e-05
4333.37373737374 2.42003856444197e-05
4424.86424242424 2.28073492107155e-05
4516.35474747475 2.15191052503894e-05
4607.84525252525 2.03259636889925e-05
4699.33575757576 1.92192927847224e-05
4790.82626262626 1.81913863616191e-05
4882.31676767677 1.72353497841186e-05
4973.80727272727 1.63450017425622e-05
5065.29777777778 1.55147894205469e-05
5156.78828282828 1.47397150234048e-05
5248.27878787879 1.40152719811101e-05
5339.76929292929 1.33373894130894e-05
5431.2597979798 1.27023836682754e-05
5522.7503030303 1.210691594045e-05
5614.24080808081 1.15479551137705e-05
5705.73131313131 1.10227451222075e-05
5797.22181818182 1.0528776214148e-05
5888.71232323232 1.00637596034258e-05
5980.20282828283 9.62560506360427e-06
6071.69333333333 9.21240108594619e-06
6163.18383838384 8.82239727520682e-06
6254.67434343434 8.45398870282968e-06
6346.16484848485 8.10570197568787e-06
6437.65535353535 7.7761828113152e-06
6529.14585858586 7.46418493853457e-06
6620.63636363636 7.1685601662961e-06
6712.12686868687 6.88824948400476e-06
6803.61737373737 6.62227507419359e-06
6895.10787878788 6.36973313351328e-06
6986.59838383838 6.12978741104178e-06
7078.08888888889 5.90166338417221e-06
7169.57939393939 5.6846430020789e-06
7261.0698989899 5.47805993520798e-06
7352.5604040404 5.28129527657664e-06
7444.05090909091 5.09377364705017e-06
7535.54141414141 4.91495966233416e-06
7627.03191919192 4.74435472427971e-06
7718.52242424242 4.58149410335368e-06
7810.01292929293 4.42594428285123e-06
7901.50343434343 4.27730053869912e-06
7992.99393939394 4.13518473157222e-06
8084.48444444444 3.99924329057585e-06
8175.97494949495 3.86914536997777e-06
8267.46545454545 3.74458116244264e-06
8358.95595959596 3.62526035396334e-06
8450.44646464646 3.51091070722481e-06
8541.93696969697 3.40127676150325e-06
8633.42747474747 3.29611863841596e-06
8724.91797979798 3.19521094391644e-06
8816.40848484849 3.09834175788851e-06
8907.89898989899 3.0053117035484e-06
8999.3894949495 2.91593308962709e-06
9090.88 2.83002911898676e-06
};
\addplot [very thick, saddlebrown1356716]
table {%
539.84 0.0176702618300637
633.675353535354 0.0091103784062054
727.510707070707 0.00528290812425063
821.346060606061 0.00333846029329201
915.181414141414 0.00225205249945508
1009.01676767677 0.00159879728187958
1102.85212121212 0.00118242459222879
1196.68747474747 0.00090418811963968
1290.52282828283 0.000710854534936792
1384.35818181818 0.000572042983726102
1478.19353535354 0.000469565540717173
1572.02888888889 0.000392081762775364
1665.86424242424 0.000332268838125484
1759.6995959596 0.000285252158541102
1853.53494949495 0.000247699076127092
1947.3703030303 0.000217276779655857
2041.20565656566 0.00019231770904045
2135.04101010101 0.000171607244361519
2228.87636363636 0.000154245594365451
2322.71171717172 0.000139555920317319
2416.54707070707 0.000127021967265495
2510.38242424242 0.000116244939655184
2604.21777777778 0.000106913178152074
2698.05313131313 9.87805069222134e-05
2791.88848484849 9.16505517169883e-05
2885.72383838384 8.53652329557126e-05
2979.55919191919 7.97962196036733e-05
3073.39454545455 7.483851040876e-05
3167.2298989899 7.04055623560245e-05
3261.06525252525 6.64255572209849e-05
3354.90060606061 6.28385141819548e-05
3448.73595959596 5.95940376450776e-05
3542.57131313131 5.66495464273817e-05
3636.40666666667 5.39688709030345e-05
3730.24202020202 5.1521133749119e-05
3824.07737373737 4.92798509678882e-05
3917.91272727273 4.72222052567516e-05
4011.74808080808 4.53284551614824e-05
4105.58343434343 4.35814519085321e-05
4199.41878787879 4.19662421614815e-05
4293.25414141414 4.04697397477884e-05
4387.0894949495 3.90804530587571e-05
4480.92484848485 3.77882576300555e-05
4574.7602020202 3.65842055748803e-05
4668.59555555556 3.54603652233733e-05
4762.43090909091 3.44096856357842e-05
4856.26626262626 3.34258816893929e-05
4950.10161616162 3.25033362549904e-05
5043.93696969697 3.16370166266739e-05
5137.77232323232 3.08224028858879e-05
5231.60767676768 3.00554262954554e-05
5325.44303030303 2.93324161535377e-05
5419.27838383838 2.86500538079463e-05
5513.11373737374 2.80053327510258e-05
5606.94909090909 2.73955238947065e-05
5700.78444444445 2.68181452722646e-05
5794.6197979798 2.62709355341702e-05
5888.45515151515 2.57518307051303e-05
5982.29050505051 2.5258943752037e-05
6076.12585858586 2.47905465811735e-05
6169.96121212121 2.43450541402667e-05
6263.79656565657 2.39210103488467e-05
6357.63191919192 2.3517075620534e-05
6451.46727272727 2.3132015774673e-05
6545.30262626263 2.27646921632484e-05
6639.13797979798 2.24140528631565e-05
6732.97333333333 2.20791248043784e-05
6826.80868686869 2.17590067220235e-05
6920.64404040404 2.14528628350688e-05
7014.47939393939 2.11599171673218e-05
7108.31474747475 2.08794484370172e-05
7202.1501010101 2.06107854508149e-05
7295.98545454546 2.03533029460086e-05
7389.82080808081 2.01064178317024e-05
7483.65616161616 1.98695857857238e-05
7577.49151515152 1.96422981692292e-05
7671.32686868687 1.94240792254929e-05
7765.16222222222 1.92144835332842e-05
7858.99757575758 1.90130936886686e-05
7952.83292929293 1.88195181920556e-05
8046.66828282828 1.86333895199322e-05
8140.50363636364 1.84543623630108e-05
8234.33898989899 1.82821120145281e-05
8328.17434343434 1.8116332894209e-05
8422.0096969697 1.79567371949521e-05
8515.84505050505 1.78030536406801e-05
8609.6804040404 1.76550263450035e-05
8703.51575757576 1.75124137614204e-05
8797.35111111111 1.7374987716728e-05
8891.18646464647 1.72425325201664e-05
8985.02181818182 1.71148441415557e-05
9078.85717171717 1.69917294523715e-05
9172.69252525253 1.68730055242794e-05
9266.52787878788 1.67584989801941e-05
9360.36323232323 1.66480453933944e-05
9454.19858585859 1.65414887306514e-05
9548.03393939394 1.6438680835708e-05
9641.86929292929 1.63394809497863e-05
9735.70464646465 1.62437552661052e-05
9829.54 1.61513765156646e-05
};
\addplot [draw=black, fill=black, mark=x, very thick, mark size=2.5pt, only marks]
table{%
x  y
134.8 0.146494654902558
539.84 0.0186736271050518
2142.72 0.00257009146392672
8545.28 0.000339260110195682
};

==> figures/quantitative_results/group_main_3.tex <==
\nextgroupplot[
ylabel shift = -0.2cm,
clip marker paths=true,
width=0.52\textwidth,
height=4.5cm,
title style={yshift=-0.2cm},
scaled x ticks=false,
xlabel style={yshift=0.1cm},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
title={Linear Elasticity},
x grid style={darkgray176},
xlabel={Elements \(\displaystyle (\times 10^3)\)},
xmajorgrids,
xmin=-551.932, xmax=12064.012,
xtick style={color=black},
xtick={-2000,0,2000,4000,6000,8000,10000,12000,14000},
xticklabels={-2.0,0.0,2.0,4.0,6.0,8.0,10.0,12.0,14.0},
y grid style={darkgray176},
ylabel={Squared Error},
ymajorgrids,
ymin=5.55992171425747e-05, ymax=1.73116598883214,
ymode=log,
ytick style={color=black},
ytick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
}
]
\addplot [
  draw=royalblue28108204,
  fill=royalblue28108204,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
271.42 0.106605814000352
341.82 0.0784128563878483
353.26 0.0910435229176025
366.52 0.0730320438086551
394.68 0.0650625149726096
407.74 0.0584584914229364
418.4 0.0606693803247372
420.2 0.0493127232028312
456.92 0.051868355302182
488.56 0.0433722037434131
504.34 0.0423955248616776
538.92 0.0293680372328286
581.72 0.0329062856737456
635.4 0.0247245469615234
645.96 0.0280494475577444
655.06 0.0318785490585947
662.56 0.0329571701160841
664.06 0.0316445770336203
666.78 0.0260319244636584
684.3 0.0246609401306
733 0.0501426321115083
795.52 0.018652945406005
819.34 0.0220466759858583
836.18 0.0206039417495388
879.9 0.0150285895250592
880.84 0.0170371041140525
893.5 0.0138103743408145
915.34 0.0180814111705197
927.7 0.02233027863137
1061.54 0.0159290070530343
1257.78 0.00661872088880234
1273.96 0.0084972475828809
1302.6 0.00761078195621184
1330.1 0.00576122589767241
1330.3 0.0066866089449338
1371.44 0.00631169862976796
1520.52 0.00579018443419992
1574.84 0.00606940289360274
1602.44 0.00542384881451712
1620.96 0.00464812571882298
1712.64 0.00401535698884066
1806.88 0.0044637024662834
1824.58 0.00343516920040012
1833.18 0.00375564190990526
1963.48 0.00445307783055
1968.74 0.00417206546008202
2008.82 0.00489464315558175
2042.92 0.0033501886862271
2085.8 0.00374242051697224
2208.88 0.00313583887067082
2239.48 0.00270746409770763
2557.36 0.00278244203287864
2666.66 0.00166573301676033
2718.5 0.0021646288442573
2784.02 0.00172471763613014
2856.26 0.00212675556447228
2924.44 0.00218190151356095
2948.92 0.00158706243707568
2999.66 0.00168118865716983
3000.32 0.00151188517783369
3252.52 0.00120634616889338
3276.08 0.00142284404994178
3363.52 0.000928262795043815
3373.44 0.000929808742658101
3423.04 0.000989698762361364
3485.36 0.00123109170905157
3545.92 0.00094465663554887
3633.94 0.00143286209006131
3738.74 0.00116756600742772
4360.52 0.000744839177498326
4517.84 0.000729231750768611
4656.3 0.000594803554837518
4665.26 0.000715647837964524
4669.16 0.000702916465450353
4704.78 0.000721063730609188
4836.92 0.000531359022049817
4884.38 0.000629589007908922
5064.22 0.000494807528208721
5155.24 0.000623847279416359
5190.18 0.000714319857965041
5345.22 0.000492787375382855
5808.88 0.000473097068654762
5933.14 0.000384271585655832
6250.5 0.000342723455901967
6383.84 0.000425994052896478
6601.32 0.000413662118391082
7028.12 0.000235637116652944
7147.82 0.000263167244281184
7285.5 0.000315641507489854
7558.78 0.000273103096464109
8004.3 0.000391863603320476
8041.88 0.000200159312559241
8102.46 0.000157479398200219
8733.48 0.000199655586592603
8894.46 0.000120733973308103
9169.26 0.000158745960107538
9242.9 0.000115577429873696
9745.58 0.000137263281414931
10341.7 0.000103640696026909
10827.44 8.89832417778698e-05
};
\addplot [
  draw=cadetblue80178158,
  fill=cadetblue80178158,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
208.92 0.153424445628512
209.86 0.14610570616009
211.28 0.119640619547173
218.24 0.14901677438442
224.08 0.178824970924827
231.88 0.148193303508201
262.32 0.147964848145385
284.3 0.27285798365575
290.94 0.366849744307524
329.72 0.200814980373319
391.78 0.0624949430996049
421.64 0.0542477714267245
421.76 0.0924687356128762
430.14 0.0845480521629051
454.5 0.0798147414580984
465.94 0.549161130928365
467.56 0.311705695949139
480.96 0.104073729985161
496.72 0.0433305514572823
525.54 0.0583366724679071
531.64 0.0515798581734869
560.3 0.0707966559435389
579.1 0.0583973546821304
602.36 0.190106452922885
603.12 0.221715819032469
606.5 0.0940116679295074
621.9 0.108467420901385
635.2 0.0818369346604553
699.74 0.107870257720654
709.5 0.0969458308342032
728 0.0294974738190566
736.64 0.155206773495116
836.06 0.0667373138416828
853.18 0.0462876834722416
884.62 0.0262531667183055
890 0.0542169249092586
905.18 0.0261443544366584
908.4 0.0596720180871403
923.18 0.282285834621994
943.26 0.0249322756429858
944.5 0.317157701536104
976.28 0.189276217718494
985.28 0.0229109291148013
1045.54 0.0295932571499663
1078.44 0.259842288786618
1092.08 0.0284957402032658
1142.46 0.0136783645022612
1146.14 0.016456246549887
1180.64 0.0260161021616322
1184.62 0.0214334559173025
1212.1 0.0376990656982806
1213.58 0.0158373362081697
1217.92 0.0151480732941594
1247.3 0.0106765815388036
1253.84 0.0768511104369187
1256.94 0.0225245667989927
1260.38 0.0116947148111287
1385.08 0.0252567151548092
1385.58 0.0125764671658645
1405.82 0.244790804923172
1479.36 0.00802392554528171
1496.56 0.0177279003331272
1513.98 0.0124381633920264
1552.58 0.0115135911313676
1582.54 0.0163142478698431
1591.22 0.0328118097534962
1605.7 0.0502079312389834
1608.66 0.00980825397069075
1647.58 0.00831853749686704
1650.44 0.0153180553126528
1670.44 0.00834941372411557
1670.8 0.0145099874588786
1673 0.0131574009621213
1677.58 0.00855457851671469
1697.24 0.00751764488463775
1725.84 0.00871400900397147
1740.02 0.027961273253409
1779.12 0.0792849270440343
1837.88 0.00837894522907555
1849.36 0.00754303149139505
1915.4 0.0481969451275689
1941.68 0.0174530773114027
1941.8 0.0110421683635074
1961.34 0.00875723201138038
2082.8 0.00636458856913025
2126.74 0.0179336217858102
2132.04 0.017012417172795
2132.64 0.00584370968576076
2272.28 0.077877386835798
2286.12 0.00518630204551364
2331.5 0.00494422627506986
2382.48 0.00558137502883495
2537.34 0.0109139011326656
2657.46 0.0064978581554907
2712.78 0.00367052958943131
2779.88 0.00460860593236314
2782.82 0.00489130436951127
2924.14 0.00767270545665162
3124.1 0.00769406064096164
3598.8 0.0399923163957668
};
\addplot [
  draw=chocolate21910927,
  fill=chocolate21910927,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
21.52 0.999999993258309
23.4 0.999999996039599
23.44 0.999999995975606
23.46 0.999999995989741
23.68 0.999999996020024
23.72 0.999999996023892
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
23.82 0.999999996122416
27.24 1.00230361365338
56.3 0.690964747053063
68 0.377521254558437
76.38 0.315633121529024
110.94 0.192999000581388
125.68 0.360801411710085
128.22 0.216813395905554
159.22 0.943242780959166
165.4 0.153415532035507
182.92 0.235941680625069
217.72 0.150380175357821
235.1 0.068158327342096
238.62 0.0760667122397123
248.88 0.251583987724092
270.68 0.76214180148582
274.88 0.0653661043432944
351.64 0.0603192573114466
376.28 0.0525078414187748
408.36 0.0974609973383949
419.06 0.0393665730695053
420.76 0.0465388379969933
426.8 0.112860977014587
432.28 0.070275067488921
439.7 0.0361793532148775
510.54 0.0341639546418358
559.04 0.086311246620783
611.06 0.0724988694693003
631.9 0.0303484204333282
639.38 0.0432326393280082
648.18 0.044717108075816
773.72 0.0450680372166332
868.66 0.0541760875458956
922.24 0.0366073868832422
1169.46 0.0124217678717432
1751.58 0.114399114366206
1823.7 0.0101068973030538
1950.46 0.00733967057516051
2170.06 0.0678777363276302
2368.96 0.0141022316227945
2573.04 0.0116711840171314
2768.32 0.019533590035356
3536.34 0.0143793497458716
4046.7 0.00581642890690849
4540.78 0.00368233037052443
6780.12 0.000623141549313094
8209.1 0.00168656097432665
8965.7 0.00337769826976722
9354.4 0.00552173695693054
};
\addplot [draw=purple11522131, fill=purple11522131, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
336.66 0.0680162646963843
363.62 0.0662187701855255
378.66 0.0721057696638585
382.46 0.0607247473558358
391.66 0.0520091287608055
395.94 0.0564679564112043
419.04 0.0577192964994661
441.44 0.0514797915392547
453 0.0369175544961218
466.94 0.0483593302840383
945.22 0.0239228847037097
1164.1 0.0220029140452478
1213.38 0.0228873565005452
1249.96 0.0241539858289707
1318.94 0.0342337164764184
1340.9 0.0224270714826669
1356.56 0.0222905770892828
1358.82 0.0228538150551287
1396.26 0.0223672383981686
1451.96 0.023500019608051
1478.14 0.0222052664448807
1479.32 0.0223532988940319
1524.06 0.0221028347922318
1525.64 0.0220825066758445
1525.66 0.0220830665934843
1525.76 0.0220825055651083
1525.76 0.0220825055651083
1525.76 0.0220825055651083
1525.76 0.0220825055651083
1525.76 0.0220825055651083
1591.12 0.0119115299943415
1647.82 0.0123997491391439
1903.68 0.0159554716555746
1913.18 0.0119695633989661
1978.66 0.016344123755007
2044.72 0.0210615214513479
2347 0.0113417245256515
2729.76 0.0110421539272058
3035.64 0.0096927394688761
3255.34 0.00654060589561155
4021.38 0.0105914273315205
4159.48 0.010595840704466
4396.38 0.0105585579200991
5052.98 0.00865652993540068
5065.7 0.0062805279627293
5838.58 0.0066942900105509
5941.06 0.0062289827358909
6108.3 0.00618836058589075
6118.26 0.00618535975880503
6118.28 0.00618414284841863
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6118.4 0.00618414503102881
6630.36 0.00576154578143396
6947.1 0.00576197983079482
6947.84 0.00576041962274625
6947.84 0.00576041962274625
6947.84 0.00576041962274625
6947.84 0.00576041962274625
6947.84 0.00576041962274625
6947.84 0.00576041962274625
6947.84 0.00576041962274625
7217.34 0.00242802232322071
10538.18 0.00249046657129108
};
\addplot [draw=black18, fill=black18, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
23.82 0.999999996122416
71.64 0.264361235781971
74.3 0.253733492059791
77.18 0.243198493106946
78.36 0.2386437311006
79.02 0.227830078214795
81.3 0.222610945912341
84.36 0.213598988557825
86.92 0.203082004712418
90.98 0.200273678583781
94.24 0.192967408501776
97.8 0.180736999885877
99 0.178845777977741
103.7 0.171590050046116
107.94 0.161352040860733
109.62 0.15739935603842
114.9 0.149757447870641
118.06 0.142907677218202
120.52 0.139301712870519
128.36 0.130626916028959
129.4 0.125091652629951
132.94 0.119406868684332
138.28 0.114565123106824
144.46 0.111653982180565
151.98 0.106606332763568
159.56 0.0987110975374893
171.08 0.0893042559494447
174.94 0.08589227782181
183.62 0.0835574314436055
192.86 0.0761089459583658
197.34 0.0715776941293519
204.84 0.0673559117578015
209.42 0.0639809253486229
220.16 0.0610352545622113
231.6 0.058424322134559
236.58 0.0565332235202671
248.94 0.0527464759055718
267.68 0.0486804715223707
282.48 0.0454172621937302
293.44 0.0432093001005805
306.84 0.0407960672152896
317.6 0.0385949498589021
325.84 0.0359303432917876
356.68 0.0324269038198332
377.36 0.0303065253303287
420.98 0.0261820705305302
431.16 0.0244424227739899
455.6 0.022406257484079
476.48 0.021157129496736
509.02 0.0193589750732689
538 0.017906841735341
582.64 0.0160330799262705
637.24 0.0146892916449538
686.24 0.0128202848885408
724.28 0.0117385684435184
755.26 0.0109314179171201
821 0.0099354408369089
898.68 0.0086327174940159
973.36 0.00759426100712432
1053.76 0.00685228468598466
1110.94 0.00647710014531992
1226.28 0.00559006290063423
1282.62 0.00535080750825029
1355.62 0.0049229715193397
1495.78 0.0043752750714869
1594.38 0.00397292361490805
1765.08 0.0036258102203011
1865.94 0.00329783173772371
1965.08 0.00286650822410327
2168.8 0.00250241846676422
2358.3 0.00221499659208974
2481.08 0.00198424943220313
2739.2 0.00179122633490661
2941.74 0.00155745769693462
3246.62 0.00136215301702053
3471.76 0.00125043657668028
3684.26 0.00116840546576866
3754.88 0.00107000695199492
4111.44 0.000978713360969101
4366.32 0.000899005808719233
4503.28 0.000812318945228849
5100.72 0.000726135509645369
5316.66 0.00066205441937008
5490.44 0.000625796056706884
5873.54 0.000550213096515521
6493.86 0.00050705376689062
6833.34 0.00047428713871769
7339.82 0.000435192728869586
7498.48 0.000394383631980102
8052.96 0.000357348029107824
8385.9 0.000332089722618927
8980.58 0.000299103448772671
9459.4 0.00026750056762253
10396.5 0.000235256371140711
11490.56 0.000205119539835594
};
\addplot [draw=darkgray153, fill=darkgray153, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
23.82 0.999999996122416
89.64 0.462587109472181
93.02 0.45552013053367
95.04 0.444081541669213
98.58 0.430748265283238
101.46 0.40745478250005
106.06 0.399010538452598
108.9 0.379761596824669
112.6 0.346823021445124
114.06 0.357083263723042
119.42 0.328956917615149
124.26 0.322038889402902
126.26 0.312484039578048
132.1 0.301420001157195
135.42 0.287747501984738
138.34 0.276552730636623
142.72 0.269185322043765
148.1 0.256479547324249
151.72 0.245080791344835
157.36 0.230695270355932
160.26 0.222656437274091
166.48 0.215305081213318
172.9 0.212981489160153
178.74 0.20787243159195
181.88 0.201052508082732
190.24 0.177500751817669
193.16 0.172480211234113
196.7 0.165367311187082
198.3 0.165329503236665
203.52 0.152516228771389
204.44 0.147172226369426
210.82 0.140736336916628
217.72 0.129010154080082
217.74 0.132205842896732
221 0.123470133549031
231.24 0.113653376175103
232.9 0.1200319192999
239.9 0.105978852251599
245.36 0.101290901469224
250.2 0.0992742045674702
252.16 0.0952854905924079
256.98 0.0955016948093499
262.7 0.0929591414109634
266.5 0.0901552325460188
278.82 0.087177429689896
280.24 0.0852646454684384
287.94 0.0849199228955915
295.34 0.0820800041293871
296.3 0.0794516751224546
298.72 0.0777128671770473
305.34 0.0765901893992716
316.64 0.0741915305123521
320.48 0.070834818893093
322.06 0.0681582049716273
323.54 0.0681977830742222
329.5 0.0667049925115096
338.1 0.0644641709329616
344.18 0.0623947090390265
349.54 0.0598662779016721
358.38 0.0598914159239075
362.7 0.0582669091416217
368.3 0.0577295497791849
377 0.0554445491804335
381.6 0.0531512962073003
389.04 0.050405978433773
402.74 0.0478474459690963
409.1 0.0466032106996372
423.22 0.0458412238839294
437.32 0.0443248905648719
458.8 0.04117154027962
463.48 0.0385887532596061
494.48 0.0376143591338595
505.58 0.035700030947914
537.2 0.0332713844485226
544.68 0.0321899645394493
554.38 0.0302438609950498
585.86 0.0282900306682315
586.94 0.0293924998680429
604.02 0.02644566984099
664.92 0.02454456244716
670.6 0.0231450599137319
705.98 0.0222471306204199
718.48 0.0212742108439797
750.98 0.0199711515246733
771.94 0.0183597529205405
828.66 0.0167608311333103
891.34 0.0153213502836595
1007.02 0.0139509988609692
1078.44 0.0130132201592853
1170.62 0.0114174301287161
1350.5 0.00955287338369882
1543.08 0.00789633276520308
1770.36 0.00631651204600218
2136.42 0.00491095226516821
2516.2 0.00373533052615471
3102.78 0.00271670928607792
4130 0.0018022900679753
5545.4 0.00106320843761488
8963.64 0.000526888045983455
};
\addplot [
  draw=saddlebrown1356716,
  fill=saddlebrown1356716,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
380.48 0.0734326103192033
410.1 0.0493964013911281
412.06 0.0486516161359166
414.82 0.0476185269157886
420.7 0.0463321307943505
426.78 0.0454433168547066
427.36 0.0454127563554697
428.92 0.0429422751049597
431.88 0.0438258641887263
446.56 0.041138104332603
449.24 0.0395963454244448
454.72 0.0391538689675709
464.16 0.0363639240838864
472.16 0.0344789943551879
478.46 0.0324091872493685
492.02 0.0308525205145728
496.12 0.0300018438047113
505.36 0.0289917578523967
520.76 0.0278162419930432
534.7 0.0268313346909194
553.04 0.0244941952754446
564.32 0.0226039861432298
593.12 0.0213402976812707
613.36 0.020431748839929
642.3 0.0198949256513419
645.3 0.0188868776420828
693.16 0.0175095248940163
707.66 0.0165780012722334
724.92 0.0152458171511421
756.4 0.0140814079298055
758.24 0.0132710712411183
800.24 0.0126174902526147
825.64 0.0121162081766054
826.9 0.011338942382997
861.22 0.0107074345189484
874.3 0.0105240835711341
921.36 0.00978783039916408
944.22 0.00914979625925667
974.54 0.008851990122137
1020.64 0.00814567845679383
1054.26 0.00780933365115575
1071.54 0.00749664488730295
1094.46 0.00720910880808132
1117.78 0.00695782236402211
1159.74 0.0066410887471975
1182.82 0.00644841184303877
1225.44 0.00615730861854686
1259.1 0.00584924375126788
1300.94 0.0056527222940849
1356.74 0.00533494021371753
1421.08 0.00513247068965617
1454.48 0.00470868876017539
1511.64 0.00442026628646087
1560.24 0.00414158868061136
1636.42 0.00393600853143326
1678.12 0.00374340633559206
1719.64 0.0035604016187971
1752.6 0.0034216908199776
1844.4 0.00330532237618093
1856.66 0.00315628191594103
1923.66 0.00303578124555907
1987.92 0.00289152806910853
2071.44 0.00276871989364593
2181.42 0.00262774635918919
2238.54 0.00252060543141329
2266.82 0.00240417260996668
2457.5 0.00225619467766429
2531.46 0.0021123272064577
2672.72 0.00199996697749183
2773.14 0.00191997713931957
2858.76 0.00173268741156666
2889.78 0.00181752067247969
2932.48 0.00163145944312184
3081.22 0.00155345256089381
3177.36 0.00147478748980192
3272.2 0.00142390935626903
3429.18 0.00128181781484339
3429.68 0.00134003477051596
3724.44 0.00121879688679259
3849.4 0.00118757138507059
4052.06 0.00113927763774321
4099.5 0.0010791433846045
4331.5 0.00102662905953599
4466.52 0.000993461958949783
4562.4 0.000949487779922288
4705.14 0.00090148399771363
5026.92 0.000869716763234638
5184.82 0.000826546818440021
5396.86 0.000783120841693535
5563.08 0.000743995404829932
5796.48 0.000696161457605359
5937.7 0.00066653551422614
6275.34 0.000639466316478862
6513.98 0.000604912250794598
6738.1 0.000579157487694004
7025.48 0.000554459167929781
7165.32 0.000531337855653063
7476.46 0.000495716505529276
7588.3 0.000472058413059
8014.84 0.000444731440151822
};
\addplot [very thick, royalblue28108204]
table {%
271.42 0.117708506263896
378.046464646465 0.0697562660168146
484.672929292929 0.0464722463466168
591.299393939394 0.0332899706033041
697.925858585859 0.0250609399204711
804.552323232323 0.0195623797230379
911.178787878788 0.0156989208589442
1017.80525252525 0.0128771269187678
1124.43171717172 0.0107516541750654
1231.05818181818 0.00910994473503389
1337.68464646465 0.00781511977674178
1444.31111111111 0.00677568741031254
1550.93757575758 0.00592854948000911
1657.56404040404 0.00522901432342094
1764.19050505051 0.00464469114662887
1870.81696969697 0.00415162904945996
1977.44343434343 0.00373180278725579
2084.0698989899 0.00337143286432216
2190.69636363636 0.00305983727943743
2297.32282828283 0.00278863061095677
2403.94929292929 0.00255115513699649
2510.57575757576 0.00234207009538168
2617.20222222222 0.00215705068666345
2723.82868686869 0.00199256449474634
2830.45515151515 0.00184570334499837
2937.08161616162 0.00171405540834793
3043.70808080808 0.00159560689353827
3150.33454545455 0.00148866574667496
3256.96101010101 0.00139180189678787
3363.58747474747 0.00130380006642774
3470.21393939394 0.00122362221340672
3576.8404040404 0.00115037741928608
3683.46686868687 0.00108329758265755
3790.09333333333 0.00102171767193574
3896.7197979798 0.00096505958527407
4003.34626262626 0.000912818883461894
4109.97272727273 0.000864553825678322
4216.59919191919 0.000819876262241151
4323.22565656566 0.00077844403335264
4429.85212121212 0.000739954595786671
4536.47858585859 0.000704139655933279
4643.10505050505 0.000670760631620054
4749.73151515152 0.000639604799629468
4856.35797979798 0.000610482013038091
4962.98444444445 0.000583221894079391
5069.61090909091 0.000557671425432887
5176.23737373737 0.000533692876625559
5282.86383838384 0.000511162013329364
5389.4903030303 0.000489966546316202
5496.11676767677 0.000470004784125975
5602.74323232323 0.000451184459455541
5709.3696969697 0.000433421704152974
5815.99616161616 0.000416640151712861
5922.62262626263 0.000400770149480144
6029.24909090909 0.000385748065514334
6135.87555555556 0.000371515677347879
6242.50202020202 0.000358019631776347
6349.12848484849 0.000345210966411648
6455.75494949495 0.000333044685067579
6562.38141414142 0.000321479380173804
6669.00787878788 0.000310476896366161
6775.63434343434 0.000300002030207299
6882.26080808081 0.000290022261676328
6988.88727272727 0.000280507513649141
7095.51373737374 0.000271429936088807
7202.1402020202 0.000262763712091347
7308.76666666667 0.000254484883297638
7415.39313131313 0.000246571192496358
7522.0195959596 0.000239001941513624
7628.64606060606 0.000231757862718861
7735.27252525253 0.000224821002678753
7841.89898989899 0.000218174616666721
7948.52545454546 0.00021180307288783
8055.15191919192 0.000205691765411855
8161.77838383838 0.000199827034923084
8268.40484848485 0.000194196096496651
8375.03131313131 0.000188786973699836
8481.65777777778 0.000183588438394499
8588.28424242424 0.000178589955685092
8694.91070707071 0.000173781633516789
8801.53717171717 0.000169154176481219
8908.16363636364 0.00016469884343405
9014.7901010101 0.000160407408569992
9121.41656565657 0.00015627212563737
9228.04303030303 0.000152285695006898
9334.6694949495 0.000148441233338051
9441.29595959596 0.000144732245612084
9547.92242424242 0.000141152599323559
9654.54888888889 0.000137696500642538
9761.17535353535 0.00013435847237782
9867.80181818182 0.000131133333587758
9974.42828282828 0.000128016180699779
10081.0547474747 0.000125002370012697
10187.6812121212 0.000122087501467608
10294.3076767677 0.000119267403583634
10400.9341414141 0.000116538119464219
10507.5606060606 0.000113895893788143
10614.1870707071 0.000111337160707104
10720.8135353535 0.000108858532578581
10827.44 0.000106456789468948
};
\addplot [very thick, cadetblue80178158]
table {%
208.92 0.198285222783853
243.161212121212 0.180913831313006
277.402424242424 0.16530605346624
311.643636363636 0.15139120148013
345.884848484848 0.139012283858049
380.126060606061 0.127993205588893
414.367272727273 0.118165159058227
448.608484848485 0.109375996065347
482.849696969697 0.101492414441346
517.090909090909 0.0943991944175775
551.332121212121 0.0879973489144419
585.573333333333 0.0822020072629344
619.814545454545 0.0769403796264135
654.055757575758 0.0721499336464773
688.29696969697 0.0677768171873323
722.538181818182 0.0637745186648302
756.779393939394 0.0601027400064516
791.020606060606 0.0567264528584239
825.261818181818 0.0536151095414305
859.50303030303 0.0507419832460146
893.744242424242 0.0480836155399188
927.985454545455 0.0456193527516872
962.226666666667 0.0433309559235075
996.467878787879 0.0412022717112831
1030.70909090909 0.0392189538596838
1064.9503030303 0.0373682267391125
1099.19151515152 0.0356386839558321
1133.43272727273 0.0340201162909436
1167.67393939394 0.0325033642379421
1201.91515151515 0.0310801912346109
1236.15636363636 0.0297431743584085
1270.39757575758 0.0284856098042789
1304.63878787879 0.0273014309135653
1338.88 0.0261851368914976
1373.12121212121 0.0251317306538998
1407.36242424242 0.0241366644936922
1441.60363636364 0.0231957924643694
1475.84484848485 0.0223053285489324
1510.08606060606 0.0214618098251742
1544.32727272727 0.0206620639569891
1578.56848484849 0.0199031804406945
1612.8096969697 0.0191824851186547
1647.05090909091 0.0184975175425492
1681.29212121212 0.0178460108277049
1715.53333333333 0.0172258736898697
1749.77454545455 0.0166351743981556
1784.01575757576 0.0160721264138841
1818.25696969697 0.0155350755157394
1852.49818181818 0.0150224882378449
1886.73939393939 0.0145329414698162
1920.98060606061 0.0140651130871022
1955.22181818182 0.0136177734964947
1989.46303030303 0.0131897779959676
2023.70424242424 0.0127800598603499
2057.94545454545 0.0123876240750176
2092.18666666667 0.0120115416490611
2126.42787878788 0.0116509444474415
2160.66909090909 0.011305020488667
2194.9103030303 0.0109730096606448
2229.15151515152 0.0106541998127195
2263.39272727273 0.0103479231865951
2297.63393939394 0.010053553152954
2331.87515151515 0.00977050122420076
2366.11636363636 0.00949821431694186
2400.35757575758 0.00923617224061688
2434.59878787879 0.00898388539117746
2468.84 0.00874089263090037
2503.08121212121 0.00850675933736308
2537.32242424242 0.00828107560633341
2571.56363636364 0.00806345459485367
2605.80484848485 0.00785353099216257
2640.04606060606 0.00765095960730957
2674.28727272727 0.00745541406339904
2708.52848484848 0.00726658558936739
2742.7696969697 0.00708418190106064
2777.01090909091 0.00690792616415412
2811.25212121212 0.00673755603214877
2845.49333333333 0.00657282275330273
2879.73454545455 0.0064134903409152
2913.97575757576 0.00625933480188402
2948.21696969697 0.00611014341891152
2982.45818181818 0.00596571408214229
3016.69939393939 0.00582585466638555
3050.94060606061 0.00569038245040862
3085.18181818182 0.00555912357508925
3119.42303030303 0.00543191253748851
3153.66424242424 0.00530859171815247
3187.90545454545 0.00518901093917684
3222.14666666667 0.00507302705077139
3256.38787878788 0.00496050354424746
3290.62909090909 0.00485131018952
3324.8703030303 0.00474532269536915
3359.11151515152 0.00464242239084656
3393.35272727273 0.00454249592633915
3427.59393939394 0.00444543499291995
3461.83515151515 0.00435113605872133
3496.07636363636 0.00425950012116429
3530.31757575758 0.00417043247396587
3564.55878787879 0.00408384248792878
3598.8 0.00399964340459198
};
\addplot [very thick, chocolate21910927]
table {%
21.52 1.08168090754878
115.791515151515 0.270228216604031
210.06303030303 0.156343010383921
304.334545454545 0.109573710861452
398.606060606061 0.0839895413441919
492.877575757576 0.0678472930506371
587.149090909091 0.0567403222886828
681.420606060606 0.0486371409291398
775.692121212121 0.0424697644941405
869.963636363636 0.0376226609772885
964.235151515151 0.0337159970625372
1058.50666666667 0.030502662777314
1152.77818181818 0.0278149663318392
1247.0496969697 0.0255351155663826
1341.32121212121 0.0235779555252204
1435.59272727273 0.0218804080218973
1529.86424242424 0.0203947615430352
1624.13575757576 0.0190842673968631
1718.40727272727 0.0179201674744056
1812.67878787879 0.0168796386369333
1906.9503030303 0.0159443401239769
2001.22181818182 0.0150993672828608
2095.49333333333 0.0143324849778753
2189.76484848485 0.0136335572188593
2284.03636363636 0.0129941168434405
2378.30787878788 0.0124070367344279
2472.57939393939 0.0118662756994939
2566.85090909091 0.0113666799696203
2661.12242424242 0.0109038266265165
2755.39393939394 0.0104738989875419
2849.66545454545 0.0100735865963807
2943.93696969697 0.00970000433798139
3038.20848484848 0.00935062654794058
3132.48 0.00902323297455408
3226.75151515151 0.00871586418169347
3321.02303030303 0.00842678452528053
3415.29454545455 0.00815445124625666
3509.56606060606 0.00789748853448594
3603.83757575758 0.00765466565662386
3698.10909090909 0.00742487842512406
3792.38060606061 0.0072071334286999
3886.65212121212 0.00700053455660323
3980.92363636364 0.00680427143735426
4075.19515151515 0.00661760948252735
4169.46666666667 0.00643988128198769
4263.73818181818 0.0062704791417043
4358.0096969697 0.00610884859131772
4452.28121212121 0.00595448271784544
4546.55272727273 0.00580691720568236
4640.82424242424 0.00566572598249076
4735.09575757576 0.00553051738654139
4829.36727272727 0.00540093078423367
4923.63878787879 0.00527663357742794
5017.9103030303 0.00515731854928615
5112.18181818182 0.00504270150488062
5206.45333333333 0.00493251916916267
5300.72484848485 0.00482652731020375
5394.99636363636 0.00472449906010636
5489.26787878788 0.00462622340977511
5583.53939393939 0.00453150385695431
5677.81090909091 0.00444015718967621
5772.08242424242 0.0043520123895976
5866.35393939394 0.00426690964170038
5960.62545454545 0.00418469943854415
6054.89696969697 0.00410524176873233
6149.16848484848 0.00402840538052289
6243.44 0.00395406711261157
6337.71151515152 0.00388211128506684
6431.98303030303 0.00381242914421925
6526.25454545455 0.00374491835602678
6620.52606060606 0.00367948254306227
6714.79757575758 0.0036160308608163
6809.06909090909 0.00355447760948642
6903.34060606061 0.00349474187784363
6997.61212121212 0.00343674721613533
7091.88363636364 0.00338042133530814
7186.15515151515 0.00332569583012028
7280.42666666667 0.00327250592396564
7374.69818181818 0.00322079023345526
7468.9696969697 0.00317049055099985
7563.24121212121 0.00312155164381308
7657.51272727273 0.00307392106791126
7751.78424242424 0.00302754899582438
7846.05575757576 0.00298238805685772
7940.32727272727 0.00293839318885343
8034.59878787879 0.00289552150050105
8128.8703030303 0.00285373214333452
8223.14181818182 0.0028129861926323
8317.41333333333 0.00277324653650918
8411.68484848485 0.00273447777255202
8505.95636363636 0.00269664611140964
8600.22787878788 0.00265971928679896
8694.49939393939 0.00262366647143645
8788.77090909091 0.00258845819844628
8883.04242424242 0.00255406628783496
8977.31393939394 0.00252046377765675
9071.58545454545 0.00248762485952568
9165.85696969697 0.00245552481815853
9260.12848484848 0.00242413997465885
9354.4 0.00239344763327571
};
\addplot [very thick, purple11522131]
table {%
336.66 0.0634210201288621
439.705656565657 0.0524408608376257
542.751313131313 0.0449724041910137
645.79696969697 0.0395163345482046
748.842626262626 0.0353321744692379
851.888282828283 0.0320083670348552
954.933939393939 0.0292963407089876
1057.9795959596 0.0270363689750439
1161.02525252525 0.0251207612263027
1264.07090909091 0.0234740650478597
1367.11656565657 0.0220417249915719
1470.16222222222 0.020783245246651
1573.20787878788 0.0196678895945222
1676.25353535354 0.018671879053711
1779.29919191919 0.0177765091594883
1882.34484848485 0.0169668513666917
1985.39050505051 0.0162308365206276
2088.43616161616 0.0155585947438634
2191.48181818182 0.0149419713656408
2294.52747474748 0.0143741661837091
2397.57313131313 0.0138494607117875
2500.61878787879 0.0133630092307651
2603.66444444444 0.0129106767985298
2706.7101010101 0.0124889122901621
2809.75575757576 0.0120946478946884
2912.80141414141 0.0117252188207524
3015.84707070707 0.0113782986009455
3118.89272727273 0.0110518465530615
3221.93838383838 0.0107440648011293
3324.98404040404 0.0104533628767544
3428.0296969697 0.0101783283780064
3531.07535353535 0.00991770250422759
3634.12101010101 0.00967035954238803
3737.16666666667 0.00943528957634934
3840.21232323232 0.00921158384056633
3943.25797979798 0.00899842225588602
4046.30363636364 0.00879506277556822
4149.34929292929 0.00860083224062297
4252.39494949495 0.00841511849960357
4355.44060606061 0.00823736359252902
4458.48626262626 0.0080670578342078
4561.53191919192 0.00790373466085155
4664.57757575758 0.00774696612699387
4767.62323232323 0.00759635895851458
4870.66888888889 0.00745155108290343
4973.71454545455 0.00731220857047053
5076.7602020202 0.00717802293056693
5179.80585858586 0.00704870871544464
5282.85151515151 0.00692400139149902
5385.89717171717 0.00680365544356744
5488.94282828283 0.00668744268292066
5591.98848484849 0.00657515073375156
5695.03414141414 0.00646658167647714
5798.0797979798 0.00636155082913994
5901.12545454545 0.00625988565071231
6004.17111111111 0.00616142475224986
6107.21676767677 0.00606601700366824
6210.26242424242 0.00597352072548091
6313.30808080808 0.00588380295617806
6416.35373737374 0.00579673878708046
6519.39939393939 0.00571221075749809
6622.44505050505 0.00563010830388355
6725.49070707071 0.00555032725741645
6828.53636363636 0.00547276938510265
6931.58202020202 0.00539734197003627
7034.62767676768 0.00532395742696436
7137.67333333333 0.00525253294972435
7240.71898989899 0.00518299018750119
7343.76464646465 0.00511525494718191
7446.8103030303 0.00504925691937609
7549.85595959596 0.00498492942592728
7652.90161616162 0.00492220918696626
7755.94727272727 0.00486103610575742
7858.99292929293 0.00480135306976653
7962.03858585859 0.00474310576653523
8065.08424242424 0.00468624251308757
8168.1298989899 0.0046307140977178
8271.17555555556 0.00457647363311987
8374.22121212121 0.00452347641991751
8477.26686868687 0.00447167981974282
8580.31252525253 0.0044210431370896
8683.35818181818 0.0043715275092396
8786.40383838384 0.00432309580362273
8889.44949494949 0.00427571252202998
8992.49515151515 0.00422934371114933
9095.54080808081 0.00418395687894106
9198.58646464647 0.00413952091641125
9301.63212121212 0.00409600602437953
9404.67777777778 0.00405338364487192
9507.72343434343 0.00401162639680028
9610.76909090909 0.00397070801561788
9713.81474747475 0.00393060329666648
9816.8604040404 0.00389128804195312
9919.90606060606 0.00385273901011586
10022.9517171717 0.00381493386935722
10125.9973737374 0.00377785115314107
10229.043030303 0.00374147021846501
10332.0886868687 0.00370577120653456
10435.1343434343 0.00367073500567891
10538.18 0.00363634321636008
};
\addplot [very thick, black18]
table {%
23.82 1.06521776190511
139.645656565657 0.113300280663535
255.471313131313 0.0507098426562563
371.29696969697 0.0305272552818242
487.122626262626 0.0210176005001351
602.948282828283 0.0156320084136306
718.773939393939 0.0122266788857753
834.599595959596 0.00990857331614284
950.425252525253 0.00824466170185893
1066.25090909091 0.00700159992929231
1182.07656565657 0.00604345117534511
1297.90222222222 0.00528611696544571
1413.72787878788 0.00467501877512436
1529.55353535354 0.00417332603627578
1645.37919191919 0.00375536447806132
1761.20484848485 0.00340273865580738
1877.0305050505 0.00310195465912946
1992.85616161616 0.00284291023109378
2108.68181818182 0.00261790614619883
2224.50747474747 0.00242098146514995
2340.33313131313 0.00224745598815334
2456.15878787879 0.00209360872188224
2571.98444444444 0.00195644770053078
2687.8101010101 0.00183354243663535
2803.63575757576 0.00172290010961984
2919.46141414141 0.00162287281396169
3035.28707070707 0.00153208720211012
3151.11272727273 0.0014493905007501
3266.93838383838 0.00137380865178234
3382.76404040404 0.00130451353799601
3498.5896969697 0.00124079708996012
3614.41535353535 0.0011820506578348
3730.24101010101 0.00112774844931121
3846.06666666667 0.00107743413534391
3961.89232323232 0.00103070994399216
4077.71797979798 0.000987227723479824
4193.54363636364 0.000946681574989161
4309.36929292929 0.000908801745191247
4425.19494949495 0.000873349536162394
4541.02060606061 0.00084011304188743
4656.84626262626 0.000808903560139538
4772.67191919192 0.000779552559148018
4888.49757575757 0.000751909102314172
5004.32323232323 0.000725837652929845
5120.14888888889 0.000701216195597774
5235.97454545454 0.000677934622750291
5351.8002020202 0.000655893343994687
5467.62585858586 0.000635002083497706
5583.45151515151 0.000615178836654284
5699.27717171717 0.000596348962172055
5815.10282828283 0.000578444389679115
5930.92848484848 0.00056140292621233
6046.75414141414 0.000545167647610734
6162.5797979798 0.000529686363036773
6278.40545454545 0.000514911142666719
6394.23111111111 0.000500797900101848
6510.05676767677 0.000487306022310589
6625.88242424242 0.000474398040964477
6741.70808080808 0.000462039339913938
6857.53373737374 0.000450197894293418
6973.35939393939 0.000438844037373187
7089.18505050505 0.000427950251806705
7205.01070707071 0.000417490982374113
7320.83636363636 0.000407442467706923
7436.66202020202 0.000397782588807441
7552.48767676768 0.000388490732457687
7668.31333333333 0.000379547667853895
7784.13898989899 0.000370935435010434
7899.96464646465 0.000362637243656068
8015.7903030303 0.000354637381500347
8131.61595959596 0.000346921130882047
8247.44161616162 0.000339474692928076
8363.26727272727 0.00033228511845258
8479.09292929293 0.000325340244914312
8594.91858585858 0.000318628638827534
8710.74424242424 0.000312139543089188
8826.5698989899 0.000305862828744363
8942.39555555555 0.000299788950764015
9058.22121212121 0.00029390890745471
9174.04686868687 0.000288214203160504
9289.87252525252 0.000282696813952628
9405.69818181818 0.000277349156034208
9521.52383838384 0.000272164056615089
9637.34949494949 0.000267134727036615
9753.17515151515 0.000262254737948158
9869.00080808081 0.000257517996356792
9984.82646464646 0.000252918724388884
10100.6521212121 0.000248451439617961
10216.4777777778 0.000244110936827061
10332.3034343434 0.000239892271086266
10448.1290909091 0.00023579074203714
10563.9547474747 0.000231801879285898
10679.7804040404 0.000227921428816003
10795.6060606061 0.00022414534033899
10911.4317171717 0.000220469755509571
11027.2573737374 0.000216890996937584
11143.083030303 0.000213405557935297
11258.9086868687 0.000210010092943844
11374.7343434343 0.000206701408587448
11490.56 0.000203476455308401
};
\addplot [very thick, darkgray153]
table {%
23.82 2.48637746878994
114.121212121212 0.314730652905395
204.422424242424 0.140563060948021
294.723636363636 0.0838896879492185
385.024848484848 0.0572498767931484
475.326060606061 0.0422350341499462
565.627272727273 0.0327913508917356
655.928484848485 0.026396611931209
746.229696969697 0.0218297601715134
836.530909090909 0.0184343757553967
926.832121212121 0.0158290993296765
1017.13333333333 0.0137786788249962
1107.43454545455 0.01213088514657
1197.73575757576 0.0107832893685034
1288.03696969697 0.00966469276319343
1378.33818181818 0.00872422397635052
1468.63939393939 0.00792466763197208
1558.94060606061 0.00723823563345972
1649.24181818182 0.00664380390607147
1739.54303030303 0.00612505810761954
1829.84424242424 0.00566921983868209
1920.14545454545 0.00526615325492257
2010.44666666667 0.00490772673608189
2100.74787878788 0.00458734911474704
2191.04909090909 0.00429962760290779
2281.3503030303 0.00404011199564956
2371.65151515152 0.00380510098031233
2461.95272727273 0.00359149377886657
2552.25393939394 0.00339667530675093
2642.55515151515 0.00321842640529498
2732.85636363636 0.00305485303697844
2823.15757575758 0.00290432996752761
2913.45878787879 0.00276545561969872
3003.76 0.00263701561790558
3094.06121212121 0.00251795314922772
3184.36242424242 0.00240734471168967
3274.66363636364 0.00230438015101064
3364.96484848485 0.00220834613426675
3455.26606060606 0.00211861239557791
3545.56727272727 0.00203462023101955
3635.86848484848 0.00195587282894403
3726.1696969697 0.00188192710609949
3816.47090909091 0.00181238678543626
3906.77212121212 0.00174689650277879
3997.07333333333 0.00168513676994796
4087.37454545455 0.00162681965393886
4177.67575757576 0.00157168505727681
4267.97696969697 0.00151949750511746
4358.27818181818 0.00147004336111812
4448.57939393939 0.00142312840742664
4538.88060606061 0.00137857573496118
4629.18181818182 0.00133622389899471
4719.48303030303 0.00129592530230613
4809.78424242424 0.00125754477412845
4900.08545454545 0.00122095831805646
4990.38666666667 0.00118605200616904
5080.68787878788 0.00115272100002821
5170.98909090909 0.00112086868206428
5261.2903030303 0.00109040588324265
5351.59151515151 0.00106125019491524
5441.89272727273 0.00103332535445272
5532.19393939394 0.00100656069568631
5622.49515151515 0.000980890656404033
5712.79636363636 0.000956254336180646
5803.09757575758 0.000932595098703417
5893.39878787879 0.000909860213511161
5983.7 0.000888000532711508
6074.00121212121 0.000866970198798348
6164.30242424242 0.000846726380171285
6254.60363636364 0.000827229031373314
6344.90484848485 0.000808440675421884
6435.20606060606 0.000790326205919668
6525.50727272727 0.000772852706902084
6615.80848484848 0.000755989288614259
6706.1096969697 0.000739706937615897
6796.41090909091 0.000723978379792509
6886.71212121212 0.000708777955009014
6977.01333333333 0.000694081502280153
7067.31454545454 0.000679866254453793
7157.61575757576 0.000666110741510382
7247.91696969697 0.000652794701676298
7338.21818181818 0.000639898999632461
7428.51939393939 0.000627405551173457
7518.82060606061 0.000615297253737957
7609.12181818182 0.000603557922289498
7699.42303030303 0.000592172230078299
7789.72424242424 0.000581125653860975
7880.02545454545 0.000570404423195968
7970.32666666667 0.000559995473469305
8060.62787878788 0.000549886402337957
8150.92909090909 0.000540065429307494
8241.2303030303 0.000530521358187023
8331.53151515152 0.000521243542187992
8421.83272727273 0.00051222185145463
8512.13393939394 0.000503446642832933
8602.43515151515 0.000494908731702229
8692.73636363636 0.000486599365708896
8783.03757575757 0.000478510200255734
8873.33878787879 0.000470633275613221
8963.64 0.000462960995530227
};
\addplot [very thick, saddlebrown1356716]
table {%
380.48 0.0546279248549204
457.594747474747 0.0375761238166947
534.709494949495 0.0276473355616558
611.824242424242 0.0213422490376262
688.93898989899 0.017076111628135
766.053737373737 0.0140465142095557
843.168484848485 0.0118115630873212
920.283232323232 0.0101113947966948
997.39797979798 0.00878491749924047
1074.51272727273 0.00772784901603347
1151.62747474747 0.00687019352273007
1228.74222222222 0.00616350275274906
1305.85696969697 0.0055733456869402
1382.97171717172 0.00507468553283893
1460.08646464646 0.00464894702355347
1537.20121212121 0.00428210191451724
1614.31595959596 0.00396338716925204
1691.43070707071 0.00368442724210257
1768.54545454545 0.00343862085594392
1845.6602020202 0.00322070474513777
1922.77494949495 0.00302643816930202
1999.8896969697 0.00285237134135106
2077.00444444444 0.00269567312266016
2154.11919191919 0.00255400120852631
2231.23393939394 0.00242540319750968
2308.34868686869 0.00230824039453447
2385.46343434343 0.00220112854536674
2462.57818181818 0.00210289131858443
2539.69292929293 0.00201252348231683
2616.80767676768 0.00192916152372817
2693.92242424242 0.0018520600327588
2771.03717171717 0.00178057258703981
2848.15191919192 0.00171413617890192
2925.26666666667 0.00165225845005301
3002.38141414141 0.00159450716703994
3079.49616161616 0.00154050149663847
3156.61090909091 0.00148990473588893
3233.72565656566 0.0014424182245335
3310.8404040404 0.00139777622383324
3387.95515151515 0.00135574158932053
3465.0698989899 0.00131610209904073
3542.18464646465 0.00127866732552625
3619.29939393939 0.00124326596082249
3696.41414141414 0.00120974352062281
3773.52888888889 0.00117796036693367
3850.64363636364 0.00114778999941535
3927.75838383838 0.00111911757419326
4004.87313131313 0.0010918386159428
4081.98787878788 0.00106585789475473
4159.10262626263 0.00104108844395051
4236.21737373737 0.0010174506988443
4313.33212121212 0.000994871739601872
4390.44686868687 0.000973284623955673
4467.56161616162 0.000952627797701253
4544.67636363636 0.000932844572704914
4621.79111111111 0.000913882663661312
4698.90585858586 0.000895693776105183
4776.02060606061 0.000878233239246219
4853.13535353535 0.000861459678094911
4930.2501010101 0.00084533472010777
5007.36484848485 0.000829822732226331
5084.4795959596 0.000814890584733844
5161.59434343434 0.000800507438823008
5238.70909090909 0.000786644555169292
5315.82383838384 0.000773275121149073
5392.93858585859 0.000760374094637757
5470.05333333333 0.000747918062578499
5547.16808080808 0.000735885112732523
5624.28282828283 0.00072425471721306
5701.39757575758 0.000713007626570522
5778.51232323232 0.000702125773340641
5855.62707070707 0.000691592184092669
5932.74181818182 0.000681390899124376
6009.85656565657 0.000671506899046319
6086.97131313131 0.000661926037581837
6164.08606060606 0.000652634979982846
6241.20080808081 0.000643621146526348
6318.31555555555 0.000634872660613657
6395.4303030303 0.000626378301044608
6472.54505050505 0.000618127458083594
6549.6597979798 0.000610110092973646
6626.77454545455 0.000602316700589664
6703.88929292929 0.000594738274952922
6781.00404040404 0.000587366277356532
6858.11878787879 0.000580192606876122
6935.23353535353 0.0005732095730618
7012.34828282828 0.00056640987062707
7089.46303030303 0.000559786555967876
7166.57777777778 0.000553333025360435
7243.69252525253 0.000547042994700761
7320.80727272727 0.00054091048066113
7397.92202020202 0.000534929783150266
7475.03676767677 0.000529095468973999
7552.15151515152 0.000523402356602464
7629.26626262626 0.000517845501958088
7706.38101010101 0.000512420185146063
7783.49575757576 0.000507121898055822
7860.6105050505 0.000501946332768052
7937.72525252525 0.000496889370707312
8014.84 0.000491947072485376
};
\addplot [draw=black, fill=black, mark=x, very thick, mark size=2.5pt, only marks]
table{%
x  y
93.04 0.254825928505529
380.48 0.0734326103191988
1525.76 0.0220825055651117
6118.4 0.00618414503102848
};


==> figures/quantitative_results/group_main_4.tex <==
\nextgroupplot[
ylabel shift = -0.2cm,
clip marker paths=true,
width=0.52\textwidth,
height=4.5cm,
title style={yshift=-0.2cm},
xlabel style={yshift=0.1cm},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
title={Heat Diffusion},
x grid style={darkgray176},
xlabel={Elements \(\displaystyle (\times 10^3)\)},
xmajorgrids,
xmin=-310.541, xmax=6886.121,
xtick style={color=black},
xtick={-1000,0,1000,2000,3000,4000,5000,6000,7000},
xticklabels={-1.0,0.0,1.0,2.0,3.0,4.0,5.0,6.0,7.0},
y grid style={darkgray176},
ylabel={\empty},
ymajorgrids,
ymin=3.64827548515554e-06, ymax=1.84109103460723,
ymode=log,
ytick style={color=black},
ytick={1e-07,1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
yticklabels={
  \(\displaystyle {10^{-7}}\),
  \(\displaystyle {10^{-6}}\),
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
}
]
\addplot [
  draw=royalblue28108204,
  fill=royalblue28108204,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
133.44 0.047045130071596
138 0.0507864194561023
141.8 0.0436467341466666
146.1 0.041595628406001
146.44 0.0431985392053121
153.3 0.048111856013925
162.38 0.039234193570476
165.54 0.036722796102492
167.9 0.0318069238739355
189.6 0.0395225586595994
204.06 0.0164140677886604
207.74 0.022549976037297
230.58 0.019292235425908
233.06 0.0184788514416036
248.06 0.0178093502311033
250.44 0.0186196776748131
255.44 0.0167875203112952
260.52 0.0278971827571598
261.76 0.0148847783473722
264.6 0.0188861888711061
271.96 0.0102236878328443
272.44 0.0188986997027052
281 0.0145454083092935
289.62 0.0144909772580529
291.4 0.0109901758949574
305.72 0.00936418060193728
307.56 0.0094509344901877
311.56 0.0198633711127232
360.82 0.0100530383169772
375.08 0.00378731042176533
377.74 0.00780603410569311
394.44 0.0119469208957523
405.78 0.00599154987887895
406.78 0.015581920094371
408.02 0.00454939552704384
417.92 0.00727564000753055
438.64 0.00413117251095636
451.72 0.00547194097777625
453.22 0.00399241286783048
476.84 0.00784375566598355
498.92 0.00229424699673669
512.3 0.00356084931760927
519.94 0.0034996758020079
599.06 0.00335374188286673
641.6 0.00303070841471098
675.32 0.00165450049348524
727.7 0.00132003439014545
744.84 0.00106498537186491
773.4 0.00204367955776631
795.8 0.00145662740139769
988.5 0.00894502938571521
1005.6 0.00320776590748635
1147.96 0.000588255596296905
1286.12 0.000702729423133018
1398.16 0.000292716550753597
1447.7 0.000299958648012235
1471.64 0.000295599678350048
1521 0.000325003167840349
1573.26 0.000419838670069375
1590.04 0.000433113013779453
1621.4 0.000439333508342352
1623.6 0.000325164512552009
1647.38 0.000372014777501486
1673.4 0.000249365679521255
1677.58 0.000247996544806882
1678.06 0.000239678331558339
1688.4 0.000295485547958837
1702.14 0.000306202140894956
1703.96 0.000239520017990434
1838.72 0.000185465211337022
1855.98 0.000243173362705213
1873.36 0.000245727177588385
1895.58 0.00025794447751702
1947.64 0.000176026127686935
1951.76 0.00018650528094501
2003.7 0.000141121785570566
2037.88 0.000179835848743748
2053 0.000214593494353814
2129.38 0.000375280882639659
2177.14 0.000196539580594045
2455.48 0.0001352859147008
2549.96 0.000147336439401315
2560.1 0.000100644191827
2585.28 0.000133643201791573
2647.58 0.000150342389035403
2742.8 8.02356523261813e-05
2755.7 0.0001036669671328
3016.2 6.82470430995834e-05
3138.74 5.78064378619215e-05
3482.62 5.25214426582331e-05
3543.48 7.8335631190399e-05
3660.34 9.80640271670677e-05
3751.12 5.76188288018684e-05
3935.06 3.44683609022441e-05
4118.32 4.15799755404963e-05
4133.4 5.93783328167404e-05
4705.12 1.60384519967028e-05
5146.54 1.21947975271891e-05
5720.14 1.30584798707453e-05
6132.4 1.86291848603597e-05
};
\addplot [
  draw=cadetblue80178158,
  fill=cadetblue80178158,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
242.86 0.0198571974102344
244.46 0.0198720518826477
249.04 0.0136883657429868
280.28 0.0104018624080352
283.86 0.0176056627432769
285.52 0.0239339743075028
292.24 0.0189859298684862
293 0.0116301601944133
400.12 0.0494534633437264
425.56 0.0407396272763355
462.82 0.0148775072380652
464.62 0.0387717878580091
468.74 0.0038330014636409
468.84 0.0296975567567635
498.72 0.0127000154812053
522.52 0.0122241067277326
539.04 0.0936455288307691
546.72 0.00456974922172698
565.04 0.369501916452377
623.98 0.00680470294537138
648.04 0.0958922452977854
677.08 0.00215513420923335
677.54 0.823268652727098
704.1 0.0201012574955357
707.3 0.700574528136578
760.7 0.0045735568096571
768.4 0.0198277126705638
773 0.00215217380664695
805.24 0.00590474638985617
818.28 0.0272045606166493
867.76 0.00845889211864289
872.84 0.014218418684689
910.48 0.316507355434827
939.3 0.00651731620701779
939.48 0.452158440449719
960.74 0.225461716439083
964.18 0.00584988082135006
976.46 0.00712341156976097
986.18 0.0042812518896803
995.72 0.15199611344221
1026.42 0.0162708734093366
1142.7 0.0126900607046592
1162.52 0.341463635807447
1238.78 0.00135819335622785
1267.16 0.81624455842829
1276.48 0.0126109153129103
1339.94 0.873377275500827
1385.76 0.00317149312153767
1448.54 0.00166409386270422
1448.84 0.00239649024567723
1463.72 0.00739387945993167
1494.7 0.0779190085999611
1497.04 0.00752130736021602
1549.56 0.0111495011806632
1669.84 0.0926691628136607
1684.26 0.000644355544411874
1696.46 0.0043989897900895
1716.16 0.0545987256128962
1728.54 0.00113602868572218
1787.26 0.00202948935359028
1793.2 0.0850461043882475
1846.68 0.00968173377849679
1945.1 0.185451407105218
1959.24 0.00551738880303571
1990.96 0.000256465850563723
2039.32 0.357323506353042
2042.28 0.0119988707029396
2050.58 0.000707624508485956
2062.24 0.00220805093536573
2090.9 0.000765225464447418
2169 0.00333627728254569
2220.56 0.0236216009697536
2258.82 0.00709575199783313
2389.04 0.00320665095155077
2396.12 0.017447629959343
2418.42 0.00402575924674348
2421.88 0.00408664959222032
2512.32 0.0269034836430061
2527.1 0.0216766149411586
2555.66 0.000407484628888346
2570.22 0.00109189605200772
2575.02 0.000906569015439736
2603.7 0.000287972301565965
2653.1 0.736738367412721
2672.96 0.00133311781954047
2764.78 0.14122881912057
2783.64 0.00574863235786217
2832.38 0.00100081200044148
2843.2 0.000726444753060773
2888.32 0.00518699141205565
2937.84 0.0763556905558947
3005.38 0.0118242935976043
3042.28 0.0140038819876859
3104.16 0.00611290751643724
3134.4 0.000640268108968404
3328.28 0.000323326047477188
3463.82 0.00110457947906092
3628.18 0.00027412290410932
3958.96 0.129844714646427
4206.46 0.00610491892786528
};
\addplot [
  draw=chocolate21910927,
  fill=chocolate21910927,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
16.58 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.68 0.999999999999989
16.7 0.999999999999989
16.7 0.999999999999989
16.74 0.999999999999984
16.76 0.999999999999989
16.78 0.999999999999988
16.78 0.999999999999985
16.9 0.999999999999987
17.04 0.999999999999988
20.2 0.923240002969972
23.3 0.796738332509069
96.36 0.0915418355714445
131.06 0.163907452721159
136.18 0.0824334880482369
138.98 0.342382640129188
139.74 0.0839139795491292
146.76 0.0416444078546878
194.46 0.0178795874802294
200.86 0.494279828675559
212.24 0.0201676810017231
221.08 0.0225383558011681
240.62 0.0156005320225963
245.76 0.0133082361955253
252.5 0.0177063706773103
259.4 0.0152671217612651
264.38 0.0150201461001418
267.14 0.0150370060376077
267.44 0.0142961486868349
277.1 0.0184277391335557
299.76 0.0121833874354614
300.84 0.0120229637804141
326.4 0.0140547875514943
331.18 0.0244723519289912
343.62 0.174680669670905
347.94 0.00941173211349001
348.64 0.00801390638480188
357.02 0.00690926685747384
429.12 0.00974397139591365
434.36 0.00482158486527231
567.46 0.00515037835270986
613.9 0.00252025181582528
673.56 0.00234827454416232
676.66 0.00597088715661607
1108.78 0.00436144155018397
1122.64 0.0338237155175123
1220.12 0.00108172240346929
1430.06 0.00157758620447943
1486.08 0.0003538446418223
1500.26 0.00434560358361244
1638.86 0.0013998826330158
1718.16 0.00205536140519535
1793.98 0.000480799248909965
1861.24 0.00125980742805052
1863.4 0.584053156313898
1890.38 0.000636707862880662
2224.2 0.0012159973626992
2582.46 0.000928260821747862
2774.54 0.000363665528376675
2803.58 0.000133463364187408
2883.7 0.000656186007030664
3132.78 0.000403645222911668
3925.72 5.97605867750261e-05
4226.56 9.04806340483399e-05
4335.16 5.56710940447278e-05
4357.52 0.000412527198101017
5409.22 0.000130873059084774
5812.3 1.79900713280854e-05
6139.62 0.00148719507869924
6148.78 5.38531645559123e-05
6559 7.48747767075303e-05
};
\addplot [draw=purple11522131, fill=purple11522131, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
274.5 0.0649176731507602
320.76 0.0233847044941131
331.1 0.017295975769587
333.98 0.0395745999606315
344.44 0.0131984877492167
347.52 0.0285131950817031
356.6 0.0258832430377004
373.94 0.0210026217727957
394.16 0.0303104936493865
422.36 0.0318036121168123
481.86 0.0164946853118827
485.74 0.012474750674391
493.26 0.0144886150248845
549.1 0.0102903582587852
756.08 0.00999059915642741
756.24 0.0178667758116475
759.56 0.00953016032264267
777.64 0.0112350677304944
813.1 0.00979849097353723
825.74 0.00830519838966002
877.62 0.00722190663343028
993.24 0.00768571377148029
1061.38 0.00778471645828506
1105.6 0.007606687814
1107.1 0.00773758689644161
1107.72 0.00760194760355461
1120.24 0.007599259231322
1120.6 0.00773758726832065
1120.92 0.00773758905606582
1121.24 0.00773758898991344
1121.28 0.00773758905606573
1121.28 0.00773758905606573
1125.56 0.00701756432664323
1146.36 0.00706994889817948
1167.96 0.00769617040601349
1176.5 0.00609263706256041
1186.5 0.00750925450913847
1212.14 0.0068761558356007
1260.72 0.00491290868877773
1290.72 0.00494936541835966
2094.94 0.00234897952146803
2892.54 0.000846134272347596
3257.9 0.0008495907920145
3549.62 0.000761826060990904
3711.96 0.000742568001817013
3713.04 0.000780580489559968
4115.82 0.00111885644773874
4209.2 0.000734002281883085
4244.24 0.000681509301001615
4271.36 0.000681339242325744
4280.28 0.00073399685934094
4280.32 0.00073399685934094
4302.66 0.000688372694071686
4356.08 0.000693769409156868
4370.64 0.000681339281969654
4397.32 0.00068134273038931
4407.56 0.00068650376611244
4415.12 0.000681339364615352
4416.36 0.000681339364649673
4432.04 0.000681339364709567
4437.9 0.000681339364709533
4440.34 0.000681441468991161
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4464.64 0.000681339364709526
4521.94 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
4531.2 0.000661349223622249
5272.6 0.000416211062465289
5631.54 0.000406808388574851
5711.74 0.000406881456520103
5819 0.000406811177091083
5830.42 0.000406811163067053
5844.4 0.000406813548168337
5847.04 0.000406811163065364
5847.04 0.000406811163065364
5847.04 0.000406811163065364
5847.04 0.000406811163065364
};
\addplot [draw=black18, fill=black18, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
16.68 0.999999999999989
77.8 0.0688649304649009
79.44 0.0680472597159073
81 0.0625100190748133
82.74 0.061371735312965
85.92 0.0569618491819852
86.44 0.0542693759697416
87.66 0.051605672928069
91.52 0.0491149594373838
92.94 0.0473588097599363
93.98 0.0463034772003285
99.32 0.0437675047715378
102.58 0.0418403965934691
105.5 0.039406192158903
109.24 0.0361719299872419
114 0.0335483555281824
116.86 0.031672126087107
120.12 0.0300303086555698
122.02 0.03024326087012
125.62 0.0285828591043438
129.54 0.0252370742923603
129.84 0.0268824838484178
136.36 0.0236087465904019
140.88 0.022615590391521
144.04 0.0217436441123498
149.66 0.0200280545762559
153.18 0.0180179125247634
157.54 0.0163151669404546
161.02 0.0155215586155428
167.9 0.015091071952331
170.76 0.0146367714477994
178 0.0143579243370352
187.12 0.0132068570216783
195.54 0.0123488136838134
198.1 0.0115090905155284
206.9 0.0108829147344744
207.98 0.009920937760097
212.98 0.00926240426491047
224.72 0.00897503529028386
235.78 0.00839742071131921
250.6 0.00757904343276923
269.76 0.00698244774480459
271.28 0.00718010422083999
290.08 0.00645538650669142
304.22 0.00583892354505665
322.26 0.00546794399655007
334.04 0.00496177145129576
349.58 0.00432604766616311
363.44 0.0039374080146898
369.16 0.00379571680472949
377.22 0.0033096390602915
395.88 0.00348678916005446
426.74 0.00304291558290446
439.98 0.00284326052122896
445.14 0.00287094950717384
480.32 0.00260967718194329
493.32 0.00228090972050766
517.48 0.00211967870335943
538.46 0.0017619024842644
541.32 0.00183269599319876
579.58 0.0015603681445374
628.92 0.00134700451404256
666.98 0.00117490873609758
705.2 0.000953547135893107
778.1 0.000824103552718091
810.42 0.000789705052537695
852.04 0.000776953935282881
905.22 0.000635912835359384
957.84 0.000576458584919411
1070.9 0.000484444665222281
1108.9 0.000435722353407869
1196.12 0.000389482930064432
1243.88 0.000356557743096479
1318.56 0.000307833714448349
1386.2 0.000272223980640556
1522.42 0.000230170001874882
1645.88 0.00018841733254625
1842.6 0.000176925854176365
1906.74 0.000149207283362542
2102.66 0.000115851288045106
2344.02 9.92318411891702e-05
2500.22 7.68251995105854e-05
2585.32 7.19367679516674e-05
2885.16 5.64532832634981e-05
3077.52 4.7034440042438e-05
3157.16 4.50236737166088e-05
3628.72 3.54111330408942e-05
3674.48 3.07280049895359e-05
4159.02 2.38419441179487e-05
4803.86 1.68175495399259e-05
5171.64 1.26110970977015e-05
5582.08 1.10232321955006e-05
6202.34 6.62695979463675e-06
6261.22 9.18739876917272e-06
};
\addplot [draw=darkgray153, fill=darkgray153, forget plot, mark=*, mark size=1, only marks, draw opacity=0,
 fill opacity=0.5]
table{%
x  y
16.68 0.999999999999989
123.12 0.0456831115849286
132.8 0.0437064699353301
137.32 0.0417256737827629
141.22 0.0411483521370875
145.26 0.0398350899081917
150.22 0.0354018725161364
158.28 0.0325740369499728
162.68 0.0318354583484522
163.5 0.0302545117759796
172.4 0.0286298296936205
176.98 0.0281534097992785
180.3 0.0256865423943131
181.24 0.0253010755992902
186.1 0.0230455459787634
192.76 0.0226297972051247
202.98 0.0204708517092555
211.06 0.0198193128949171
213.84 0.0183138068392256
215.4 0.0175650753818173
221.1 0.0167116930658601
226.28 0.0165532100872246
247 0.0153263577494176
247.92 0.0148419781986684
263.22 0.0129696022695405
277.72 0.0114634843273833
291.86 0.011081661841874
296.04 0.0110334737029188
300.44 0.0105300386004348
305.82 0.0103430184012356
313.6 0.0100933040416747
324.84 0.00950387863758912
334.22 0.00906185073334895
351.24 0.00863593152025356
371.9 0.00867988122823222
378.02 0.00825704651740491
386.84 0.00768871368000414
399.68 0.00687357345848579
425.16 0.00608769072391468
434.1 0.0055570160576165
444.68 0.00542073621770003
466.32 0.00521320569814292
487.1 0.00489768567083043
496.02 0.00466124930343267
506.22 0.0041367278873783
523.8 0.00377660118095113
534.3 0.00378585509850544
557.12 0.00350410855065373
561.4 0.00360932734144618
586.14 0.00323137334094422
596.6 0.00336484322242352
608.8 0.00311990216336173
621.52 0.00296069721224494
650.08 0.00271344885212747
672.76 0.00264933693746978
718.8 0.00239329542235597
763.84 0.00213538621311893
776.66 0.00223302706221147
790.26 0.00187412097388463
801.32 0.00179464465363944
834.98 0.00171929374967511
847.74 0.00139866303418157
871.6 0.00138102244409424
887.38 0.0013119866111509
926.4 0.0011984483194511
971.38 0.00111684174376608
986.62 0.00100595123397026
1028.16 0.000935450915517334
1046.82 0.000796744280737098
1076.12 0.00075960682418478
1150.98 0.000770708515848027
1221.3 0.000663269001353277
1239.52 0.000605504734232028
1277.56 0.000603337595421516
1308.02 0.000533347605542618
1387.56 0.0004627140228908
1426.04 0.000435170839185786
1457.12 0.000385932345697423
1463.86 0.000381160730253037
1561.9 0.000319663768988013
1633.76 0.000279230301599724
1804.22 0.000237966332340915
1809.12 0.000221111033508545
2003.52 0.000178312240153392
2019.94 0.000198297079248302
2168.5 0.000153042323514669
2257.96 0.000124382850172624
2487.48 0.000106153457320061
2624.88 8.97771441963406e-05
2876.98 7.50948773494533e-05
3050.02 6.36246532441755e-05
3246.08 4.73170574550317e-05
3548.2 4.24962642330668e-05
3847.44 3.25539971238481e-05
4380.16 2.45384858234908e-05
4791.34 1.54697117806043e-05
5893.32 9.97730478934581e-06
};
\addplot [
  draw=saddlebrown1356716,
  fill=saddlebrown1356716,
  forget plot,
  mark=*, mark size=1,
  only marks,
  draw opacity=0,
 fill opacity=0.5
]
table{%
x  y
275.52 0.0639982120304522
333.08 0.0108254999546955
337.4 0.010608303692181
340.38 0.0105760184126206
340.4 0.0101627421237738
342.82 0.00965118407108243
352.12 0.00938868881413495
359.28 0.00916115819065932
361.6 0.00896132110257746
369.38 0.00861774865167718
373.34 0.00850037582960301
384.44 0.00830381990084657
389.84 0.00810542962608424
395.4 0.00787269330513739
405.64 0.00755378632908325
414.72 0.0074390671227715
431.18 0.00730256770430657
444.06 0.00703382557457678
458.76 0.00679540172552916
482.98 0.00676333894487965
498.52 0.00639462601656605
511.38 0.00626012556402665
527.92 0.00616543919864461
543.98 0.00610701855283887
556.78 0.00602413849469301
567.14 0.00585303170158177
584.04 0.00565084910199258
606.44 0.00535029108952207
625.06 0.00516974110472809
639.84 0.00491623034391196
654.22 0.00487418766494069
665.52 0.00478585825697367
684.18 0.00472487924460663
703.68 0.00463810277361599
723.22 0.00450090214159358
738.86 0.00443462545070508
762.04 0.00443144068269943
780.38 0.00432779514059826
799.4 0.00431375624848503
821.88 0.00419005535235987
832 0.00389870490583642
861.22 0.00379998826678883
884.98 0.00376029085460264
901.46 0.00367018238930044
935.88 0.00371798279192552
972.14 0.00367510171446593
990.94 0.00360292463289592
1021.2 0.0036144430363605
1047.7 0.00342286150029205
1072.1 0.00333765696539728
1104.52 0.00329400084828474
1130.42 0.00315832916895844
1170.92 0.00299755729248055
1207.02 0.00296887776603204
1233.98 0.00289290777187202
1260.44 0.00285158734709604
1299.7 0.00281735357033377
1338.36 0.00262640282866239
1376.78 0.00243485568497157
1398.86 0.00231793931906804
1440.44 0.00230116131554842
1460.16 0.00227574222888813
1509.86 0.00218796725729045
1547.34 0.00199805094212733
1579 0.00193990931555715
1606.44 0.00171854092641719
1660.5 0.00167672995932544
1703.38 0.00160208350908261
1759.04 0.0016088680480027
1846.28 0.00148442409437299
1889.56 0.00136801470477335
1926.34 0.00139798373134732
1955.04 0.0013693982647206
1996.42 0.00133618871946899
2103.56 0.00132591270398722
2131.5 0.0012556658200759
2183.64 0.00115374334099008
2209.7 0.00118646667445867
2308.42 0.00110086002911878
2346.52 0.0010451643868691
2386.7 0.000971203661433711
2492.74 0.000882514927065916
2570.78 0.000863691355291669
2603.16 0.000818242252350413
2690.2 0.000783091019457488
2758.58 0.000732105834713767
2772.14 0.000660031599790854
2794.26 0.00053318647001289
2914.18 0.000484897245040833
2993.08 0.000468142799034201
3050.48 0.000410988765286422
3194.52 0.000375489531397673
3311.36 0.000365233898164106
3373.8 0.000366706581836901
3458.26 0.000355121921425683
3595.54 0.000324888049052027
3675.4 0.000287354537202793
3746.22 0.000268951531781234
3875.46 0.000243065006708306
4001.56 0.000214584597578839
};
\addplot [very thick, royalblue28108204]
table {%
133.44 0.052914131699766
194.035555555556 0.0272909897440479
254.631111111111 0.0165391993803489
315.226666666667 0.0110279662528483
375.822222222222 0.00783618597369246
436.417777777778 0.0058279674698964
497.013333333333 0.00448601845546727
557.608888888889 0.00354722761147311
618.204444444444 0.00286631110764573
678.8 0.00235777356174655
739.395555555556 0.00196867640233161
799.991111111111 0.00166484491618396
860.586666666667 0.00142343616104739
921.182222222222 0.00122872410676928
981.777777777778 0.00106960412537255
1042.37333333333 0.000938060091839143
1102.96888888889 0.000828192340394511
1163.56444444444 0.000735583892385053
1224.16 0.000656876981107601
1284.75555555556 0.000589483860510899
1345.35111111111 0.000531385428161307
1405.94666666667 0.000480988514001797
1466.54222222222 0.000437023124229121
1527.13777777778 0.000398467376646547
1587.73333333333 0.000364491935834079
1648.32888888889 0.000334418381098546
1708.92444444444 0.000307687663528464
1769.52 0.00028383595946192
1830.11555555556 0.000262476008506575
1890.71111111111 0.000243282561680941
1951.30666666667 0.000225980940135684
2011.90222222222 0.000210337969696945
2072.49777777778 0.000196154745670641
2133.09333333333 0.000183260819007454
2193.68888888889 0.000171509494647339
2254.28444444444 0.000160774006321969
2314.88 0.000150944386695004
2375.47555555556 0.000141924892648428
2436.07111111111 0.000133631876447363
2496.66666666667 0.000125992017057628
2557.26222222222 0.000118940843940269
2617.85777777778 0.00011242149958028
2678.45333333333 0.000106383697830994
2739.04888888889 0.000100782843616228
2799.64444444444 9.55792861838516e-05
2860.24 9.07376833628149e-05
2920.83555555556 8.6226458454703e-05
2981.43111111111 8.20173347288655e-05
3042.02666666667 7.80849351693001e-05
3102.62222222222 7.4406437281744e-05
3163.21777777778 7.09612745190508e-05
3223.81333333333 6.77308773059827e-05
3284.40888888889 6.46984478067446e-05
3345.00444444444 6.1848763531431e-05
3405.6 5.91680056617202e-05
3466.19555555556 5.66436086238564e-05
3526.79111111111 5.42641279737782e-05
3587.38666666667 5.20191241057167e-05
3647.98222222222 4.98990596680692e-05
3708.57777777778 4.78952088821118e-05
3769.17333333333 4.59995772208272e-05
3829.76888888889 4.42048301254654e-05
3890.36444444444 4.25042296234998e-05
3950.96 4.08915778691366e-05
4011.55555555556 3.93611667612429e-05
4072.15111111111 3.79077329073356e-05
4132.74666666667 3.65264172993437e-05
4193.34222222222 3.5212729149877e-05
4253.93777777778 3.39625134088854e-05
4314.53333333333 3.27719215417375e-05
4375.12888888889 3.16373852023748e-05
4435.72444444444 3.05555924806248e-05
4496.32 2.95234664420203e-05
4556.91555555556 2.85381457124991e-05
4617.51111111111 2.75969668898906e-05
4678.10666666667 2.6697448589782e-05
4738.70222222222 2.58372769557429e-05
4799.29777777778 2.50142924834162e-05
4859.89333333333 2.4226478025077e-05
4920.48888888889 2.34719478562187e-05
4981.08444444444 2.27489376988581e-05
5041.68 2.20557956077913e-05
5102.27555555556 2.13909736361882e-05
5162.87111111111 2.07530202058656e-05
5223.46666666667 2.01405731154879e-05
5284.06222222222 1.95523531269327e-05
5344.65777777778 1.89871580762474e-05
5405.25333333333 1.84438574611142e-05
5465.84888888889 1.79213874616118e-05
5526.44444444444 1.7418746355396e-05
5587.04 1.69349902922815e-05
5647.63555555556 1.64692293966408e-05
5708.23111111111 1.60206241691127e-05
5768.82666666667 1.55883821618485e-05
5829.42222222222 1.51717549039857e-05
5890.01777777778 1.47700350562293e-05
5950.61333333333 1.43825537754004e-05
6011.20888888889 1.40086782715758e-05
6071.80444444444 1.36478095420353e-05
6132.4 1.32993802676662e-05
};
\addplot [very thick, cadetblue80178158]
table {%
242.86 0.0168749472981206
282.896363636364 0.0194681068262484
322.932727272727 0.0215155742919511
362.969090909091 0.0230702298317119
403.005454545455 0.0241976973381836
443.041818181818 0.0249640678158707
483.078181818182 0.0254303607252255
523.114545454545 0.0256504308762051
563.150909090909 0.0256705853597396
603.187272727273 0.025530001960597
643.223636363636 0.0252614783732917
683.26 0.0248922736092586
723.296363636364 0.0244449258736507
763.332727272727 0.0239379958436817
803.369090909091 0.023386717727589
843.405454545455 0.0228035571886085
883.441818181818 0.0221986829826068
923.478181818182 0.0215803622113177
963.514545454546 0.0209552897336719
1003.55090909091 0.0203288617499319
1043.58727272727 0.0197054025436392
1083.62363636364 0.0190883521835288
1123.66 0.0184804218260725
1163.69636363636 0.0178837221991313
1203.73272727273 0.0172998699177578
1243.76909090909 0.0167300754880424
1283.80545454545 0.0161752161850816
1323.84181818182 0.0156358964325679
1363.87818181818 0.015112497848755
1403.91454545455 0.0146052207417982
1443.95090909091 0.0141141185233843
1483.98727272727 0.0136391262515032
1524.02363636364 0.0131800843013423
1564.06 0.0127367579893189
1604.09636363636 0.0123088538323846
1644.13272727273 0.0118960330072849
1684.16909090909 0.0114979224778182
1724.20545454545 0.0111141241785427
1764.24181818182 0.0107442225777198
1804.27818181818 0.0103877908880634
1844.31454545455 0.0100443961490201
1884.35090909091 0.00971360336716128
1924.38727272727 0.00939497887046391
1964.42363636364 0.00908809300666929
2004.46 0.00879252229462475
2044.49636363636 0.00850785111978868
2084.53272727273 0.00823367305029158
2124.56909090909 0.00796959183760186
2164.60545454545 0.00771522215551886
2204.64181818182 0.0074701901225757
2244.67818181818 0.00723413364568972
2284.71454545455 0.00700670261682328
2324.75090909091 0.00678755898931632
2364.78727272727 0.00657637675626021
2404.82363636364 0.00637284184967908
2444.86 0.00617665197624483
2484.89636363636 0.00598751640269577
2524.93272727273 0.00580515570197324
2564.96909090909 0.00562930146927177
2605.00545454545 0.00545969601566736
2645.04181818182 0.00529609204569391
2685.07818181818 0.00513825232414807
2725.11454545455 0.0049859493364826
2765.15090909091 0.00483896494637204
2805.18727272727 0.00469709005338167
2845.22363636364 0.00456012425311804
2885.26 0.0044278755017782
2925.29636363636 0.00430015978662266
2965.33272727273 0.00417680080357105
3005.36909090909 0.00405762964284494
3045.40545454545 0.00394248448335274
3085.44181818182 0.00383121029632025
3125.47818181818 0.00372365855851091
3165.51454545455 0.00361968697524855
3205.55090909091 0.0035191592133453
3245.58727272727 0.00342194464394983
3285.62363636364 0.00332791809525586
3325.66 0.00323695961495444
3365.69636363636 0.00314895424226447
3405.73272727273 0.0030637917893396
3445.76909090909 0.00298136663182079
3485.80545454545 0.00290157750828131
3525.84181818182 0.00282432732829586
3565.87818181818 0.00274952298885298
3605.91454545455 0.00267707519882451
3645.95090909091 0.00260689831120037
3685.98727272727 0.00253891016279741
3726.02363636364 0.00247303192115136
3766.06 0.00240918793830464
3806.09636363636 0.002347305611207
3846.13272727273 0.0022873152484521
3886.16909090909 0.00222914994307947
3926.20545454545 0.00217274545117898
3966.24181818182 0.00211804007604254
4006.27818181818 0.00206497455761654
4046.31454545455 0.00201349196701637
4086.35090909091 0.0019635376058736
4126.38727272727 0.00191505891029471
4166.42363636364 0.00186800535921938
4206.46 0.00182232838697409
};
\addplot [very thick, chocolate21910927]
table {%
16.58 1.01355787505051
82.6650505050505 0.134154662487269
148.750101010101 0.0588085448724881
214.835151515151 0.0342955036456257
280.920202020202 0.0228805499306358
347.005252525253 0.016523289427305
413.090303030303 0.0125752276662732
479.175353535354 0.0099356166818885
545.260404040404 0.00807391639200868
611.345454545455 0.00670647640320403
677.430505050505 0.00566950070521721
743.515555555556 0.00486258973298335
809.600606060606 0.00422119951503979
875.685656565657 0.00370218683717727
941.770707070707 0.00327576016179586
1007.85575757576 0.00292077286623092
1073.94080808081 0.00262185527800517
1140.02585858586 0.00236760463120357
1206.11090909091 0.00214940746579318
1272.19595959596 0.00196065288791892
1338.28101010101 0.00179619452257337
1404.36606060606 0.0016519748221202
1470.45111111111 0.00152475782044852
1536.53616161616 0.00141193582421013
1602.62121212121 0.00131138745413316
1668.70626262626 0.00122137195201908
1734.79131313131 0.00114044949390228
1800.87636363636 0.00106742041428736
1866.96141414141 0.00100127835939168
1933.04646464646 0.000941173821669034
1999.13151515152 0.000886385496408066
2065.21656565657 0.000836297592056427
2131.30161616162 0.000790381715045756
2197.38666666667 0.000748182300384449
2263.47171717172 0.000709304813269535
2329.55676767677 0.000673406132956874
2395.64181818182 0.000640186667666346
2461.72686868687 0.00060938385194681
2527.81191919192 0.000580766755200344
2593.89696969697 0.000554131588714087
2659.98202020202 0.000529297943403945
2726.06707070707 0.000506105625031237
2792.15212121212 0.000484411980459273
2858.23717171717 0.000464089629446643
2924.32222222222 0.00044502453291685
2990.40727272727 0.000427114341638152
3056.49232323232 0.000410266979574007
3122.57737373737 0.000394399424414893
3188.66242424242 0.000379436654427503
3254.74747474747 0.000365310736103662
3320.83252525253 0.000351960031425426
3386.91757575758 0.000339328507092322
3453.00262626263 0.000327365130943059
3519.08767676768 0.000316023343174155
3585.17272727273 0.000305260591911883
3651.25777777778 0.000295037924310674
3717.34282828283 0.000285319625694025
3783.42787878788 0.000276072900372872
3849.51292929293 0.000267267588712255
3915.59797979798 0.000258875915802058
3981.68303030303 0.000250872267748223
4047.76808080808 0.000243232992158417
4113.85313131313 0.000235936219868175
4179.93818181818 0.000228961705354175
4246.02323232323 0.00022229068362241
4312.10828282828 0.000215905741650068
4378.19333333333 0.000209790702708974
4444.27838383838 0.000203930522112077
4510.36343434343 0.000198311193108083
4576.44848484848 0.000192919661807611
4642.53353535354 0.000187743750160917
4708.61858585859 0.000182772086125545
4774.70363636364 0.000177994040264854
4840.78868686869 0.000173399668107588
4906.87373737374 0.000168979657676279
4972.95878787879 0.000164725281660083
5039.04383838384 0.000160628353766869
5105.12888888889 0.000156681188841262
5171.21393939394 0.000152876566380882
5237.29898989899 0.000149207697123007
5303.38404040404 0.000145668192409127
5369.46909090909 0.000142252036065872
5435.55414141414 0.000138953558568298
5501.63919191919 0.000135767413275687
5567.72424242424 0.000132688554551599
5633.80929292929 0.000129712217598916
5699.89434343434 0.000126833899857607
5765.97939393939 0.000124049343827995
5832.06444444444 0.000121354521195762
5898.14949494949 0.000118745618146886
5964.23454545454 0.000116219021771441
6030.3195959596 0.000113771307464744
6096.40464646465 0.000111399227242924
6162.4896969697 0.000109099698897682
6228.57474747475 0.000106869795921911
6294.6597979798 0.000104706738144049
6360.74484848485 0.00010260788301464
6426.8298989899 0.000100570717493595
6492.91494949495 9.85928504911885e-05
6559 9.66720058199339e-05
};
\addplot [very thick, purple11522131]
table {%
274.5 0.0319497526786542
330.788282828283 0.0271439797318403
387.076565656566 0.0234090487078508
443.364848484848 0.0204369272244378
499.653131313131 0.0180251520198394
555.941414141414 0.0160358304779057
612.229696969697 0.0143720864206564
668.51797979798 0.0129640143649865
724.806262626263 0.011759992678465
781.094545454545 0.0107211297903553
837.382828282828 0.00981760701293628
893.671111111111 0.00902620643060264
949.959393939394 0.0083286006125134
1006.24767676768 0.00771014468209714
1062.53595959596 0.00715900728224948
1118.82424242424 0.00666553489247606
1175.11252525253 0.00622177981887889
1231.40080808081 0.00582114492007624
1287.68909090909 0.00545811286804267
1343.97737373737 0.00512803748092148
1400.26565656566 0.00482698121708512
1456.55393939394 0.00455158740177081
1512.84222222222 0.00429897887049839
1569.13050505051 0.004066676905955
1625.41878787879 0.00385253590940258
1681.70707070707 0.00365469037738134
1737.99535353535 0.00347151157949433
1794.28363636364 0.00330157194186836
1850.57191919192 0.00314361559455671
1906.8602020202 0.0029965338823134
1963.14848484848 0.00285934489693788
2019.43676767677 0.00273117628725012
2075.72505050505 0.00261125075519957
2132.01333333333 0.00249887376490637
2188.30161616162 0.00239342308385496
2244.5898989899 0.00229433984813029
2300.87818181818 0.00220112090107665
2357.16646464646 0.00211331220050235
2413.45474747475 0.0020305031261505
2469.74303030303 0.00195232154858984
2526.03131313131 0.00187842954446925
2582.3195959596 0.00180851966240011
2638.60787878788 0.00174231165949235
2694.89616161616 0.00167954964148466
2751.18444444444 0.00161999955003499
2807.47272727273 0.00156344694951536
2863.76101010101 0.00150969507293291
2920.04929292929 0.00145856309265728
2976.33757575758 0.00140988458669334
3032.62585858586 0.00136350617547809
3088.91414141414 0.00131928630774553
3145.20242424242 0.00127709417700936
3201.49070707071 0.00123680875275699
3257.77898989899 0.00119831791260604
3314.06727272727 0.00116151766351031
3370.35555555556 0.00112631144166871
3426.64383838384 0.00109260948212995
3482.93212121212 0.00106032825023499
3539.2204040404 0.0010293899280267
3595.50868686869 0.000999721949607009
3651.79696969697 0.000971256580157142
3708.08525252525 0.000943930533972348
3764.37353535354 0.000917684627414649
3820.66181818182 0.000892463463166691
3876.9501010101 0.000868215142587722
3933.23838383838 0.000844891003337376
3989.52666666667 0.000822445379751789
4045.81494949495 0.000800835383736044
4102.10323232323 0.000780020704182001
4158.39151515152 0.000759963423136225
4214.6797979798 0.000740627847132534
4270.96808080808 0.000721980352271154
4327.25636363636 0.00070398924177446
4383.54464646465 0.000686624614880221
4439.83292929293 0.00066985824604938
4496.12121212121 0.000653663473568354
4552.4094949495 0.000638015096717535
4608.69777777778 0.000622889280759123
4664.98606060606 0.000608263469070162
4721.27434343434 0.000594116301811515
4777.56262626263 0.000580427540581563
4833.85090909091 0.000567177998555217
4890.13919191919 0.000554349475655486
4946.42747474747 0.000541924698346507
5002.71575757576 0.000529887263674433
5059.00404040404 0.000518221587216331
5115.29232323232 0.000506912854627613
5171.58060606061 0.000495946976505856
5227.86888888889 0.000485310546313608
5284.15717171717 0.000474990801125077
5340.44545454545 0.000464975584981775
5396.73373737374 0.000455253314660467
5453.02202020202 0.000445812947673349
5509.3103030303 0.000436643952335344
5565.59858585859 0.000427736279747117
5621.88686868687 0.000419080337554733
5678.17515151515 0.000410666965358188
5734.46343434343 0.000402487411651334
5790.75171717172 0.000394533312184997
5847.04 0.000386796669653725
};
\addplot [very thick, black18]
table {%
16.68 0.786042967447538
79.7561616161616 0.0627512225786697
142.832323232323 0.0224809112493397
205.908484848485 0.0115271868735355
268.984646464646 0.00699494474140307
332.060808080808 0.00468581355065977
395.13696969697 0.00335090332593563
458.213131313131 0.00251039629911645
521.289292929293 0.00194745519828733
584.365454545454 0.00155232510132722
647.441616161616 0.00126457880048544
710.517777777778 0.00104871096946166
773.593939393939 0.000882747794293203
836.670101010101 0.00075250006295641
899.746262626263 0.000648475164148034
962.822424242424 0.000564129205496286
1025.89858585859 0.000494833424529353
1088.97474747475 0.000437239731729392
1152.05090909091 0.000388878483618625
1215.12707070707 0.000347896195009813
1278.20323232323 0.00031288020419979
1341.27939393939 0.000282738851459633
1404.35555555556 0.000256617963875606
1467.43171717172 0.000233841603583119
1530.50787878788 0.000213869350003386
1593.58404040404 0.000196265049569097
1656.6602020202 0.000180673647783335
1719.73636363636 0.000166803802059548
1782.81252525253 0.000154414685343232
1845.88868686869 0.000143305865844279
1908.96484848485 0.000133309470787685
1972.04101010101 0.000124284064220838
2035.11717171717 0.000116109823955917
2098.19333333333 0.000108684712305415
2161.26949494949 0.000101921413627688
2224.34565656566 9.57448683479083e-05
2287.42181818182 9.00902744932904e-05
2350.49797979798 8.49014582900298e-05
2413.57414141414 8.01295380695727e-05
2476.6503030303 7.5731822766189e-05
2539.72646464646 7.16708991731447e-05
2602.80262626263 6.79138719457005e-05
2665.87878787879 6.44317278782312e-05
2728.95494949495 6.11988018096182e-05
2792.03111111111 5.81923260436588e-05
2855.10727272727 5.53920487187323e-05
2918.18343434343 5.27799093536938e-05
2981.2595959596 5.03397620077697e-05
3044.33575757576 4.80571382516686e-05
3107.41191919192 4.59190435544552e-05
3170.48808080808 4.39137818218919e-05
3233.56424242424 4.20308037353654e-05
3296.6404040404 4.02605752813592e-05
3359.71656565657 3.85944634648978e-05
3422.79272727273 3.70246366939496e-05
3485.86888888889 3.55439777270321e-05
3548.94505050505 3.41460074102932e-05
3612.02121212121 3.28248177066331e-05
3675.09737373737 3.15750127487962e-05
3738.17353535354 3.03916568393954e-05
3801.2496969697 2.92702284804509e-05
3864.32585858586 2.82065796488416e-05
3927.40202020202 2.7196899646556e-05
3990.47818181818 2.62376829494973e-05
4053.55434343434 2.53257005588113e-05
4116.63050505051 2.44579744267257e-05
4179.70666666667 2.36317545867102e-05
4242.78282828283 2.28444986670629e-05
4305.85898989899 2.20938535091346e-05
4368.93515151515 2.13776386474808e-05
4432.01131313131 2.06938314401946e-05
4495.08747474747 2.00405536643259e-05
4558.16363636364 1.94160594142621e-05
4621.2397979798 1.88187241608146e-05
4684.31595959596 1.82470348459398e-05
4747.39212121212 1.76995809029531e-05
4810.46828282828 1.71750461050639e-05
4873.54444444444 1.66722011563591e-05
4936.62060606061 1.61898969492242e-05
4999.69676767677 1.57270584208156e-05
5062.77292929293 1.52826789487412e-05
5125.84909090909 1.48558152327383e-05
5188.92525252525 1.44455826149517e-05
5252.00141414141 1.40511507965417e-05
5315.07757575758 1.36717399128669e-05
5378.15373737374 1.33066169334737e-05
5441.2298989899 1.29550923566517e-05
5504.30606060606 1.26165171714347e-05
5567.38222222222 1.22902800626977e-05
5630.45838383838 1.19758048374594e-05
5693.53454545455 1.16725480526831e-05
5756.61070707071 1.13799968268224e-05
5819.68686868687 1.10976668190873e-05
5882.76303030303 1.08251003619617e-05
5945.83919191919 1.05618647338857e-05
6008.91535353535 1.03075505602573e-05
6071.99151515152 1.00617703320203e-05
6135.06767676768 9.82415703209759e-06
6198.14383838384 9.59436286083073e-06
6261.22 9.37205805238602e-06
};
\addplot [very thick, darkgray153]
table {%
16.68 0.649435888371614
76.04 0.108158612129932
135.4 0.0451198475089225
194.76 0.0246303376672065
254.12 0.0153988173014088
313.48 0.0104619004734361
372.84 0.00752200356447138
432.2 0.0056361891289597
491.56 0.00435845624370039
550.92 0.00345548860181465
610.28 0.0027956399651216
669.64 0.0023001087586682
729 0.00191942878176105
788.36 0.00162130910930547
847.72 0.00138396725616665
907.08 0.00119229297351462
966.44 0.00103554878849815
1025.8 0.000905942575445172
1085.16 0.000797714141396339
1144.52 0.000706534977263917
1203.88 0.000629104425220474
1263.24 0.00056287224454811
1322.6 0.00050584440422725
1381.96 0.000456444815781654
1441.32 0.000413415371591255
1500.68 0.000375742659650015
1560.04 0.000342603544412522
1619.4 0.000313324279606466
1678.76 0.000287349453732892
1738.12 0.00026421816627892
1797.48 0.000243545580455883
1856.84 0.000225008515090286
1916.2 0.000208334100164034
1975.56 0.000193290776968455
2034.92 0.000179681107670189
2094.28 0.00016733599225699
2153.64 0.000156109988260464
2213 0.000145877500599003
2272.36 0.00013652966247959
2331.72 0.000127971768552872
2391.08 0.000120121151988543
2450.44 0.000112905420375623
2509.8 0.000106260983196584
2569.16 0.000100131817418131
2628.52 9.44684284714934e-05
2687.88 8.92269722918963e-05
2747.24 8.43685106954266e-05
2806.6 7.98583776008542e-05
2865.96 7.56656377636013e-05
2925.32 7.17626230141432e-05
2984.68 6.81245336637831e-05
3044.04 6.47290948955403e-05
3103.4 6.15562597040261e-05
3162.76 5.85879513691298e-05
3222.12 5.58078396092516e-05
3281.48 5.32011455119968e-05
3340.84 5.07544711240883e-05
3400.2 4.8455650229845e-05
3459.56 4.62936173844317e-05
3518.92 4.42582927146255e-05
3578.28 4.23404803724537e-05
3637.64 4.0531778838922e-05
3697 3.8824501536878e-05
3756.36 3.72116064324858e-05
3815.72 3.56866334908833e-05
3875.08 3.42436490091532e-05
3934.44 3.28771959834484e-05
3993.8 3.15822497809e-05
4053.16 3.0354178483992e-05
4112.52 2.91887073580719e-05
4171.88 2.8081886963786e-05
4231.24 2.70300644973086e-05
4290.6 2.60298579938186e-05
4349.96 2.50781330750285e-05
4409.32 2.41719819607743e-05
4468.68 2.33087044986297e-05
4528.04 2.24857909949678e-05
4587.4 2.17009066565133e-05
4646.76 2.09518774737322e-05
4706.12 2.02366773968819e-05
4765.48 1.95534166725514e-05
4824.84 1.89003312234267e-05
4884.2 1.82757729670769e-05
4943.56 1.76782009810366e-05
5002.92 1.71061734315569e-05
5062.28 1.65583401922928e-05
5121.64 1.60334360870492e-05
5181 1.55302746976445e-05
5240.36 1.50477426840901e-05
5299.72 1.4584794569732e-05
5359.08 1.41404479488225e-05
5418.44 1.37137790782887e-05
5477.8 1.33039188192799e-05
5537.16 1.29100488974789e-05
5596.52 1.25313984541964e-05
5655.88 1.21672408629814e-05
5715.24 1.18168907888975e-05
5774.6 1.14797014697946e-05
5833.96 1.11550622008385e-05
5893.32 1.08423960053162e-05
};
\addplot [very thick, saddlebrown1356716]
table {%
275.52 0.0110278015432298
313.156767676768 0.0103352438701218
350.793535353535 0.0096679464598576
388.430303030303 0.00903828664922173
426.067070707071 0.00845102122620312
463.703838383838 0.00790688418474378
501.340606060606 0.0074045221874749
538.977373737374 0.00694155639585491
576.614141414141 0.00651517052321294
614.250909090909 0.0061224356395933
651.887676767677 0.00576048609844719
689.524444444444 0.00542661033627804
727.161212121212 0.0051182928257533
764.79797979798 0.00483322816370948
802.434747474747 0.00456931956679324
840.071515151515 0.00432466899929837
877.708282828283 0.00409756318809869
915.34505050505 0.00388645801282144
952.981818181818 0.00368996270019362
990.618585858586 0.00350682461413824
1028.25535353535 0.00333591505013039
1065.89212121212 0.00317621621381062
1103.52888888889 0.00302680942977793
1141.16565656566 0.00288686455023124
1178.80242424242 0.00275563049220443
1216.43919191919 0.00263242681264157
1254.07595959596 0.00251663622386203
1291.71272727273 0.00240769795271067
1329.34949494949 0.00230510185155913
1366.98626262626 0.00220838317627834
1404.62303030303 0.00211711795410234
1442.2597979798 0.00203091887221418
1479.89656565657 0.00194943162549016
1517.53333333333 0.00187233166891644
1555.1701010101 0.00179932132664331
1592.80686868687 0.00173012721544051
1630.44363636364 0.0016644979454771
1668.0804040404 0.00160220206590983
1705.71717171717 0.00154302622677712
1743.35393939394 0.00148677353221292
1780.99070707071 0.00143326206307216
1818.62747474747 0.00138232354974781
1856.26424242424 0.00133380217830524
1893.90101010101 0.0012875535151067
1931.53777777778 0.00124344353688408
1969.17454545455 0.00120134775477698
2006.81131313131 0.00116115042221331
2044.44808080808 0.0011227438176989
2082.08484848485 0.00108602759462177
2119.72161616162 0.00105090819108715
2157.35838383838 0.00101729829359608
2194.99515151515 0.000985116349079888
2232.63191919192 0.00095428612041687
2270.26868686869 0.000924736281097167
2307.90545454545 0.000896400045176964
2345.54222222222 0.000869214829081845
2383.17898989899 0.0008431219421885
2420.81575757576 0.000818066303440341
2458.45252525252 0.000793996181541233
2496.08929292929 0.000770862956527179
2533.72606060606 0.000748620900742472
2571.36282828283 0.000727226977448035
2608.9995959596 0.000706640655468582
2646.63636363636 0.000686823738444361
2684.27313131313 0.000667740207395112
2721.9098989899 0.000649356075430375
2759.54666666667 0.000631639253553244
2797.18343434343 0.000614559426605758
2834.8202020202 0.00059808793849446
2872.45696969697 0.000582197685915765
2910.09373737374 0.000566863019873419
2947.73050505051 0.000552059654345674
2985.36727272727 0.000537764581518421
3023.00404040404 0.000523955993053418
3060.64080808081 0.000510613206908322
3098.27757575758 0.000497716599268082
3135.91434343434 0.00048524754118611
3173.55111111111 0.00047318833956854
3211.18787878788 0.000461522182166611
3248.82464646465 0.00045023308627086
3286.46141414141 0.000439305850826774
3324.09818181818 0.00042872601171512
3361.73494949495 0.000418479799961549
3399.37171717172 0.00040855410265954
3437.00848484848 0.000398936426408355
3474.64525252525 0.000389614863083831
3512.28202020202 0.000380578057774446
3549.91878787879 0.000371815178728482
3587.55555555556 0.000363315889170275
3625.19232323232 0.000355070320854695
3662.82909090909 0.000347069049239171
3700.46585858586 0.000339303070161864
3738.10262626263 0.000331763777923141
3775.73939393939 0.00032444294467527
3813.37616161616 0.000317332701032434
3851.01292929293 0.000310425517819717
3888.6496969697 0.000303714188885744
3926.28646464646 0.000297191814909161
3963.92323232323 0.000290851788134275
4001.56 0.000284687777975822
};
\addplot [draw=black, fill=black, mark=x, very thick, mark size=2.5pt, only marks]
table{%
x  y
67.92 0.3383996024071
275.52 0.0639824753778923
1121.28 0.00773404899693277
4464.64 0.000681339364709533
};

